Effective Technical Reviews

There are two ways to check if a program is correct, namely execute it or review it. While executing a program is the ultimate test for its correctness reviewing the program can occur earlier in its development and find problems if done effectively. This work focuses on review techniques. It enables the programmer to effectively review a program and find a range of problems from concurrency to interface issues. The review techniques can be applied in a time constrained industrial development context and are enhanced by knowledge on programming pitfalls.

==> Business.tex <==
\chapter{Optimal Integration of the ML Solution in the Business Decision Process}
\label{optimal}

As previously discussed ML embedded systems are non deterministic.  They make mistakes by design.  What we hope to achieve instead of a bug free system is a system for which the error on the choices we want to utilize in the business decision process is statistically controlled.  Such control enables the appropriate allocation of human resources for the correction of errors made by the ML embedded system and the insurance that overall we obtain a stable process that increases the profit of the organization.  In addition, the way the ML embedded system is used may need to be updated over time as the factors impacting the performance of the ML embedded system may change.  The last issue, drift identification, was dealt with in chapter \ref{Chapter:drift} while the question of statistical control was studied in chapter \ref{Chapter:MLtesting}.    

The ML embedded system is integrated in a business process and should help increase value obtained from the process by the organization.   For example, there are many consideration involved in reaching a decision of whether or not to give a loan to a bank's customer.  One of the consideration is if the loan payments to the bank will occur on time.  Assume that we have developed a ML embedded system that predicts if the loan will be paid on time by a given customer. We want to integrate the prediction of the system in the overall decision process followed by the bank.  The embedding should be made in such a way that the bank will maximize the profit from giving loans to customers.  Giving loans that will be paid on time and not giving loans that will not be paid on time can help maximize the overall bank profit but this is not the only consideration.  Other considerations may apply and influence the final bank decision.   For example, if the bank can get the payments for the loans by other means such as accessing the customers assets.  Let's spell out two fundamentally different ways in which we can integrate the ML system in the business process.
\begin{enumerate}
    \item If we can trust the recommendation of the ML system we can just act according to the recommendation.  For example, a software problem is reported.   The software is composed of components.  Each component has an owner that can solve problems of the component that she owns.  If we can trust the ML system to route the software problems correctly most of the time we can just route them automatically according to the ML recommendation.   As long as the routing recommendation made by the ML system is mostly correct the value from the business process is clear as we no longer require a team to route the software problems to the appropriate component.
    \item The ML system recommendation is correct most of the time but can not be "blindly" trusted.  In our problem routing scenario a person is required to consider each ML recommendation.   This can still be beneficial as given the recommendations, especially if the ML system provides the reasons for the recommendation, the time required to route each software problem is reduced. 
    \item A hybrid case.   There are some conditions in which we have established, through an appropriate experiment, that we can trust the ML system "blindly" and some conditions for which we need a person to inspect the recommendation and make the final decision.  A simple example of that is if we have established that for some software components we can route the problem report automatically according to the ML system recommendation and for some components we can not and a person should make the final decision.
\end{enumerate}

If the ML recommendation is not followed blindly (cases two and three above), a person sometimes should make the final decision taking into account the ML recommendation or potentially ignoring it all together.  In this situation whether or not the person makes a correct decision depends on the incentive defined by the organization.  Thus, as part of the optimal business definition process, if there are decision points in which a person needs to make a decision while taking into account a ML system recommendation that can not be fully trusted, optimal incentives should be defined for that person.  This calls for the application of mechanism design, see \href{https://www.investopedia.com/terms/m/mechanism-design-theory.asp}{link}.   We will attempt to get a better understanding on how this can be achieved in practice in the next section.

\section{Business process optimization and incentive design}

We start with an example of optimization of the business process associated with the ticket routing ML embedded system.  The ML embedded system uses several models and utilizes different parts of the problem report such as the report text and the report meta data.  In addition, the system may utilize other sources of information such as the software installation configuration.   Finally, the system may also use some deterministic rules based on certain error codes.  For example, if out of memory error is reported route the problem to the memory management of the software.   As discussed in chapter \ref{unitSystem}, the ML system is thus typically composed of a hybrid decision tree.  We are emphasising this as one may think the assumptions we are making next only apply to a single model and they typically do not.   Hence the consistent use of the terminology ML embedded systems throughout this work.  

We assume that the software has four components, namely, $c_1, c_2, c_3, c_4$.   Previous experiments have shown that the average conditional probability of correct routing decision given that the decision is one of the components,$c_1, c_2, c_3, c_4$. is  $P(correct|c_1) = 0.6, P(correct|c_2) = 0.7, P(correct|c_3) = 0.8, P(correct|c_4) = 0.9$ respectively.  A human resource is available that can analyze the problem and correctly route it at the cost of 1 unit.   We are also given that the observed probabilities of reporting a problem by the ML system from each of the components $c_1, c_2, c_3, c_4$ is $\frac{1}{4}$.  The average performance of the system if the human resource is not used is thus
$\sum_{i = 1, 2, 3, 4}\frac{1}{4}P(correct|c_i) = 0.75$.  We consider applying the human resource only in case that the system predicts $c_1$ which we refer to as the elimination of $c_1$ policy.   On the average that will be a quarter of the time, so on the average we expect to pay 250 units of payments in a 1000 software problems.   What is the expected performance of the joint business process that utilizes the human resource in that way?   It is expected to be completely correct for $c_1$ thus $P(correct|c_1) = 1$.  We will have the average performance of $\sum_{i = 1, 2, 3, 4}\frac{1}{4}P(error|c_i) = 0.85$.  We thus increased the average performance of the system from $0.75$ to $0.85$ at a cost of 250 units of cost in a 1000 software reported problems.  This highlights the trade-off involved in applying the human resource.  Consider the following exercise to better understand the concept. 

\begin{exercise}
Assume the routing problem as explained above.  
\begin{enumerate}
    \item What will be the average performance if we only eliminate policy $c_2$?  Same question for policy $c_3$ and $c_4$?  What are the average costs in that case?
    \item We randomly choose to apply the human resource in probability $p$. What will be the average performance of the system and the average cost in this case?
    \item You are given a budget of 100 cost units per a 1000 software problems how would you spend it?  What will be the average performance then?
    \item What is the standard error of an elimination policy $c_i$ given that we know that the standard errors of each of the conditional probability $P(correct|c_i)$ from previous experiments?  How would you check the stability of an elimination policy?
    \item What will be the impact of change in the probability of the ML system reporting a problem in a components.  For example, what will be the impact of the ML system reporting a $c_1$ problem in probability $0.7$ and $c_2, c_3, c_4$ in probability $0.1$ each?  Assume the conditional probabilities of the ML system being correct given the component prediction stays the same.  Explain why such a phenomenon is possible?
    \item What will be your recommendation if you do not have an estimate of the probability in which the ML system will choose one of the components? Explain.
\end{enumerate}
\end{exercise}

We can thus consider a general category of policies, namely elimination of $c_i$ given that the ML system recommended routing to $c_i$ in probability $p_i$.  The expected accuracy in such a case will be 
$\sum_{i = 1, 2, 3, 4} \frac{1}{4}(p_i + (1-p_i)P(correct|c_i))$.  We denote this expected accuracy by $P(correct|p_1,\ldots,p_4)$.  We can think of our problem as the problem of maximizing $P(correct|p_1,\ldots,p_4)$ under a given budget con train. We are ensured that this optimization problem has a solution.  See next exercise for details. 

\begin{exercise}
Show that $P(correct|p_1,\ldots,p_4)$ is continuous and that the set of possible utilization of the budget constrains, e.g., if the budget is 250 cost units per a 1000 software problems and is utilized so that $\frac{1}{4}(p_1+p_2+p_3+p_4)1000 = 250$, is compact.  Deduce that the optimization problem has a a maximum.  See appendix for details on why this is the case.     
\end{exercise}

In a way the above approach to the problem is the simplest possible approach as either the ML embedded system is making the routing decision or the human resource does.  Concerns are thus "separated".   We can measure the performance of the ML embedded system when its decision is trusted and separately measure the performance of the human resource when she makes the decision on the routing.  In other words, for each routing decision there is a single "owner", either the ML embedded system or the human resource.  Next we consider a more hybrid scenario in which the two are brought together to make the final decision.

Assume that the human resource spends up to some time bound on the routing decision and that the accuracy is proportional to the time spent.  For example, assume that the human resource spends up to 2 hours on the routing decision and that the accuracy in routing of a decision that was made after t time is $\frac{t}{2}$.  The cost now of applying the human resource is the overall time that the human resource spent on making routing decisions.  We also assume that other assumption on the routing problem and the ML embedded system remain the same.  Assume that the overall time the user can allocate for a 1000 software problems is T. The human resource can perfectly handle $n = \frac{T}{2}$ routing decisions (ignore the reminder).  One approach could be to assume that we have n cost units as before and solve the previous optimization problem.  

\begin{exercise}
Assume the routing problem described above.  Further assume that we would like to raise the average accuracy from $0.85$ to $0.9$.  One way to achieve that would be to spend $0.9 \times 2$ time on each routing decision for which the ML embedded system recommended $c_1, c_2, c_3$.  This will raise the the conditions probabilities $P(correct|c_i), i=1, 2, 3$ to $0.9$.  How big should T be to implement this approach?
\end{exercise}

We now consider the problem of incentive.   We observe that there are two different type of decision makers.  The first design the overall business process.   For example, decides what type of elimination policy to choose in the problem routing example.   The second decision are the decision made by a human resource that participate in the decision process.   In our routing problem example the human resource making the routing decision.  The first principle of incentive definition is to tie incentive to the 
the part of the organization business goal controlled by the decision maker.  In our ticket routing example the decision maker that optimizes the entire business incentive should be tied to the entire business process performance.  For example, in the ticket routing example the business process optimizer should be rewarded for a decrease in the overall time required to solve problems, a decrease in the overall expense required to solve the software problems, and so on.  In contrast, the human resource used to route software problems only controls the correct and efficient routing of a given software problem.  Thus, she needs to be rewarded in proportion to volume of correct routing and in reverse proportion to time it took her to make the decision.  Note to provide such incentives the organization will need to measure the performance of the system.   This should be thus part of the system requirement and experiment design from day one of the ML embedded system development!   

\begin{exercise}
Consider the bank loaning example.  Assume that two ML embedded system are developed.  The first estimates if a loan will be return on time by a customer with accuracy 0.8.  The other ML embedded system estimate if a customer will increase her business with the bank as a result of given a loan.  There are budget con trained human resources that can make the two decisions.  The bank is expanding so if the business with the customer is likely to increase and the customer is likely to pay the loan the bank policy is to given it.  Define appropriate optimization process and incentives for the business process optimizer and human resource decision maker.  Make additional assumption as needed similar to the one made in previous exercises of this chapter.  
\end{exercise}







==> MLtesting.tex <==
\chapter{ML Testing}
\label{Chapter:MLtesting}




\begin{comment}


\newglossaryentry{Monte Carlo}
{
    name=Monte Carlo,
    description={The central limit theorem states that the samples average of a random variable converges to the normal distribution.  Monte Carlo techniques utilizes utilizes the central limit theorem and computation power to calculate averages that are analytical manageable. }
    
}





\end{comment}


\begin{comment}

\section{Target audience} 
The book's target audience includes the following two type of practitioners.  
\begin{enumerate}
    \item Practitioners who want to ensure optimal and stable over time integration of AI with the business process and organization decision making in a way that optimize the business process.  
    \item Practitioners responsible for the governance of AI embedded systems. 
\end{enumerate}

\section{Book extended abstract}


Book outline 

Motivation 
The AI promise and it’s challenge.   Just give it a lot of data.  Non deterministic system.  Data changes of time. Decision under uncertainty.    The approach. 

Given an example of when statistics is not needed.


Fundamentals and their usage in Ai system operations

Probability classical and Bayesian 

Statistics 

Non parametric statistic 

Generalization and control

Statistical experiments 

Measure the business value 

Decision theory games 

Optimal business process integration 

Advance topics 

Governess and trust fairness privacy security. And all the rest

Black box models model readability and why you made that decision 

Engineering composition of models effect on control 


Should the book enable access to methods that are needed instead of reading end to end?



The following sections include some sample material. 

\end{comment}

As discussed in previous chapters ML based systems are becoming embedded in our everyday life. This chapter outlines how to confidentially engineer ML infused systems.  Indeed, it is challenging to build ML infused systems that we can rely on. Cutting to the heart of the matter: ML infused systems contain ML models. Such models are non deterministic and may sometimes make the wrong decision.  To handle the system inherit non determinism, we introduce statistical experimental design and explain how it is utilized to control the errors introduced by a ML infused system and thus make it reliable.     

This chapter is organized as follows.  We first introduce the problem of controlling ML infused system quality through an ideal and simple example and then deep dive into the design of statistical experiments and how they are used to develop, analyze and validate high quality ML based systems. At the heart of the chapter lies the identification of a random variable that represents a desired behaviour of the system and the analysis of its average and standard deviation.  This, in turn, let us define an envelope of control under which the system behaviour is acceptable.  The chapter builds on chapter \ref{Chapter:scientific-method} that discusses the design of statistical experiments to drive the development of ML based systems.

\section{Business grade ML solutions}

We are going to discuss the creation of business-grade ML solutions. The objective is to create an ML solution decision makers can use to guide their decisions with confidence or even let the ML solution make decisions without a human in the loop. This is not new.  For years statistics has been used to guide decisions and make them with confidence. For example, a production line is only profitable if up to $5\%$ of its produced items are defective.  We sample the production line every $20$ minutes and determine the percentage of defective items in the sample.  Apply a statistical test or a confidence interval that was previously developed we determine if production should be stopped and the production line re-tuned as there are too many defects making the current production not profitable.  The decision is made at a certain confidence level as there are probabilities associated with the two types of errors that we can make; The first is that the production line is profitable when it is not and the second is that the production line is not profitable when it is.

%TBD statistical test, confidence interval
%TODO formally explain what we mean by the performance of a ML model. Loss function choice and business value 

We make the following crucial observation.   ML solutions are a complicated version of the above production line example.  They are heavily dependent on data and are random by nature.  In other words, if a fresh training data sample is chosen the resulting ML model and its performance will change.  Thus, repeating the learning process on two different samples of training data will probably produce two slightly different ML models.  Also by definition sometimes ML models are correct and sometimes they are not correct! It's the nature of the beast.     

In order to achieve business-grade ML solutions we need to statistically control the solution error.  The following is meant by statistical control.  The solution performance, say accuracy, is a random variable.  We would like to be able to claim the following type of claim: with probability of error of no more than $5\%$, the accuracy of the solution lies between $84\%$ to $87\%$.
We call this interval a control interval as this interval is used to "control" the ML performance and determine if it is within the expected bounds.  

In other words, we want to be able to say what the expected performance of the system will be and quantitatively determine the probability we will make a mistake.  If we are able to do that we will also be able to determine if a ML solution is performing correctly in the field as we should rarely, if ever, see a performance that is outside the control interval.


Our approach as mentioned before is \gls{non parametric} as for modern ML infused systems it is hard to determine a distribution family and fit a distribution to the data.  Another motivation to the use of \gls{non parametric} approaches is the availability of modern computers. Utilizing the computation power of modern computers we will be able to rely on approaches such as \gls{bootstrapping} and Monte Carlo\footnote{Eitan - explain what Monte Carlo is.} to develop our ML infused system's control.  

We will start by studying how to estimate any random variable distribution in a \gls{non parametric} way.  This will serve as the foundations for our first ideal control interval example.  

For those not familiar with parametric confidence intervals it is recommended to review \ref{parametricControl} at this point.

\section{Random variables and empirical distribution}
\label{randomVariable}

We are given a probability space $(E, \Omega, P)$, $\Omega \subseteq P(E)$.  E is the set of possible events that can occur when we run our experiment.  Sometimes E is referred to as the set of elementary events to distinguish from subset of E which are also referred to as events.   $\Omega$ is a set of subsets of E.  We refer to elements of $\Omega$ as events.  For the purpose of this chapter it is enough to think of $\Omega$ as the set of all possible subsets of E.  A random variable is simply a function from E to the real numbers, $X : E \rightarrow R$.
We define the distribution function associated with a given random variable X, $F : R \rightarrow [0, 1]$ by $F(x) = P(\{\omega \in E | X(\omega) \leq x \}) = P(X \leq x)$.  Thus, the value of the distribution function is a function from R, the real numbers, to numbers between 0 and 1 such that the value of F at x, $F(x)$, is the probability that the random variable will get a value that is less than or equal to x.   The following example and exercises clarify these definitions.

\begin{example}
Consider a fair dice.   In that case, $E = \{1, 2, 3, 4, 5, 6\}$ which are the possible results of a throw of the dice and we consider each possible result to be equally likely.  Thus, $P(i) = \frac{1}{6}, i = 1, \dots, 6$. As $E$ is finite, all possible subsets of $E$ are possible events in the probability space.  Thus, $\Omega = P(E)$.  A possible event is the event of getting some even number when throwing the dice.  It is represented as $EVEN = \{2, 4, 6 \}$ and is indeed a subset of E.  In addition, $P(EVEN) = P( \{2, 4, 6 \}) = \frac{3}{6} = \frac{1}{2}$.  Let us define a random variable $X(i) = i, i = 1, \ldots 6$.  We then have $F(3) = P(\{\omega \in E | X(\omega) \leq 3 \}) = P(\{1, 2, 3\}) = \frac{3}{6} = \frac{1}{2}$.  
\end{example}

\begin{exercise}
\label{Chapter:MLtesting:Excercise:distribution}
Calculate $F(i)$ for $i \in \{-1, 0, 1, 2, 5, 6, 10, 10.1\}$.
\end{exercise}

As part of our experiment that tests the ML based system we focus on some random variable and estimate different aggregates of the random variable behaviour such as its average.  We would like to do that in a robust manner without assuming anything about the distribution.  As an example, in the case of a chatbot ML based system we would like to determine the average number of service calls that will be routed to a human agent. We would like to be able to say that on the average, say, 20$\%$ of the calls will be routed to a human agent.  In addition, we would like to say that with high confidence the average will fall between 18$\%$ to 22$\%$ of the calls.  In order to do that we would need to estimate the distribution of the random variable. We next study the concept of the empirical distribution that will let us estimate the distribution of the random variable.   

We are given a sample, $S = \{x_1, \ldots, x_n\}$ of the random variable, chosen randomly and independently from $E$.  Next, we define the empirical distribution function, $F_e(x) = \Sigma_{i \in S} \frac{I(x_i \leq x )}{n}$ where $I(condition)= 1$ if the condition is true and $0$ otherwise. Intuitively, $F_e(x)$ estimates the probability that the random variable will have a value that is less than x, i.e., $P(X \leq x)$, by determining the percentage of the elements of the sample S that are less than x.  The next example helps clarify the concept.

\begin{example}
Consider the fair dice again. Define the random variable to be $X(i) = 1$ if and only if $i$ is even and zero otherwise.   Assume we got the following sample 
$S = \{ 0, 0, 1, 1, 1, 0, 1, 1, 0\}$.   Then $F(0) = P(\{1, 3, 5\}) = \frac{1}{2}$ as $X(1) = X(3) = X(5) = 0 \leq 0$ but $F_e(0) = \Sigma_{i \in S} \frac{I(x_i \leq 0 )}{n} = \frac{4}{9}$.  Importantly note that the empirical distribution is not equal to the distribution of the random variable.  
\end{example}

The following exorcise develops the intuition of when the empirical distribution represents the distribution of the random variable.  In fact, as the size of the sample increases the empirical distribution converges to the distribution of the random variable.  

\begin{exercise}
\label{Chapter:MLtesting:Excercise:emericalDistribution}
Write a simulation that obtains a large S from a fair dice distribution.   What is $F_e(0)$ converging to?   Same question for $F_e(1) - F_e(0)$?

Solution can be found in Appendix \ref{chapter:solution_appendix} in \ref{Chapter:MLtesting:Excercise:emericalDistribution_sol}
\end{exercise}

TBC - add material on average and variance here or in the appendix by expanding \ref{probability}. 

Recall that the Bernoulli distribution, $Br(p)$, is obtained by a trail that has success probability $p$. Success is denoted by $1$ and failure by $0$. For each point, $x_i$, in the sample $S$, $P(x_i \leq x) = F(x)= P(I(x_i \leq x ) = 1)$.   Thus, the random variable $I(x_i \leq x)$ is distributed Bernoulli with probability $F(x)$.   Or $I(x_i \leq x)  ~~_{\tilde{}}~~Br(F(x))$. We thus have $E(I(x_i \leq x)) = F(x)$ and $V(I(x_i \leq x)) = F(x)(1-F(x))$.

Let's pause here to better appreciate what have just happened.  We are taking a \gls{non parametric} approach.   One of the fundamental patterns of \gls{non parametric} statistics has just been realized above.  The argument above applies for any distribution $F()$.   Regardless, we have made an observation that connected the statistics of interest, in this case, $I(x_i \leq x)$, with some known distribution,$Br(F(x))$, thus returning to the well known grounds of parametric statistics!. \footnote{Eitan - clarify - add some definitions and examples to distinguish between parametric and non parametric statistics.}

\begin{exercise}
Using the fact that $I(x_i \leq x)$ is distributed Bernoulli prove that $E(I(x_i \leq x) = F(x)$ and $V(I(x_i \leq x)) = F(x)(1-F(x))$. As a consequence what is the average and variance of $F_e()$?  
\end{exercise}

As a consequence $E(F_e(x)) = E(\Sigma_{i \in S} \frac{I(x_i \leq x )}{n}) = \frac{\Sigma_{i \in S} E(I(x_i \leq x )}{n} = \frac{n F(x)}{n} = F(x)$.   $F_e(x)$ is thus an unbiased estimator of $F(x)$.  In addition, $V(F_e(x)) = V(\Sigma_{i \in S} \frac{I(x_i \leq x )}{n}) = \frac{\Sigma_{i \in S} V(I(x_i \leq x )}{n^2} = \frac{nF(x)(1-F(x))}{n^2} = \frac{F(x)(1-F(x))}{n}$.   The important point to note here is that as $n$ grows the variance of $F_e(x)$ vanishes making $F_e(x)$ an excellent estimate of $F(x)$. 

Let's take a deep dive into the behaviour of the empirical distribution.  

\begin{definition}
We are given a sequence of random variables $X_1, X_2,\ldots$ with a corresponding distribution functions $F_1(), F_2(),\ldots$.   In addition, we are given a random variable $X$ with distribution function $F()$.  We say that $X_1,X_2,\ldots$ converges in distribution to $X$ at $x \in R$ if $F_n(x) \rightarrow F(x)$.  If that is the case for each $x \in R $ for which $F()$ is continuous we say that $X_1, X_2,\ldots$ converges to $X$ in distribution.   
\end{definition}

\begin{exercise}
\label{excercise:525_gn_fn}
Consider the series of functions $f_n(x) = \frac{1}{2}(1-\frac{1}{n})^2x+(1-\frac{1}{n})$, $n \in N$.   Show that for each $n \in N$, the function $g_n(x) = f_n(x)$ if $-\frac{1}{(\frac{1}{2}(1-\frac{1}{n}))} \le x \le 0$ and $0$ otherwise is a density function.  Also show that for each $x \in R$,  the series $f_n(x)$ converges as $n$ goes to infinity to $f(x) = \frac{1}{2}x+1$.   Show that $g(x) = f(x)$ if $-2 \le x \le 0$ and $0$ otherwise is also a density function.  Is it also true that the random variables defined by $g_n(x) = \frac{1}{2}(1-\frac{1}{n})^2x+(1-\frac{1}{n})$ converges in distribution to $g(x)=\frac{1}{2}x+1$?   If this is the case what needs to be proven?

\href{https://colab.research.google.com/github/GuysBarash/MLBook/blob/main/ex_5_2_4.ipynb}{Click here for a simulation} or see appendix \ref{chapter:solution_appendix} in solution \ref{excercise:525_gn_fn_sol}

\end{exercise}



\section{Control interval example with unlimited sampling with replacement}

%control interval, ML model, deployment time, label data,bootstrapping Monte Carlo techniques, non-parametric statistics, statistics, 

We provide an example of obtaining a \gls{control interval} for a \gls{ML model}.  We assume unlimited access to labeled data that represents data at deployment time.   That is an ideal assumption. Much of our discussion in latter sections will focus on how to remove that assumption using \gls{bootstrapping} and Monte Carlo techniques but the 
\gls{non parametric} statistical approach will remain the same.   As previously mentioned, We will be applying mostly non parametric statistics throughout this chapter as we typically do not know the type of probability distribution.  This is another complication that is typical to modern ML work.  An exception to this rule is when we are dealing with averages and large samples.   The central limit theorem will then guaranty that the distribution of the average converges to the normal distribution and we'll be able to use that to utilize parametric techniques.     



We assume a model $f()$  was developed that given an image $x$ determines if $x$ is a dog or a cat.  As we are given access to unlimited set of labeled data of cats and dogs that represents the data we will encounter when the model is deployed, we sample from the data and get a fresh set of labeled cats and dogs 
$(x_i, y_i), i=1, \ldots, n$. $x_i$ are the images and $y_i$ is the label $y_i \in \{cat, dog\}$.  We then calculated the sampled accuracy $a = \frac{\sum I(f(x_i) = y_i)}{n}$ where $I(c)$ is the indicator function that is equal to $1$ if the condition, $c$, is true and zero otherwise. 

We make the following observation. If we repeat the above procedure, and obtain a fresh random sample, we will get different results for the accuracy.  Thus, accuracy is a statistic that estimates the real accuracy of $f()$.  In order to determine the actual accuracy with high confidence we need to develop a control interval.   We proceed as follows.  We repeat the above procedure $k$ times and obtain $k$ accuracy scores $a_1, \ldots, a_k$.  We order them in descending order, wlog, $a_1 \ge a_2 \ge , \ldots , \ge a_k$.  We take away $2.5\%$ of the first numbers in the list and $2.5\%$ at the end.  The remaining numbers define the control interval.   The accuracy will lie in this interval in probability $95\%$.  

\begin{example}
We make the connection to the empirical distribution studied in the previous section explicit through an example.  Assume $k = 1000$ and $a_i = i$.  Thus, $2.5\%$ of the top will be the $25$ numbers $1000,\ldots,976$ and the bottom $2.5\%$ will be the the $25$ numbers $1,\ldots,25$. According to the definition of the empirical distribution, $P_e(a \leq 25) = \frac{25}{1000} = 2.5\%$, and $P_e(a \leq 975) = \frac{975}{1000} = 97.5\%$.   Thus, $P_e(a > 975) = 1-\frac{975}{1000} = 2.5\%$.  It turns out that $P_e( 25 < a \leq 975) = 95\%$.  As discussed in the previous section, when $k$ grows that will be a better and better approximation of the unknown $P()$ distribution.  
\end{example}\footnote{Eitan - check why $P_e$ is used here and not P.   Also give a continuous example.}

\begin{exercise}
Repeat the example with $k=100$ and $a_i = i$.  Be careful to handle the boundaries correctly.  
\end{exercise}

\begin{example}
\href{https://colab.research.google.com/drive/1CIA9_CHjoqAaLrrDwSdExffKcPtC6AmE?usp=sharing}{Click here for an example of a non parametric confidence interval.}  As the data is sampled from the normal standard distribution, and we take 2.2$\%$ of the largest and smallest points we expect the $96\%$ confidence interval to be approximately $[-2, 2]$ when the sample size increases.  
\end{example}


\section{Bootstrapping}

Bootstrapping is a way to overcome budget limitations.    Ideally we would like to obtain a set of fresh samples as previously explained and obtain a confidence interval for the accuracy or other performance measures of the ML model using non parametric statistics. As discussed this is then used to anticipate and control the performance of the system in the field.  Additional usage includes to compare models and determine if indeed one of them is better than the other or if the difference in their performance is a result of noise.  We thus see that the techniques we are discussing here influence the end to end process of development of a ML solution.  We deep dive into that the coming sections.  

In practice we can not obtain unlimited number of fresh data samples representing the field data.  In fact, if we are lucky, we have one sample that represents the field data and is labeled.  As long as this sample is not used for training the model we can use it to estimate the field behaviour of the model, but how do we overcome our budget limitation, namely, having only one sample?  We follow the bootstrapping procedure to obtain new data samples.   We call such data samples bootstrapped data samples.  Technically, we repeatably sample with replacement from the one sample that we have to get our new sample and then proceed as before.   
To understand bootstrapping consider a data sample of blue and red balls.  The probability of getting a blue ball is $\frac{1}{3}$ but we do not know that.  If the data sample is big enough we will have roughly $\frac{1}{3}$ of the balls being blue.   This is the big "if"  of bootstrapping - we require that the data sample distribution represents the real distribution.   Now if we sample balls randomly from the data set we will get a new data set that will also have the $\frac{1}{3}$ blue balls proportion. It is "as if" we have sampled a fresh sample where as we actually sampled from our existing sample.   This is the core idea behind bootstrapping.  We can do that as many times as we like to get a set of "fresh" samples and then apply the non parametric procedure described in the beginning of the chapter for the dogs and cats classification example to obtain a confidence interval on the accuracy. We treat the bootstrapped samples as fresh samples hence the name "bootstrapping".        

\begin{example}
\href{https://colab.research.google.com/drive/1XbuklUZrB5h6wUneAMJhboaIGCnSEZXV?usp=sharing}{Click here} to see an example of a bootstrapping and non bootstrapping confidence interval for the balls. The expected range should be around $\frac{1}{3}$.  Note that the sample size should be big enough in order for the bootstrap confidence interval to work.
\end{example}


\begin{example}
\href{https://colab.research.google.com/drive/1v6VudBYzgrymG-ZjQqMTWKlsvRm0GAUb?usp=sharing}{Click here for an example of trained models performance analyzed non-parametric confidence interval.}
\end{example}

\begin{exercise}
\label{mlTesting:dataBalance}
Bootstrapping can be also used when training a ML model.  In this exercise we consider how.  A training set, D, of 200 images of cats and 800 images of dogs is given. 
\begin{enumerate}
    \item If you sample with replacement from D 2000 times what is the average number of cat images that you are going to get?
    \item Can you change the sampling procedure so that the average number of cats will be $\frac{1}{2}$
    \item How will you use the second sampling method in the training of a ML model that classifies dogs and cats?
\end{enumerate}
\end{exercise}

\section{Using the central limit theorem instead}

Given our idealized assumptions of independent random sampling with replacement the central limit theorem could have been applied as well in order to obtain a confidence intervals.  In any case, it is a good idea to apply, if possible, more than one method to validate the confidence interval being developed.  

Recall that the normal variable is close under linear transformations.   Specifically if $X$ is normally distributed $N(\mu, \sigma)$ then $Y = aX+b$ is distributed with normal distribution $N(aX+b, |a|\sigma)$. 


\begin{exercise}
Prove that 
if $X$ is normally distributed $N(\mu, \sigma)$ then $Y = aX+b$ is distributed with normal distribution $N(aX+b, |a|\sigma)$. Is that correct for $a = 0$?
\end{exercise}

The central limit theorem states that if $X_1, \ldots, X_n$ are sampled independently from an identical unknown distribution $F()$ that has a finite average $\mu$ and a finite standard deviation $\sigma^2$ then setting $S_n = \frac{\Sigma_{i= 1}^{i = n} X_i}{n}$ we have that $\frac{\sqrt{n}(S_n - \mu)}{\sigma}$ approaches the standard normal distribution, $N(0, 1)$, for sufficiently large $n$.  

Setting $a = \frac{\sigma}{\sqrt n}$ and $b = \mu$ we get that $\frac{\sigma}{\sqrt n}(\frac{\sqrt n(S_n - \mu)}{\sigma}) + \mu$  is distributed $N((\frac{\sigma}{\sqrt n})0+\mu, (\frac{\sigma}{\sqrt n})1 = N(\mu, \frac{\sigma}{\sqrt n})$. In other words, $S_n$ is distributed $N(\mu, \frac{\sigma}{\sqrt n })$. Thus, in order to develop a confidence interval we need to estimate the average and standard error of $S_n$ assuming it is normally distributed.  

TBC - explain the difference between the two possible estimates to the standard deviation as n is large it does not matter.  Give a Python example.

\begin{example}
\href{https://colab.research.google.com/drive/1L2n-9wsPbjq8_5kikkVRjfuC4078-276?usp=sharing}{Click here} for an example of how a large sample that is distributed normally can be used to estimate its average and standard deviation and thus obtain a confidence interval.  
\end{example}





%\section{Related work}

%In this work confidence intervals guaranties are derived - \href{http://ceur-ws.org/Vol-2808/Paper_33.pdf}{link}.

%In this work the relation between shallow approximation of the neural network and learning is studied - \href{https://arxiv.org/pdf/2102.00434.pdf}{link}.

%In this work calculating of VC dimension is studied \cite{DBLP:journals/corr/ManurangsiR17}.

==> ScientificMethod.tex <==
\chapter{Scientific Analysis of ML Systems}%The Scientific Approach to AI Analysis}
\label{Chapter:scientific-method}
A major objective of an ML project is to facilitate learning of general models from data. A significant risk of an ML project is failure to generates successful models, which deems the ML project ineffectual.  %Typically, training data will also serve as input to the ML solution once it is deployed. 
A fundamental assumption of ML theory is that the data used for learning is representative of the data that will be encountered once the ML solution is deployed.  Thus,  the primary requirement from a good learning system is generalization, i.e., the ability to generate rules that will perform well on data input that is of the same sort of the data used for training.  
For example, an ML model that was trained to identify a human face on data that includes all types of animal and human faces may not perform well when presented with an image of a car.  %As typical in software engineering, this significant ML project risk should be addressed first. 

In software engineering, significant project risks are typically addressed first. We advocate that ML projects should not be an exception.
Thus, one should first address the question of whether, given the available data and the business requirements, the ML system can successfully learn. To address this concern, we design experiments whose results indicate whether the ML system can learn, and at what quality. An additional result of the experiments should typically show the type of decomposition to components, or the preferred architecture the system should have.  Another result of the analysis of experiments is the focusing of future experiments on specific aspects of the system. %suggestion of next development iteration typically formalized through additional experiments.  

\begin{example}
In this example we show how ML based architectures can be selected through the process of experiments and their analysis. Consider a scenario in which a consultant assists a bank customer in investment planning and profiling. An ML system is developed to support that process. 
%The ML based system helps consult an investor and design their investment profile and risk level.  
The ML system needs to determine the preferred risk profile of the investment, e.g., what percentage of the investment will be in saving instruments, government bounds and stocks. To this end, it should determine major future expenses such as kids' college tuition, buying a new house or annual vacations. The available database includes investors' personal profiles, past investment history, and assets inventory. There are many possible architectures of the intended ML system. For instance, it can consist of one monolithic ML model. In contrast, %and on the other end of the spectrum, we 
it can comprise several ML models: one to predict the desired investment risk level, and a few others for each major expense, e.g., buying a house. It is alternatively possible to have a single model for all of the expenses. The output of the models that predict expenses can serve as input for the risk level model.  Chapter \ref{mindDirecting} provides insights into the trade-off among the architectures.  As the experiments are done on data that represent typical data that will be encountered by the ML system at deployment time, the performance of the different architectures in the experiments represents their projected performance once the ML system is deployed.  Thus, 
the experiment let us compare possible architecture and select the best alternative.  Note that in order to do that it is enough to build the models described above and connect them for the purpose of running the experiment and it is not required to build the entire system in order to do that.
\end{example}

\begin{exercise}
A self-driving car is trained using data on traffic in Tokyo.   The manufacturer claims that the car can drive in large European cities as they are similar to Tokyo.  Form an opinion about the claim and discuss relevant factors that you think impact the self-driving car's performance.  What  experiment might validate the manufacturer's claim?
\end{exercise}


It is useful to draw an analogy with the Test First \cite{} software development process. In Test First, a functional test is written before the code is implemented.  The test formally defines what the system is required to do.  The code that is implementing the functionality captured by the test is then implemented.  Next, the test is executed against the code.  If the test passes, then the code is OK.  The test is added to a set of passing tests that accumulate and serve as a functional test suite of the system being developed.  At every development stage, all tests in the test suite must pass before the next test is designed.  

%In the case of a ML solution, an experiment is defined instead of a test.

% The 
% Theory and Practice of Quality Assurance for Machine
% Learning SystemsAn Experiment Driven Approach
% Samuel Ackerman1, Guy Barash3, Eitan Farchi1, Orna Raz1, and Onn Shehory2
% 1IBM Haifa Research Lab2Bar Ilan University3Western Digital
% 2022
% Contents
% 1 Introduction 2
% 2 The Scientific Approach to AI analysis 6
% 2.1 The scientific method . . . . . . . . . . . . . . . . . . . . . . . . . . . . . . 7
% 2.2 Mapping the scientific method to ML development . . . . . . . . . . . . . . 8
% 2.3 Conjectures . . . . . . . . . . . . . . . . . . . . . . . . . . . . . . . . . . . . 10
% 2.4 Experimental design . . . . . . . . . . . . . . . . . . . . . . . . . . . . . . . 11
% 3 Pitfalls and Best Practices for the Machine Learning Designer and Tester 14
% 3.1 Overview . . . . . . . . . . . . . . . . . . . . . . . . . . . . . . . . . . . . . 14
% 3.2 From day one determine if the data is relevant for the business objective . . 14
% 3.3 Think science and experiments . . . . . . . . . . . . . . . . . . . . . . . . . 15
% 3.4 Data must be of valuable volume; When not to use learning . . . . . . . . . 15
% 3.5 Use all relevant data and information: Do NOT ignore structure . . . . . . 16
% 3.6 Is the training data representative of deployment data? . . . . . . . . . . . 16
% 3.7 Get to a supervised learning problem . . . . . . . . . . . . . . . . . . . . . . 17
% 3.8 Minimize manual labeling, instead utilize experiments, rules and boosting . 17
% 4 Unit Test vs. System Test of ML Based Systems 18
% 5 ML Testing 23
% 5.1 Business grade ML solutions . . . . . . . . . . . . . . . . . . . . . . . . . . . 23
% 5.2 Random variables empirical distribution . . . . . . . . . . . . . . . . . . . . 24
% 5.3 Control interval example with unlimited sampling with replacement . . . . 25
% 5.4 Bootstrapping . . . . . . . . . . . . . . . . . . . . . . . . . . . . . . . . . . . 26
% 5.5 Using the central limit theorem instead . . . . . . . . . . . . . . . . . . . . 27
% 6 Drift Detection and ML Solution Retraining 28
% 6.1 Types of drift . . . . . . . . . . . . . . . . . . . . . . . . . . . . . . . . . . 28
% 6.2 Measuring distribution differences . . . . . . . . . . . . . . . . . . . . . . . 30
% 6.2.1 Two-sample distribution difference measures on X . . . . . . . . . . 31
% 6.2.2 Two-sample distribution difference measures on y . . . . . . . . . . . 32
% 6.3 Drift in characterizations of data . . . . . . . . . . . . . . . . . . . . . . . . 32
% 6.3.1 Drift in data slices . . . . . . . . . . . . . . . . . . . . . . . . . . . . 32
% 6.3.2 Drift in density-based slices . . . . . . . . . . . . . . . . . . . . . . . 33
% 6.3.3 Drift in feature polynomial relations . . . . . . . . . . . . . . . . . . 34
% 6.4 Sequential drift detection . . . . . . . . . . . . . . . . . . . . . . . . . . . . 35
% i
% 7 Optimal Integration of the ML Solution in the Business Decision Process 36
% 7.1 Business process optimization and incentive design . . . . . . . . . . . . . . 37
% 8 A Detailed Chatbot Example 40
% 8.1 Chatbots as a ML embdded system . . . . . . . . . . . . . . . . . . . . . . . 40
% 8.2 Quality challenges . . . . . . . . . . . . . . . . . . . . . . . . . . . . . . . . 41
% 8.3 Control for chatbot success . . . . . . . . . . . . . . . . . . . . . . . . . . . 42
% 8.4 Trend analysis . . . . . . . . . . . . . . . . . . . . . . . . . . . . . . . . . . 42
% A Solutions 44
% B Annotated References 45
% ii

%using an appropriately designed statistical experiment that estimates the expected average
%and variance of those measures. A good experiment will provide accurate estimates of the
%requirement measures when the ML based system is deployed. This practice tackles the
%challenge of crafting a robust ML solution.
%Creating a good set of training examples for a given requirement is challenging too. The
%data may be lacking criteria without which the desired model cannot make correct decisions.
%We might have too few examples, or examples that are not representative of the type and
%distribution of data that the system will encounter when the model is applied. Finally,
%in order to guide the learning, the data needs to include the ”correct answer” as well as
%indication that it is indeed correct. Such indication is typically provided by labeled data, in which case the problem is a supervised learning problem. However, it often happens that
%an organization holds a representative set of examples that is readily available but are not
%labeled.
%As suggested above, this book aims to address the challenges of crafting robust ML
%solutions that meet their design requirements and hence can be confidently deployed. We
%focus on an experimental approach to the crafting of ML solutions. This approach can be
%thought of as the ML equivalent of the test-first approach applied with regular software.
%To emphasize this similarity, we name our approach experiment-first. The focus of this
%approach is on crafting, validating, and continually monitoring ML-based solutions via
%a series of carefully designed experiments at different levels of abstraction. The book is
%self-contained and addresses the mathematical and statistical techniques needed to apply
%the experiment-first approach. It contains numerous practical programming as well as
%theoretical exercises and their solutions. Exercises are an integral part of the text and are
%designed to facilitate understanding of the ideas, concepts and methods introduced.
%The main target audience of this book is data scientists who craft ML-based solutions,
%architects who define what the solutions need to do, and testers who need to validate that
%the system actually works and meets its specifications. The book also attempts to bridge
%communication gaps between the stakeholders involved in the development of ML-based
%solutions. The experiment-first approach introduced in this book facilitates an end-to-
%end, unambiguous, quantitative definition of the steps to be taken in the development of
%an ML-based system. Our approach details the activities performed, and the artifacts
%consumed and generated, throughout the development and deployment of the solution.
%The book introduces the statistical experiment and its results as the language by which the
%stakeholders communicate effectively to craft the ML-based solution.
%A preferred way to design and implement experiments entails following a scientific ex-
%perimental methodology. This methodology includes the definition of a problem, the for-
%mulation of a quantitative conjecture, and the design and implementation of an experiment
%that validates or rejects the conjecture. For example, a problem could consist of finding
%the speed at which a ball will touch the ground when dropped from a high tower. The
%conjecture is that the speed is proportional to the time, and the experiment involves drop-
%ping balls from towers of different heights and measuring how long it takes them to hit the
%ground.
%This book is organized as follows. In Chapter 2 we paint in broad strokes the scientific
%method and highlight its relation to ML system development and validation. As mentioned
%in the previous paragraph, following the scientific method includes defining a problem,
%making a conjecture that may solve it, and then designing and implementing an experiment
%to check and validate the conjecture. When crafting an ML-based solution, the problem is
%defined by the system requirements. The standard conjecture entails generalization, namely,
%3
% experiment results are used to determine whether the system meets the requirements, but with two major differences:  (1) the experiment result is a statistic, e.g., an average, and not a success or pass binary result; and (2) the experiment result may help us choose among design alternatives. 

In the case of an ML system, an experiment is defined instead of a test. The experiment's
results are used to determine whether the system meets the requirements, but with two
major differences: (1) the experiment's result is a statistic, e.g., an average, and not a
success or a pass binary result; and (2) the experiment's result may help us choose among
design alternatives.

\begin{exercise}
\label{estimatePrecentage}
Given a number, x, a function returns $x^2$ most of the time, i.e., in p percentage of the cases.  Write a test that finds the percentage p.  How is that different from a test that checks that a deterministic function correctly evaluates $x^2$ ?

\href{https://colab.research.google.com/drive/1uO8CDjovgLwVng2rVFnfri9tPKWJBBAo?usp=sharing}{Click here for a Solution.} or see code in \textit{Solutions} appendix \ref{estimatePrecentage_sol}.
\end{exercise}


\begin{exercise}
Test First goes hand in hand with automation; we require that the test suite can be executed and its pass or failed results determined programmatically.  What is the analogous requirement in the case of an experiment-based approach to ML development? 
\end{exercise}

We thus advocate that a good ML development process should consist of a series of statistical experiments.  The results of each experiment reduce the risk of the project and help determine its architecture.  %It is similar to a sail boat that depends on the direction of the wind  -  the data in our case is the wind.  
This approach, which we call Experiment First, focuses on simultaneous consideration of the data \textit{and} the business goal from day one. In what follows, we delineate the design and analysis of statistical experiments and discuss their applicability to the implementation of the Experiment First approach.

TODO:  add a general mapping of the scientific approach to AI analysis to setup the stage for the more detailed discussion in latter chapters in second part of the book.

\section{The empirical methodology}

The scientific empirical methodology includes problem consideration, conjecture formulation, design of experiments that can validate or refute the conjecture, and analysis of the results of the experiments.   Insights from that analysis may lead to new conjectures and new experiments, and the process can iterate.

The scientific empirical methodology is general. It applies to problems such as finding a cure for a disease, discovering the laws that govern the dynamics of bodies, or determining whether a production line is reliable.  Experiments that validate conjectures made regarding such problems are typically designed using statistics as an underlying technique. In Section \ref{} we explore the design and analysis of statistical experiments, with a focus on ML. Prior to that, we exemplify the scientific empirical methodology via a mechanics problem.


\begin{example}
The problem is to determine the rule that governs the fall of bodies on Earth.  We drop a small metal ball from a height of 2 meters and use a camera to determine where the ball is after 1 ms, 2 ms, etc. We repeat the experiment several times.  Analyzing the results, we see that the location of the ball at time t, $x(t)$, is given by a formula of the form $x(t) = At^2$, where $A$ is determined by the experiment.  We are happy and declare victory - in determining the rule of falling bodies.
\end{example}

\begin{exercise}
Can you suggest factors that were ignored in the experiment above and may have changed the result?  Hint - think about experimenting with other, different objects.   
\end{exercise}

It turns out that designing good experiments may be challenging. %is tricky as it requires domain knowledge. 
In that design, one needs to consider the factors that influence the results of the experiment. However, without domain knowledge, this is a difficult task. %which is hard to do if we lack that knowledge.  
For instance, in the experiment above, factors such as wind or the nature of the object being dropped, e.g., a feather instead of a metal ball, are applicable to the Earth but not to the Moon. Similarly, domain knowledge is key to successful design of ML solutions. This is wide agreement is often expressed through feature engineering, among other techniques. Feature engineering is the practice of designing the features extract from the raw data that will be used in the learning process. %What is less obvious is that 
Apparently, domain knowledge is also key to the analysis and validation of ML solutions. The Experiment First approach emphasizes this point. In this approach, domain knowledge is embedded in the validation process through careful design of the experiments and identification of the factors that govern them.  We next consider the relationship between the scientific empirical methodology and the ML solution development process.

\section{Mapping the scientific empirical methodology to ML development}

As discussed above, the scientific empirical methodology includes defining a problem, coming up with a conjecture and the design, implementation and analysis of an experiment that confirms or rejects the conjecture. In the case of ML embedded systems, the problem is expressed in the form of a business requirement.  For example, the bank would like to develop a system that determines whether a customer should be given a loan.  The conjecture may be that the personal and past data on the customer financial transactions is sufficient to develop an ML model that determines whether the bank can profit from giving the loan. The experiment should determine the performance of the ML system on a new and representative set of customers. That is, it should check whether the ML model was able to determine correctly, based on customer unseen personal and financial transaction data %that the model has never seen before if 
whether the bank will profit from giving the loan or not.  

Key points in the design and analysis of the experiment include translating the business objective to quantitative measures that can be measured in the experiment, determining the factors that are impacting the experiment, insuring coverage of these factors, and statistically analyzing experiment outcomes to reliably deduce results from the outcomes. Error and randomness should be taken care of when analyzing and interpreting the results. The last point is illustrated by the next thought exercises.

\begin{exercise}
Consider the tossing of two coins, 100 times each.  %This is done for two coins.  
The first coin turns head 80 times and the second coin turns head 85 times.   Is the second coin more likely to turn head than the first one?  Discuss why it may be the case that it is not.  How would you go about increasing your confidence that the coins have a different chance of turning head? 
\end{exercise}

\begin{exercise}
The bank also has data  on whether or not its customers paid previous loans.   Using that data customers who previously paid on time are labeled as  customers that  "can be given a loan" but if they did not pay on time they are labeled as "can not be given a loan" .    Only using data available before the loan was given, two  ML models that predict if the customer can be given a loan are developed.  Next the percentage of correct  answers the models gave  is calculated on a fresh set of customers that were given a loan.   One model predicts correctly 80 percent of the time and the other 85 percent of the time.   Which model is better and how is the answer to the question related to the previous question with the coin tossing?
\end{exercise}

It is important to note when analyzing ML embedded systems that randomness is ingrained in the  solution.  If we use the two models developed for loan prediction in different time windows we expect percentage of the correct  answers to change. We are thus interested in whether or not most of time it is likely that the percentage of correct  prediction of one model is going to be larger than the  percentage of the correct prediction of the other model.   This is a statistical question and requires statistical techniques we will develop in chapter \ref{Chapter:MLtesting}.  


Two other points are interesting to note when considering the bank loan example.  The translation of the business requirement to a quantitative measure is a non trivial part of the system definition as well as the experiment definition.  In our case, a customer could be late, but not too much, and still the bank may make a profit on the loan.  Thus, other more refined labels could be defined.  In addition, there are customers that were never given a loan.  Maybe such customers are of different "type"?  Maybe our prediction will not work well on customers that were never given a loan?  Consider the following thought exercise. 

\begin{exercise}
Can you suggest a new experiment that will help distinguish if the models have different performance on customers that were never given loans before?  What would be a conjecture in this case?
\end{exercise}

We could distinguish between customers that were given a loan only once and customers that were given a loan more than once. We can then take the label for loan payments for each loan the bank gave to the customer separately.  We can thus have a model for customers that were given the loan for the first time and design a second experiment that determines if the model work well on  such customers.  In fact we have identified a factor that governs the experiments, namely, whether or not customers are given a loan for the first time and an implicit requirement - the model should preform well on customers that are given a loan for the first time as well as on customer that were previously given a loan.  Such a factor identification leads to an architecture question - should we have two models one for customers that were never given a loan before and one for customer that were?  

\begin{exercise}
How would you determine which architecture option to take?
\end{exercise}

We have seen how business requirements are translated into quantitative ML embedded systems performance requirements on fresh data.  We also seen how an experiment designed to validate initial models lead to the identification of factors governing the experiment, the identification of not yet articulated business requirements and the design of additional tests to validate the evolving ML embedded solution performance and determine its architecture.  Next, we will discuss each stage of the scientific method in the context of ML in more details.  

A comment on randomness is in order.  When we say that we choose a fresh sample, we mean that we randomly choose a new set of customers.  If the choice is skewed, for example with more customers that were previously given a loan, then the percentage we obtain may be skewed and not reflect the real behavior of the system.  The important point is that randomness will take care of factors that impact performance even if we have not yet identified them -  a fundamental principle of statistical experiment design that applies to the crafting and analysis of ML solutions.  We will revisit this point in various ways throughout this book. 

\section{Conjectures}

We next continue in the discussion of the relation between the scientific method and the development of a ML embedded system and recall that the scientific method includes the following steps - problem definition, conjecture formulation and experiment design.  The problem is defined by the system requirements and the conjecture is driven from them.  Deriving the conjecture includes the translation of the system requirements to a quantitative measure and the identification of factors that govern the quantitative measure and desired performance expressed using this measure.   Typically, the ML conjecture is that independent of the governing factors the quantitative measure desired performance can be learned. Learned here means that the ML embedded system 
will preform according to the desired level as measured by the performance measure on new data that was never used in the training of the ML models embedded the system.

Interestingly the step of quantifying the system requirements and the factors that govern them help identify system requirements that are not a good candidate to be implemented as a ML embedded systems.   Generally speaking systems could be too complex or too simple to be good candidates for a ML emended implementation.  If a close form of the relation between the governing factors and the desired performance can be expressed and only the optimal parameters that define the relation obtained, the desired system is a too simple to be a good candidate for a ML embedded implementation.  The example of the law of mechanics that were given above is a good example of such a system.   On the other hand, if the governing factors are hard to identify and it is not clear of what type the relation that implements the system is the system is too complex and will probably not be a good candidate for a ML embedded system implementation.  An example of that is a long term accurate weather predication systems.  There is a sweet spot in between of the two extreme which serves as a good candidate for a ML embedded solution which we discuss next.

A good ML solution candidate will at least meet the following criterion. 
\begin{enumerate}
    \item We are able to quantify the business requirements.
    \item The factors that govern the business requirements can be identified.
    \item We identify a search space in which we can search for a good solution automatically.  This is sometimes referred to as the learning phase and the search space is referred to as a model (e.g., a regression, a neural network with some specific architecture or a decision tree).
\end{enumerate}

The last requirement is many times met implicitly by choosing a ML learning method that previously worked well in some domain, e.g, convolution neural network (CNN) for anomaly detection. Making it an explicit step increases the chance of successful learning.  In addition, autoML \cite{???} can help automate this step.  The following exercise is designed to help clarify the concepts of a model and model choice. It requires experience in the use of ML libraries and training.  If such experience is not available it is recommended that the reader will go through some tutorial on linear regression using Python before attempting the exercise.  

\begin{exercise}
\label{Chapter:MLtesting:Excercise:parabola}
A parabola, i.e., $f(x) = ax^2+bx+c$, is given. 100 samples $D = \{(x_1, f(x_1)), \ldots (x_n, f(x_n))\}$ are obtained by randomly choosing $x_1 \ldots x_n$ and then calculating $f(x_1), \ldots, f(x_n)$.  D is used to train a linear regression model of the form $g(x) = dx+e$. 
\begin{enumerate}
    \item Do you expect the results to be good?  Explain your reasoning.  
    \item Implement the above scenario using standard learning libraries.  Validate whether or not the obtained linear regression was good.
    \item Provide a graph view that presents $f()$ and the linear model obtained by applying the regression on D.  How does that help understand the performance of the linear model?  
    \item Is there any pair of parameters d and e of $g() = dx+e$ that will work well?
    \item Use the following feature engineering.  Define $D^{'} = \{ ((x_1,x_1^2), f(x_1)) \ldots ((x_n, x_n^2), f(x_n))$.  Apply linear regression on the new data set.  Did the results improve?  Can you explain why?
    \item What will happen if you add some noise to the data?   Concretely, randomly choose some $noise_i$ from the standard normal distribution, $N(0, 1)$, $n$ times and change the data to $D = \{(x_1, f(x_1) + noise_1), \ldots (x_n, f(x_n) + noise_n)\}$.  How would your answers change given the new data set?
    
    \item Does the size of the dataset $D$ matters? if so, how?
\end{enumerate}

\href{https://colab.research.google.com/drive/15Quc4KJ9CTVBIui3-ylCQpcXo8lR0DgY?usp=sharing}{Click here for Colab Solution} or in the solution appendix \ref{Chapter:MLtesting:Excercise:parabola_sol}

\end{exercise}


TBC - explain how the parabola example is related to the model concept.  



TBC 

\section{Experimental design}

We have discussed derivation of a quantitative performance measures from business requirements and the identification of factors that impact the performance measure.   In the language of statistical experiments a performance measure is referred to as the dependent variable and the factors that impacts the performance measure are referred to as the independent variables. Our implicit conjecture is that regardless of the value of the dependent variables the performance of the ML embedded system on new unseen data will meet the require performance level as defined on the performance measure.   For example, the performance level may require that the average percentage of wrongly predicting that the bank will make a profit when giving a loan to a customer is 10\%.  In addition, its variance is required to be small.   

In order to conduct the experiment, we will 
typically collect a set of input data and apply the ML based system on the data to obtain an estimate on the performance of the dependent variable. We would like the identified independent variables to appear in the data. In reality one can not expect to identify all of the independent variables.  We thus expect to have some latent variables, possibly with their value appearing in the data, that impact the dependent variable we are estimating.  Unfortunately, the dependent variables may not even be in the data.  
  
Denote the dependent variable by Y, the identified independent variables by $X_i$ and the unidentified independent variables by $X^l_j$.  As we collect our data for our experiment we need to take into account the following.

\begin{itemize}
\item Make the data records as comprehensive as possible.  Include available features in the data record, e.g., age of the customer, if available even if it is not required as input to the ML based system and it is not identified as an independent variable.  This will allow for further analysis aimed at discovering the latent variables $X^l_j$.
\item Avoid bias.  Avoid collecting the data in a way that consistently favour some data record features.  One of the ways to mitigate the issue of latent variables is to randomly sample the experiment data.   If this is not done fundamental assumptions underlying the theory and practice of ML are broken.  In addition, by randomly sampling the data the impact of latent variables $X^l_j$ appearing in the data is amortised and we can still estimate the behaviour of the dependent variable Y although we did not identify the latent variable.
\item Choose whether or not to stratify values of dependent variables.  For example, we are given a medical system that decides if a new drug's side effect should be reported to the government based on medical reports.  An independent variable is the type of the report.  There are two types of medical reports - hand written reports and digital reports.  We may be interested in the system performance when the report type, X is $X = handWriten$ and when $X = digital$.  We will thus have two different predictions, one for each value of the independent variable X.  This is called stratification. On the other hand, we may choose not to stratify the independent variable.  That brings us back to the randomization guideline.  We need to take extra care that the variable is not biased.  For example, if our sampled data mostly have digital reports we can not expect to draw conclusions about the performance of the ML based system on hand written reports.   When do we stratify?  When we want the analysis and predication at that level of details to clarify if the system really meets the business requirement. the business requirement in our case is that the the system will work well on both values of the variable X (hand written and digital).   Note the obvious dilemma.  If we stratify all possible values of the independent variable $X_i$ we will get a combinatorial explosion of stratified values.  we will revisit this issue later in the chapter.   
\end{itemize}

The following exercise is designed to demonstrate the concepts of randomness and stratification.  

\begin{exercise}
The unknown relation the system had to learn is $f(X, Y, Z) = X + Y^2 - Z^3$.  X and Y take values in $\{-1, 1\}$ while Z is a number, $Z \in R$.  We identified the independent variable X.  Data was sampled as follows.  X was set to -1, Y was randomly chosen. Z was randomly chosen from a normal distribution with average 5 and variance 1. 
\begin{enumerate}
\item How is the data biased?
\item Suggest a correction to the sampling method
\item How would you conduct a stratification on X?
\item What are the hidden variables?
\item Assume that the system was implemented as $g(X, Y, Z) = Z + Y^2 - Z^2$.  Implement an experiment that analyze the performance of this system and suggest ways to identify that Z is a dependent variable.
\end{enumerate}
\end{exercise}

The following exercise is designed to shade light on sampling challenges used to collect the data.  

\begin{exercise}
The ML systems attempts to determine if a child will graduate from school.  Two independent variables are considered, namely, the child's neighbourhood and the size of the child's family.  It is desired that the ML system will have the same level of prediction regardless of the values of the independent variables and we are collecting data to measure and determine if this is indeed the case (the experiment).  Three sampling methods are considered as follows.
\begin{enumerate}
    \item Randomly choose a child
    \item Randomly choose the family size, then randomly choose a family of the chosen size, then randomly choose a child in the family that is attending school
    \item Randomly choose a neighbourhood, then randomly choose a family that lived in the neighbourhood in the last 5 years and then randomly choose a child in that family    
\end{enumerate}
Can you identify bias introduced by the sampling techniques above?  Assume the first technique produced a sample of 100 children and non comes from a family of more than 6 children. Can you still estimate the performance of the ML system?   What would you suspect if no child from a family of one child was chosen in the sample?
\end{exercise}












==> abstract.tex <==
\begin{abstract}
    

This book teaches the art of crafting and developing ML based systems.
Crafting machine learning  (ML) based systems that are business-grade and can be used by a business is highly challenging. It requires statistical control throughout the system development life cycle. 
This book advocates an "experiment first" approach stressing the need to define statistical experiments from the beginning of the system development life cycle.   
It does so through introducing methods for careful quantification of business requirements and identification of key factors that impact the business requirements. This reduces the risk of a project or ML system development failure.    The quantification of business requirements results in the definition of random variables representing the system key performance indicators that need to be analyzed through statistical experiments.  In addition, available data for training and experiments impacts the design of the system.  Once the system is developed, it is tested and continually monitored to ensure it meets its business requirements.  This is done through the continued application of statistical experiments to analyze and control the key performance indicators.   
This book also discusses in detail how to apply statistical control on the ML based system throughout its lifecycle. 
\end{abstract}


==> acronyms.tex <==
\DeclareAcronym{etf}{
	short = ETF,
    long = Exchange-Traded Fund,
    tag = abbrev
}

\DeclareAcronym{aum}{
	short = AUM,
    long = Assets Under Management,
    tag = abbrev
}

\DeclareAcronym{sr}{
	short = SR,
    long = Sharpe Ratio,
    tag = abbrev
}

\DeclareAcronym{nyse}{
	short = NYSE,
    long = New York Stock Exchange,
    tag = abbrev
}

\DeclareAcronym{hft}{
	short = HFT,
    long = High Frequency Trading,
    tag = abbrev
}

\DeclareAcronym{pv}{
	short = PV,
    long = present value,
    tag = abbrev
}

\DeclareAcronym{fv}{
	short = FV,
    long = future value,
    tag = abbrev
}

\DeclareAcronym{ir}{
	short = IR,
    long = interest rate,
    tag = abbrev
}

\DeclareAcronym{capm}{
	short = CAPM,
    long = Capital Assets Pricing Model,
    tag = abbrev
}

\DeclareAcronym{apt}{
	short = APT,
    long = Arbitrage Pricing Theory,
    tag = abbrev
}

\DeclareAcronym{sma}{
	short = SMA,
    long = simple moving average,
    tag = abbrev
}

\DeclareAcronym{mvo}{
	short = MVO,
    long = mean variance optimization,
    tag = abbrev
}

\DeclareAcronym{rmse}{
	short = RMSE,
    long = root mean square error,
    tag = abbrev
}

\DeclareAcronym{kNN}{
	short = kNN,
    long = k-nearest neighbor,
    tag = abbrev
}

==> algorithms.tex <==
\chapter{Machine Learning Algorithms}
\noindent In most cases, machine learning algorithms are focused on building a model. Then, the model can be used to take inputs and give outputs based on the model. The model is a tool to predict outputs based on the inputs. In our case, we will be using models to take information about stocks and predict their future prices.
\begin{figure}[h]
\centering
\begin{tikzpicture}
  [node distance=.8cm,
  start chain=going below,]
  	\node (data) [punktchain] {Data};
    \node (ml) [punktchain, join=by {->}] {Machine Learning};
      \node (model) [punktchain, join=by {->}]  {Model};
      \begin{scope}[start branch=venstre,
        %We need to redefine the join-style to have the -> turn out right
        every join/.style={->, thick, shorten <=1pt}, ]
        \node[punktchain, on chain=going left, join=by {<-}]
            (inputs) {Observation $\vec{x}$};
      \end{scope}
      \begin{scope}[start branch=hoejre,]
      \node (finans) [punktchain, on chain=going right, join=by {->}] {Prediction y};
    \end{scope}
  % Now that we have finished the main figure let us add some "after-drawings"
  %% First, let us connect (finans) with (disk). We want it to have
  %% square corners.
\end{tikzpicture}
\end{figure}

\noindent So we use machine learning to take historical data and generate a model. When we want to use it, we give the model observations, $\vec{x_i}$, and it gives us predictions, $y$. Examples of good inputs (predictive factors) are:
\begin{enumerate}
	\item Price momentum
    \item Bollinger value
    \item Current price
\end{enumerate}
\noindent while examples of outputs would be:
\begin{enumerate}
	\item Future price
    \item Future return
\end{enumerate}
\noindent We'll first talk about Supervised Regression Learning.

\section{Regression and Modeling}
\noindent Supervised Regression Learning means that we'll provide (supervised learning) a bunch of example data $(x,y)_i$ and allow the model to make a numerical prediction (regression). There are two main types of regression techniques:
\begin{itemize}
\item Linear regression (parametric)
\item \ac{kNN} (instance-based), the more popular approach
\item Decision trees
\item Decision forests
\end{itemize}

\section{Assessing a Model}
Assessing a model is much like predicting prices as it uses indicators to judge the effectiveness of the model. The first indicator is \ac{rmse}, which is as follows
\begin{align*}
\sqrt{\frac{\sum(y_{test}-y_{predict})^2}{N}}
\end{align*}
The error that is important is that of test data, which is outside of the training data. Typically 60\% of the data is used for training, and 40\% is used for testing. However, sometimes there isn't enough data to adequately evaluate a learning algorithm, in which case a method called \textbf{cross validation} is used. This method slices the data into chunks, typically fifths. One is chosen as test and the rest are for training, then a different chunk is chosen to be the test and another trial is run. For financial data, we don't want to accidentally look forward in time, so we would only use \textbf{roll forward cross validation}. This simply demands that all the training data is before the test data. \\

The second metric for how well an algorithm is working is the \textbf{correlation} of the test data and predicted values. Strong correlation, close to $\pm$1, indicates a good algorithm whereas a weak correlation, close to zero, indicates a poor algorithm. Correlation and \ac{rmse} are excellent indicators on how well an algorithm is doing, but we might also want to fine tune an algorithm; we want to answer the question "when are we trying too hard to fit data?". This is where \textbf{overfitting} comes into play. Overfitting is the point at which error for training data is decreasing while error for test data is increasing.
\begin{figure}[h]
\centering
\includegraphics[scale=.6]{images/overfit.JPG}
\end{figure}

\section{Types of Learners}

\paragraph{Ensemble Learners}
Ensemble learners are composed of several different learners, which could include \ac{kNN}, regression, and decision tree learners in one. The output of this learner is then simply a combination of the learners' answers, which is typically an average of the outputs.

\paragraph{Bagging and Boosting}
Boot-strap aggregating, or \textbf{bagging}, only uses one algorithm, but many different models. If the training data is separated into learning instances where there's a total of $n$ instances, then each model is fed a bag of these instances. Each bag is composed of $n'$ learning instances that are randomly selected with replacement, so instances may show up more than once in the same bag. These are used to train $m$ models and the result is the average of all the outputs. \textbf{Boosting} builds each subsequent bag based on the results of the last. Training data is also used to test the models, and a model's predicted data showing significant error is weighted to more likely be in the next bag for the next model. The process is continued for the desired number of models, and the results are averaged. Although this could be advantageous in predicting outliers, it's also more susceptible to overfitting.

\subsection{Reinforcement Learning}
As seen in figure 4.1, reinforcement learning describes the interaction of a robot with its environment. The robot performs an action, which has an effect on the environment and changes its state. The robot observes the change in state and its associated reward and makes decisions to maximize that reward.

\begin{figure}[h]
\centering
\includegraphics[width=6cm]{images/rl.png}
\caption{A diagram of how policy learning works}
\end{figure}

Reinforcement learning also describes the problem that is how to go about maximizing the reward. In the stock market, the reward is return on trades, and we want to find out how to maximize returns. This problem is complicated by time constraints. The value of future gains diminishes with time, so it's unreasonable to use an infinite horizon on which to base returns. However, optimizing returns over too short a time may limit rewards from seeing a much larger overall gain.

\subsection{Markov Decision Problems}
\noindent What we've been talking about is called a Markov decision problem. Here's how the problem is formalized.

We have:
\begin{itemize}
\item Set of states $S = \{s_1, \ldots, s_n\}$
\item Set of actions $A = \{a_1, \ldots, a_n\}$
\item Transition function $T[s,a,s']$
\item Reward function $R[s,a]$
\end{itemize}

\noindent What we're trying to find is a policy $\pi(s)$ that will maximize the reward. Unfortunately, we don't know the $T$ or $R$, since that's defined by the environment. So, the learner has to interact with the world and see what happens. Based on the reward, it can start generating policies.\\

\noindent A way to encode this information is using \textbf{experience tuples}. Experience tuples are as follows: given a state $s_1$ and an action $a_1$ that we took, we were put into state $s_1'$ and got reward $r_1$. The tuple is shown like this:

\begin{equation*}
\langle s_1, a_1, {s_1}', r_1 \rangle
\end{equation*}

\noindent Now, we can rename ${s_1}'$ to $s_2$, since that's our new state, and then take a new action and see what happens, and we get a new tuple:
\begin{equation*}
\langle s_2, a_2, {s_2}', r_2 \rangle
\end{equation*}

\noindent And we repeat this for many different combinations of states and actions, and then we'll use the tuples to generate the policy. There are two ways to generate the policy:

\paragraph{Model-based} For this method, we generate a model of $T[s,a,s']$ based on statistical analysis of the tuples. We look at a particular state and a particular action and see the probability of transitioning to another state. Same thing with $R[s,a]$. Then, we can use policy or value iteration to solve it.

\paragraph{Model-free} This method keeps the data around and uses the original tuples to determine what the new state will be for a certain action. This is Q-learning.

\section{Q-Learning}

\noindent Q-Learning is a model-free approach, which means that it doesn't need to have any sort of model of the transition function $T$ or the reward function $R$. It builds a table of \textit{utility values} as the agent interacts with the world. These are the Q values. At each state, the agent can then use the Q values to select the best action. Q-Learning is guaranteed to give an optimal policy, as it is proven to always converge.\\

\noindent Q represents the \textit{value} of taking action $a$ in state $s$. This value includes the immediate reward for taking action $a$, and the discounted (future) reward for all optimal future actions after having taken $a$. \\

\subsection{How do we use Q?}
\noindent What we want to find for a particular state is what policy, $\Pi(s)$ we should take. Using Q values, all we need to do is find the maximum Q value for that state.

\begin{equation}
\Pi(s) = {argmax}_{a}(Q[s,a])
\end{equation}

\noindent So, we go through each action $a$ and see which action has the maximum Q value for state $s$. Eventually, after learning enough, the agent will converge to the optimal policy, $\pi^*(s)$, and optimal Q table, $Q^*[s,a]$.

\subsection{How do we get Q?}
\noindent To use the Q table, first we must generate it by learning. How do we go about that? Well it's similar to previous learning algorithms, in that we provide it training data for which we know the outcomes. We then iterate over time and take actions based on the current policy ($Q$ values), and generate experience tuples $\langle s,a,s',r\rangle$ and generate the $Q$ values based on the experience.\par

\noindent In a more detailed fashion:

\begin{enumerate}
\item Initialize the $Q$ table with small random values
\item Compute $s$
\item Select $a$
\item Observe $r, s$
\item Update $Q$
\item Step forward in time, then repeat from step 2.
\end{enumerate}

\noindent To update $Q$, we first need a formula to decide what it should be. What we can do is assign a \textit{learning rate}, $\alpha$, to weight the new observations. We can therefore update $Q$ like this:

\begin{equation*}
Q'[s,a] = Q[s,a] + \alpha({improved\ estimate} - Q[s,a])
\end{equation*}

\noindent As you can see, $Q$ converges as the improved estimate is the same as the current estimate (we're at the best $Q$). Now, we need to know what the improved estimate is:

\begin{equation*}
improved\ estimate = immediate\ returns + (discounted\ future\ rewards)
\end{equation*}

\noindent Then, replacing \textit{discounted future rewards} with the actual way of calculating it, and rearranging to only use the current value of $Q$ once, we find that the formula to calculate the new value of Q for a state-action pair $\langle s,a\rangle$, the formula is:

\begin{equation}
Q'[s,a] = (1-\alpha)Q[s,a] + \alpha (r+\gamma\ Q[s',{argmax}_{a'}(Q[s',a'])])
\end{equation}

\noindent where:
\begin{itemize}
\item $r = R[s,a]$ is the \textit{immediate reward} for taking an action $a$ in the state $s$
\item $\gamma \in [0,1]$ is the \textit{discount factor} to reduce the value of future rewards
\item $s'$ is the resulting next state
\item ${argmax}_{a'}(Q[s',a'])$ is the action which maximizes the Q-value among all possible actions $a'$ from $s'$, and
\item $\alpha \in [0,1]$ is the \textit{learning rate} used to vary the weight given to new experiences compared to past Q-values. It's typically around 0.2.
\end{itemize}

\subsection{Exploration}
\noindent The success of a Q-learning algorithm depends on the exploration of the state-action space. If you only explore a small subset of it, you might not find the best policies. One way to ensure that you explore as much as possible is to introduce randomness into selecting actions during the learning phase. So basically, you see first whether you want to take the action with the maximal Q value or choose a random action, then if you take a random action, each action gets a probability which decreases over subsequent iterations.

\subsection{Q-Learning for Trading}
\noindent Now that we know what Q-learning is, we need to figure out how to apply it to the context of trading. That means that we need to define what \textit{state}, \textit{action}, and \textit{reward} mean. Actions are straightforward, as there are basically three of them:

\begin{itemize}
\item {\color{DarkerGreen} BUY}
\item {\color{red} SELL}
\item NOTHING
\end{itemize}

\noindent Our rewards can be daily returns or cumulative returns after a trade cycle (buy$\rightarrow$sell). However, using daily returns will allow the agent to converge on a $Q$ value more quickly, because if it waited until a sell, then it would have to look at all of the actions backwards until the buy to get that reward.\\

\noindent Now, we just need to figure out how to determine state. Some good factors to determine state are:

\begin{itemize}
\item Adjusted Close/Simple Moving Average
\item Bollinger Band value
\item P/E ratio
\item Holding stock (whether or not we're holding the stock)
\item Return since entry
\end{itemize}

\noindent Our state must be a single number so we can look it up in the table easily. To make it simpler, we'll confine the state to be an integer, which means we need to discretize each factor and then combine them into an overall state. Our state space is discrete, so the combined value is the overall state. Say we have a state like this:

\begin{table}[h]
\centering
\begin{tabular}{ccc}
\textbf{Factor} & \textbf{Value} & \textbf{Discretized}\\
$X_1$ & 25.6 & 0\\
$X_2$ & 0.3 & 5\\
$X_3$ & 2.0 & 9\\
$X_4$ & -5.1 & 2
\end{tabular}
\end{table}

\noindent The discretized state could be: 2950.

\paragraph{Discretization} To discretize, what we do is take the data for a factor over its range, then divide it into $n$ bins. Then we find the threshold by iterating over the data by the step size and taking the value at each position.

\begin{lstlisting}[style=python]
stepsize = size(data)/n
data.sort()
for i in range(0, steps):
	threshold[i] = data[(i+1)*stepsize]
\end{lstlisting}

\begin{figure}[h]
\centering
\includegraphics[width=6cm]{images/discretization.png}
\caption{What the thresholds might look like for a discretized data set if $n = 10$}
\end{figure}

\subsection{Problems with Q-Learning}
\noindent One main problem with Q-Learning is that it takes a lot of experience tuples to converge to the optimal Q value. This means the agent has to take many \textit{real} interactions with the world (execute trades) to learn. The way this has been addressed is by using \textit{Dyna}.

\section{Dyna-Q}

\noindent Dyna is designed to improve the convergence of Q learning by building a model of $T$ and $R$ and then using Q learning to make decisions based on the model. However, the Q learning portion is still model-free, so it's a mix of both.\\

\noindent So we do the Q-Learning steps, but after we take an action, we update the model of $T$ and $R$ with the new data, simulate a bunch of experiences based on the model, then update $Q$ based on these simulated experiences. To simulate the experiences, we basically generate random states and actions, and then find the new states/rewards based on the transition function and reward function.

\subsection{Learning $T$}

\noindent To figure out a model for T, what we can do is count the number of times that a transition to $s'$ by using the action $a$ in state $s$ occurred, then divide that by the total number of transitions to figure out the probability.

\begin{equation}
T[s,a,s'] = \frac{T_c[s,a,s']}{\sum_{i} T_c[s,a,i]}
\end{equation}

\noindent where $T_c$ is the number of times the transition occurred.

\subsection{Learning $R$}

\noindent To finalize the model, we need to find our expected reward, $R[s,a]$. Whenever we interact with the world, we get an immediate reward, $r$. We can use this to update our model for $R$ in a similar way to updating the Q values.

\begin{equation}
R'[s,a] = (1-\alpha)R[s,a] + \alpha r
\end{equation}

\noindent where $\alpha$ is, again, the learning rate.

\subsection{Conclusion}
\noindent So a summary of how Dyna-Q works is the following:

\begin{align*}
\noindent Q\ learning&\left\{
	\begin{tabular}{@{}l@{}}
    	init Q table\\
        observe S\\
        execute a, observe s;r\\
        update Q with $\langle s, a, s', r \rangle$\\
    \end{tabular}
\right.\\
\noindent Update\ model&\left\{
	\begin{tabular}{@{}l@{}}
    	update T'[s,a,s']\\
        update R'[s,a]
    \end{tabular}
\right.\\
\noindent Dyna\ Q&\left\{
	\begin{tabular}{@{}l@{}}
    	s = random\\
        a = random\\
        s' = infer from $T$\\
        r = R[s,a]\\
        update Q with new experience tuple\\
        repeat many times ($\sim100-200$)
    \end{tabular}
\right.
\end{align*}

\begin{figure}[h]
	\centering
	\includegraphics[width=7cm]{images/Dyna-architecture.png}
	\caption{A diagram of the Dyna architecture (courtesy Sutton and Barto)}
\end{figure}

==> annotatedReferences.tex <==
\chapter{Annotated References}

Here we briefly discuss some references on the crafting of reliable ML embedded solutions.  

In \cite{FRB2021} a general motivation for assurance of ML embedded systems is given.  

In \cite{DBLP:journals/corr/abs-2108-00941} a human in the loop in machine learning tutorial is given.  The impact of the economy of the organization is not discussed. 


==> dataframes.tex <==
\chapter{Python and Basic Interfaces}
\section{Dataframes}
\noindent A dataframe is a data structure in \textit{pandas} that allows multiple datasets to be mapped to the same indices. For example, a data frame that maps dates to closing prices could be:

\begin{center}
    \begin{tabular}{lcccc}
         & \textbf{SPY} & \textbf{AAPL} & \textbf{GOOG} & \textbf{GLD}\\
        2000-01-09 & 100.01 & 50.89 & NaN & NaN\\
        2000-01-10 & 100.05 & 50.91 & NaN & NaN\\
        \vdots & \vdots & \vdots & \vdots & \vdots \\
        2015-12-31 & 200.89 & 600.25 & 559.50 & 112.37
    \end{tabular}
\end{center}

\noindent The indices in this dataframe are the dates on the left, and the closing prices for that date are stored in each column. The "NaN"s appear because \textit{GOOG} and \textit{GLD} were not publicly traded during those periods. 

\subsection{Reading CSVs into Dataframes}
\noindent To begin using the dataframes, you need data first. Historical stock data from Yahoo is provided in the form of a CSV file, which can be easily read into a dataframe using \textit{pandas}'s function \textit{read\_csv()}.\\

\noindent\begin{minipage}{\linewidth}
\noindent\textit{example 1:}
\lstinputlisting[style=python]{code_examples/dataframes_1.py}
\end{minipage}

\noindent This example reads in a CSV corresponding to the historic data for \textit{AAPL} (Apple, Inc) into the variable \textit{df}. \textit{df} is a \textit{DataFrame} object, which means any \textit{DataFrame} methods may be used on it.\\


\noindent\begin{minipage}{\linewidth}
\noindent\textit{example 2:} An example of a method that can be used is \textit{max()}, which returns the maximum value in the range.\\
\lstinputlisting[style=python]{code_examples/dataframes_2.py}
\end{minipage}

\subsection{Plotting}
\noindent \textit{Matplotlib} can be used to plot the data in the dataframes, as pandas can conveniently tap into the \textit{matplotlib} API. Plotting data in a dataframe is as simple as calling \textit{plot()} on one of the series in the frame.\\

\noindent\begin{minipage}{\linewidth}
\noindent\textit{example 3:} Plotting the Adjusted Close\footnote{Adjusted Close is a historically-adjusted value of the stock that takes into account corporate actions (such as stock splits) and distributions (such as dividends issued).} price of \textit{AAPL}
\lstinputlisting[style=python]{code_examples/dataframes_3.py}
\end{minipage}

\begin{figure}
	\centering
	\includegraphics[width=\textwidth]{images/adj_close.png}
    \caption{Plot of adjusted close price for \textit{IBM} over all time. Notice that the indices are just numbers rather than dates and the plot goes backwards in time to the right}
\end{figure}

\noindent\begin{minipage}{\linewidth}

\noindent\textit{example 4:} Plotting multiple columns is as simple as adding a more entries to the selection statement

\lstinputlisting[style=python]{code_examples/dataframes_4.py}
\end{minipage}

\subsection{Issues}
\noindent There are some issues with the data that need to be solved to effectively use it in the way we want.

\paragraph{Trading days} The NYSE only trades for a certain number of days per year, which means that indexing by dates will return some results when the exchanges were not open. This poses problems for trying to pull out certain date ranges from the dataframe.

\paragraph{Multiple stocks} One of the dataframe's powers is to be able to contain multiple ranges, which means that we need to be able to retrieve multiple datasets and store them into the dataframe.

\paragraph{Date order} The data in the Yahoo CSV are in reverse chronological order (most recent at the top), so any analysis on the dataframe will be going backwards in time, which is not ideal.

\subsection{Solution to the issues}
\noindent To solve the trading days problem, we'll use an \ac{etf} called \textit{SPY} (S\&P 500) to serve as a basis for what days the stock market is open. The only days that exist in the dataset for this \ac{etf} are the days the stock market traded, so if we use this as a reference and use joining on the dataframes, we can recover data on only the days which had trading.\\

\noindent\begin{minipage}{\linewidth}
\noindent\textit{example 5:} Using joins to get only traded days

\lstinputlisting[style=python,firstline=1,lastline=7]{code_examples/dataframes_5.py}
\end{minipage}

\noindent If we were to print out df1, the output would be:
\begin{lstlisting}[style=python]
Empty DataFrame
Columns: []
Index: [2010-01-22 00:00:00, 2010-01-23 00:00:00, 2010-01-25 00:00:00, 2010-01-26 00:00:00]
\end{lstlisting}

\noindent This empty dataframe will be the basis for the data we want to retrieve.

\noindent The next step is to join this dataframe with a dataframe with the data for \textit{SPY}. This will keep only indices of the \textit{SPY} dataframe that also exist in the empty one.\\

\noindent\begin{minipage}{\linewidth}
\noindent\textit{example 6:} Reading in the new dataframe and joining them

\lstinputlisting[style=python,firstnumber=8,firstline=8,lastline=11]{code_examples/dataframes_5.py}
\end{minipage}

\noindent\begin{minipage}{\linewidth}
\noindent The output would now be:
\begin{lstlisting}[style=python]
				Adj Close
2010-01-22		104.34
2010-01-23		NaN
2010-01-24		NaN
2010-01-25		104.87
2010-01-26		104.43
\end{lstlisting}
\end{minipage}

\noindent To get rid of the "NaN"s, you can call \textit{dropna()} on the newly joined dataframe, but there is a better way of joining them such that the "NaN"s don't appear in the first place. The join type is called an \textit{inner} join, which joins at the intersection of the two dataframes. This way, only the dates which are in both will be kept as indices. Everything else will be thrown away.\\

\noindent\begin{minipage}{\linewidth}
\noindent\textit{example 7:} The inner join

\lstinputlisting[style=python,firstline=16,lastline=16]{code_examples/dataframes_5.py}
\end{minipage}

\subsection{Multiple stocks}
\noindent Reading in multiple stocks is as easy as just adding a for loop:\\

\noindent\begin{minipage}{\linewidth}
\noindent\textit{example 8:} Reading in multiple stocks into a single dataframe

\lstinputlisting[style=python,firstline=19,lastline=28]{code_examples/dataframes_5.py}
\end{minipage}

\noindent\begin{minipage}{\linewidth}
\noindent Here's an example of reading and plotting multiple stocks' closing price on one plot\\
\noindent\textit{example 9:} Reading and plotting multiple stocks

\lstinputlisting[style=python,firstline=31,lastline=77]{code_examples/dataframes_5.py}
\end{minipage}

\begin{figure}
	\centering
	\includegraphics[width=\textwidth]{images/adj_close_mar.png}
    \caption{Plot of adjusted close price for \textit{IBM} and \textit{spy} over the month of April 2010}
\end{figure}

\subsection{Normalizing}
\noindent Sometimes when plotting, the values of a stock will be significantly different from the other stocks such that it becomes difficult to tell some of them apart. Normalizing the data allows all of them to start at the same point and then show divergences from the initial point, making it easier to compare them at the same time.\\

\noindent Normalizing the dataframe is as simple as dividing the entire dataframe by its first row
\noindent\begin{minipage}{\linewidth}
\noindent\textit{example 10:} Normalizing a dataframe

\lstinputlisting[style=python,firstline=81,lastline=83]{code_examples/dataframes_5.py}
\end{minipage}

\begin{figure}[h]
	\centering
	\includegraphics[width=\textwidth]{images/adj_close_normalized.png}
    \caption{Normalized stock prices over the year 2010}
\end{figure}
\newpage

\section{NumPy}

\input{numpy}

==> drift.tex <==
\chapter{Drift Detection and ML Solution Retraining}
\label{Chapter:drift}

\newcommand{\nth}[1]{#1^{\text{th}}}

As previously mentioned, ML systems typically consist of input data and a target that is to be modeled or predicted on the basis of the input by an ML model. To the degree it is able, the ML model captures the relationship between the input and output target learned from training data.  The model will then be deployed (used to generate predictions) on another set of input data.  An underlying assumption of the exercise of building a model is that the input and target data in deployment will be similar to that in learning; if not, the model's predictions may not be trustworthy, and its performance (e.g., accuracy) will be unstable and different than on the training data.  What we call `drift' will be changes in the underlying data, whether or not they cause the model performance to change.  

This chapter is organized as follows.  We will first introduce basic notions of the types of drift and their effects on the model.  Then, we will discuss ways of detecting that drift has occurred, as well as some techniques to overcome these challenges.  Lastly, we will mention some statistical issues that arise in drift detection.  Since drift detection is a very wide topic, this is not exhaustive but will rather cover some basic concepts.

\section{Types of drift
\label{ssec:types_of_drift}}

Let $\mathbf{X}$ denote input data.  That is, $\mathbf{X}=\begin{bmatrix}\mathbf{X}_1,\mathbf{X}_2,\dots,\mathbf{X}_d\end{bmatrix}$, meaning each of its $d\geq 1$ columns\footnote{$\mathbf{X}$ is univariate if $d=1$ and multivariate if $d\geq 2$.} is a vector $\mathbf{X}_i$ of $n$ observations of a random variable or feature\footnote{See Appendix~\ref{ssec:random_variables}.} $X_i$.  Let $y$ be another feature that is the target random variable we wish to predict by an ML model based on $\mathbf{X}$.  $\mathbf{X}$ can denote input data of any kind, such as embeddings of natural language and or image instances, or structured tabular data; $y$ can denote a class or numeric-valued feature, in which case the ML model is a classifier or regressor. 

Letting $p(\cdot)$ denote an arbitrary probability distribution\footnote{See Appendix~\ref{ssec:random_variables}.}, let $p(y\mid\mathbf{X})$ denote the true, unobserved, probabilistic relationship\footnote{The notation `$a\mid b$' denotes $a$ conditioned on, or determined by $b$;  See Appendix~\ref{ssec:joint_distributions}}~between the value of the predictor features $\mathbf{X}$ and the target $y$; we aim to model $p$ by, say, some classifier model.  If a given dataset $D$ consists of $\mathbf{X}$ and $y$, the joint distribution of data observations in it can be denoted $p(y,\:\mathbf{X})$. This distribution can be decomposed\footnote{This follows from the laws of decomposing joint probability distributions into products of conditional distributions.  See Appendix~\ref{ssec:joint_distributions}}~as $p(y,\:\mathbf{X})=p(y\mid\mathbf{X})\times p(\mathbf{X})$, since the observations are assumed randomly sampled from an underlying population distribution $p(\mathbf{X})$.

Another dataset $D'$ consists of values $\mathbf{X}'$ and $y'$, from which its distribution $p'(\mathbf{X}',\:y')$ is estimated.  Note, if $\mathbf{X}=\mathbf{X}'$ but $y\ne y'$, then $p(\mathbf{X})=p'(\mathbf{X})$, that is, their feature distribution is the same (or at least we simply have observations on the same underlying samples), but the label distributions differ, i.e. $p(y\mid\mathbf{X})\ne p'(y\mid\mathbf{X})$.    

% need to clarify here that X and y are now arbitrary
Mathematically, drift between two observed datasets $D$ and $D'$, can be expressed as saying that $p(y,\:\mathbf{X})\ne p'(y,\:\mathbf{X})$, that is, their respective joint distributions  differ.
If we further decompose both as above, if there is drift, then either $p(y\mid\mathbf{X})\ne p'(y\mid\mathbf{X})\ne$, or $p(\mathbf{X})\ne p'(\mathbf{X})$, or both.  Figure~\ref{fig:boundary_drift} illustrates these for the case where $\mathbf{X}$ consists of two numeric features (the horizontal and vertical coordinates), displayed as a scatterplot of points; for each point $x\in \mathbf{X}$, its binary target class $y$ is indicated by point being either hollow or filled.  In this simple case, the classes $y$ are completely separable in that the curved line is able to completely separate the points by color (class value).  The line thus abstracts $p(y\mid \mathbf{X})$ in that, say, $p(y=\textrm{blue}\mid x)=1$ if $x$ is on one side of the curve and 0 if on the other.

\begin{figure}[h!]
\centering
\includegraphics[scale=0.5]{images/concept-vs-virtual-drift.png}
\caption{Examples of types of drift (Source: \cite{Iguazio_drift}).}
\label{fig:boundary_drift}
\end{figure}

In Figure~\ref{fig:boundary_drift}, the left image shows the baseline $p(y,\:\mathbf{X})$, with the other two showing different drifted $p'(y,\:\mathbf{X})$.  For illustration, imagine that the two features plotted are AGE (horizontal, say from age 16 to 65 years) and CREDIT RATING (vertical, where higher values indicate better credit), each point corresponds to an applicant for a student loan; the class $y$ is the bank's decision, indicated by the color of the point, with black being `reject' and green being `approve'.  Here we see that at younger ages, any credit rating will get you a loan (green), while as age increases, only the applicants with better credit will be approved, with the approval threshold increasing.

In the center image is what is typically called `\textbf{concept drift}', where the relationship $p(y\mid\mathbf{X})$, illustrated by the placement of the class decision boundary, has changed. In this case, it means that, say, a young applicant with a lower credit rating ($x$ in lower left corner) would now be rejected when he previously would be accepted, since this point would now fall `under' the decision boundary. In this image, $p(\mathbf{X})$ has changed relative to the left one, since the points are located in different places, but $p(\mathbf{X})$ could have also remained constant.  The right image shows an example of `\textbf{virtual drift}', where only the sampling distribution $p(\mathbf{X})$ (point placement) has changed to $p'(\mathbf{X})$.  The decision boundary, however, remains the same as in the left image, meaning that a given input $x\in\mathbf{X}$ would still have the same class, since $p(y\mid\mathbf{X})$ is constant. Drift has occurred in that $p'(y,\:\mathbf{X})\ne p(y,\:\mathbf{X})$, but only through changes in $p(\mathbf{X})$.

The intuition of distribution drift in Figure~\ref{fig:boundary_drift} can be extended to any input $\mathbf{X}$, whether higher-dimensional or non-numeric inputs like images, sound recordings, etc., however in these cases the distribution $p$ may be difficult to characterize mathematically, and high-dimensional points may be difficult to visualize.  Also, $y$ can be a numeric target, like income in dollars, rather than a class, or consist of multiple target values per observation (multi-output).

We note that there is disagreement among practitioners as to how to precisely define terms for various types of drift. \cite{MRACH12} represents one attempt to formulate coherent definitions.  The joint $p(y,\:\mathbf{X})$ can alternatively be decomposed as $p(y)\times p(\mathbf{X}\mid y)$, changing the order of conditioning from that above.  In \cite{ADFRZ2020}, for instance, $\mathbf{X}$ represents a classifier's measured confidence on an input image instance of class $y$, and only $\mathbf{X}$ and $y$ are observed, not the intermediate images, and drift in $p(y,\:\mathbf{X})$ is detected.  Here, the drift is induced by changing $p(y)$ (introducing a previously unseen class) rather than $p(\mathbf{X}\mid y)$ (characteristics of handwriting of each digit).

\section{Measuring distribution differences
\label{sec:measuring_distribution_differences}}

In Section~\ref{ssec:types_of_drift}, we introduced drift as
indicating $p(y,\:\mathbf{X})\ne p'(y,\:\mathbf{X})$ when $p(\cdot)$ and $p'(\cdot)$ are determined on two different datasets (or samples) $D$ and $D'$.  To determine if there is drift, we want to measure degree of difference or distance between the two sample distributions. Depending on the objective, a drift analysis may be conducted on one or more of the following:
\begin{itemize}
    \item $p(y)\textrm{ vs }p'(y)$, the class label distributions
    \item $p(\mathbf{X})\textrm{ vs }p'(\mathbf{X})$ or $p(\mathbf{X}\mid y)\textrm{ vs }p'(\mathbf{X}\mid y),\textrm{ for each }y$; that is, the overall or class ($y$)-conditional data distribution
\end{itemize}

Furthermore, we note that each dataset $D$ is actually treated as a random sample draw from some theoretical unobserved `population' dataset $\mathcal{D}$ (see \cite{LSHGOZ2003}, page 20) with associated distribution $P(\cdot)$ (as contrasted with $p$ or $p'$). For instance, in the example mentioned in Figure~\ref{fig:boundary_drift}, $D$ and $D'$ may represent samples (say, of sizes 1,000 each) of loan applicants in the USA in the months of January and July, 2021, respectively.  The respective populations $\mathcal{D}$ and $\mathcal{D}'$, with distributions $P$ and $P'$ respectively, are all such applicants in the USA in these two months; the samples were obtained because, perhaps, data on all such applicants (population) is not easily attainable.  The sample distributions are considered estimates (denoted $\hat{\phantom{}}\:$) of the respective population distribution; thus, we can say $p=\widehat{P}$ and $p'=\widehat{P'}$, meaning, for instance ``$p\textrm{ is an estimate of }P$".

Due to random sampling, if two sample distributions $p$ and $p'$ are drawn from the same population distribution $P$, we would not expect that $p=p'$ exactly.  Instead, if we try to decide if drift were occurred, we want to avoid considering small differences that may be due to random sampling as `drift'.  Rather, we typically try to make inferences such as the following: given $p=\hat{P}$ and $p'=\hat{P}'$, how likely is it that $P\ne P'$?  That is, the drift question often tries to infer whether the two observed samples $p$ and $p'$ are different enough (more than by random chance) to indicate that the unobserved $P$ and $P'$ themselves are different.  If they are, this is considered `drift'.  This is the nature of statistical hypothesis testing (see \cite{LSHGOZ2003}, page 375).

Such statistical drift tests can be conducted if the distribution can be characterized mathematically.  Typically, such tests are called `two-sample tests' since they compare two random samples for equality, rather than, say, evaluating one sample to a fixed baseline value or distribution.  However, sometimes a mathematical representation of the distribution cannot be constructed, and thus a measure of distance between the two samples $D$ and $D'$ may be measured instead; \cite{SamBlog} (Q4) reviews some examples.  Here, we will just cite these measures without detailed elaboration.

\begin{exercise}
Assume that $\mathbf{X} = \{ x \in R^3 | x_i \ge 0, x_1+x_2+x_3 = 1 \} $ and that $y = \{-1, 1\}$.  Assume that the model m is accurate iff $x_2 \leq \frac{1}{2}$.  The model was trained with p being uniformly distributed on $\mathbf{X}$. What is the accuracy of the model on p?  Next, the distribution on $\mathbf{X}$ is shifted to be uniformly distributed on $\{x \in \mathbf{X} | x_2 \ge \frac{1}{2}\} \bigcup \{x \in \mathbf{X} | x_3 \ge \frac{1}{2}\}$.  What is the accuracy of the model on the new distribution?  What type of drift occurred in this case?  Suggest a change to the problem conditions so that the other type of drift will occur.  
\end{exercise}

% https://tex.stackexchange.com/questions/53513/hyperref-token-not-allowed
\subsection{Two-sample distribution difference measures on \texorpdfstring{$\mathbf{X}$}{X}}
\label{ssec:two_sample_continuous}

\subsubsection{Univariate tests}
\label{sssec:two_sample_continuous_univariate}

For univariate samples (inputs $\mathbf{X}$ and $\mathbf{X}'$, from which $p$ and $p'$ are estimated, consist of a single feature), many tests exist; for those we describe in the following, we also list the test function name as it can be found in the relevant Python package, such as \texttt{scipy} (\cite{2020SciPy-NMeth}).\footnote{The cited test names are accurate as of \texttt{scipy} version 1.8.0.}  

Given two samples $D$ and $D'$, sometimes one is interested to know if they have, say, the same (arithmetic) mean, median, or variance\footnote{The arithmetic mean (average) and median ($\nth{50}$ quantile) are measures of central tendency; see \cite{LSHGOZ2003}, pages 131--133.  The variance is a commonly-used measure of variability; see \cite{LSHGOZ2003}, page 144--151.}, rather than whether the whole distributions $P=P'$. In some cases, $P\ne P'$ while their means, medians, or variances can be unchanged.  However, a change in mean, median, or variance indicates the distributions differ as well, particularly in the aspect that is important to the user.  For instance, a teacher may want to know if the mean scores on a math test increased, regardless of whether the distribution changed (e.g., more students received very low or very high scores).

In these cases, the two-sample Student T-test (\texttt{scipy.stats.ttest\_ind}) is often used to detect differences in the mean; Bartlett's test (\texttt{scipy.stats.barlett}) or Levene's test (\texttt{scipy.stats.levene}, if the samples don't appear normally-distributed\footnote{Various tools can be used to assess whether a sample appears normally-distributed.A quantile-quantile (QQ) plot (e.g., \cite{LSHGOZ2003}, page 280) can visualize these differences.  There are also statistical tests to assess similarity to a normal distribution, such as the Shapiro-Wilk (\texttt{scipy.stats.shapiro}), D'Agostino-Pearson (\texttt{scipy.stats.normaltest}), and Anderson-Darling (\texttt{scipy.stats.anderson}).}) can detect differences in variance.  The Kruskal-Wallis (KW, \texttt{scipy.stats.kruskal}) tests can be used to test for equality of medians.  If the data $\mathbf{X}$ are binary-valued ($X$ can be coded as $\in\{0,1\}$), the means are proportions restricted to $[0,1]$; in these cases, Yates' difference-in-proportions test (\cite{Y1934}) can be used. 

\begin{exercise}
\label{excercise:622}
As an example for when summary of the data such as the sample average and sample variance are of interest consider the following situation.
\begin{enumerate}
\item 
Assume that a feature $X \in R$ in the data D is normally distributed with average 0 and standard deviation (i.e., the square root of the variance) $\epsilon > 0$.  $\epsilon$ is assumed to be very small.  What is your expectation of the impact of X on the dependent variable y? 
\item  Assume that X, T, and Z are independent variables.  Also assume that the relation we are trying to learn is $X+T+Z = y$.  Write a program that generates X, T, and Z independently each from a normal distribution.  Have the average of X, T and Z be 0.  In addition, the standard deviation of X is some small $\epsilon > 0$ while the standard deviation of T is 100 and the standard deviation of Z is 1000.  Generate n samples $(x_i, t_i, z_i)$.  For each generated triple $(x_i, t_i, z_i)$ calculate $x_i+y_i+z_i = y_i$.  Also calculate the sample average of $x = \frac{1}{n} \sum x_i$. calculate $x + y_i + z_i = y^{'}_i$.   What is the maximal difference between $y_i$ and 
$y^{'}_i$?  what does it tell you about the learning of y?  
\end{enumerate}

\href{https://colab.research.google.com/drive/1h6sHrpPEhcwglv_majEZ_1ousbYGnSXC?usp=sharing}{Click here for a simulation} or see appendix \ref{chapter:solution_appendix} in solution \ref{excercise:622_sol}

\end{exercise}

\begin{exercise}
Consider the Dirichlet distribution.  It is an important distribution used in Bayesian analysis but for the purpose of this exercise all we need to know about the distribution is that it is determined by $a_1, \ldots, a_k$ parameters, $a_i > 0$.  Whenever we sample a point from the distribution we will get a point $x = (x_1, \ldots, x_k)$ in the simplex, i.e., $x_i \ge 0$ and $\sum x_i = 1$.  The average value of the i$'$th coordinate is $\frac{a_i}{\sum a_i}$ while the variance for the $\nth{i}$ coordinate is $\frac{(\frac{a_i}{a})(1-(\frac{a_i}{a}))}{a+1}$ where $a = \sum a_i$. Given the average and the variance can you determine the parameters $a_i$ of the distribution?
\end{exercise}

\begin{exercise}
Give an example for two different distributions that have the same average and variance.  (Hint - pick up a uniform distribution with some average and variance and match it with a normal distribution that has the same average and variance. )
\end{exercise}

If one wants to determine the likelihood of $P=P'$, and not just equality of summary statistics, often nonparametric tests are used; these tests make minimal or no assumptions about the shape of the distributions.  Some common ones for continuous data are Kolmogorov-Smirnov (KS, \texttt{scipy.stats.ks\_2samp}),
Cram\'er-von Mises (CvM,\\ \texttt{scipy.stats.cramervonmises\_2samp}), or Anderson-Darling (AD,\\ \texttt{scipy.stats.anderson\_ksamp}); the AD test can test simultaneous distributional equality of $k>2$ samples, not just two.  If testing equality of the distributions of orderings of values (rather than the distributions over the values themselves), the Mann-Whitney U rank test (MW, \texttt{scipy.stats.mannwhitneyu}) is often used.  Say, for instance, each of $D$ and $D'$ is associated with a separate team, and the values are the times in minutes that each racer on the team finishes a race; assume that the winners are determined only by the relative order they finish and not by the absolute times.  In this case, the MW test indicates if the racers in the two teams are approximately evenly-matched in terms of the order (but not necessarily the measured times). 

The tests mentioned so far, like many others, rely on p-values, or significance levels (see \cite{LSHGOZ2003}, page 375) to make a decision.  The null hypothesis ($H_0$) in each case is specified as equality of either the distributions $P$ and $P'$ or the statistic of interest; a low p-value, below a pre-specified $\alpha\in(0,1)$, indicates that drift is likely because the distributions differ significantly, and thus the null $H_0$ should be rejected.  Because the statistical significance measured by p-values is known to have methodological issues, measures of \textbf{effect size} (\cite{LSHGOZ2003}, page 692; \cite{SF2012}), which more closely capture the magnitude of \textit{practical} difference between the two samples' summary statistics.  Some commonly-used measures are Cohen's $d$ and $h$ measures\footnote{For two 
independent numeric samples $\mathbf{x}_1$ and $\mathbf{x}_2$, Cohen's $d$ is defined as $\frac{\bar{\mathbf{x}}_1 - \bar{\mathbf{x}}_2}{\sqrt{(s_1^2+s_2^2)/2}}$, where $\bar{\mathbf{x}}_i$ and $s_i$ are the sample mean and standard deviation of $\mathbf{x}_i$.  If the two samples are binary $0-1$ valued, the sample proportions are $\pi_i=\bar{\mathbf{x}}_i$; in this case, Cohen's $h=\textrm{arcsin}(\sqrt{\pi_1}) -\textrm{arcsin}(\sqrt{\pi_2})$.  See also \cite{NCSSPASS} documentation on `Two-Sample T-Tests using Effect Size' and `Tests for Two Proportions using Effect Size' for a clear and thorough discussion.} (\cite{C1988}) for testing two-sample differences in means and single binary proportions.  These measures are compared to specified thresholds rather than an $\alpha$ value, to make a significance decision.  For instance, for both the $d$ and $h$ measures, values of 0.2, 0.5, and 0.8 represent small, medium, and large differences, respectively (\cite{C1988}, pages 40, 198).    

The local kernel-density-difference test from \cite{D2013} (implemented in \texttt{RJournal of Modern Applied Statistical Methods} as the \texttt{ks} package, \cite{DWCG2018}) identifies regions where the two densities $p$ and $p'$ differ significantly, as opposed to simply \textit{if} they differ. An illustration on univariate data, with Python implementation, is shown in \cite{SamBlog} (Q9).

Two other distribution distances that are commonly used are Kullback-Leibler divergence %(\texttt{scipy.stats.rel_entr})


\subsubsection{Multivariate tests}
\label{sssec:two_sample_continuous_multivariate}\footnote{Eitan - how do we handle drift of many features?}\footnote{Eitan - Is the difficulty caused by many variables is related to the curse of high dimension?}\footnote{Eitan - are we recommending non parametric always regardless if one or more variables and why?}
Here we consider multivariate samples, where the inputs $\mathbf{X}$ and $\mathbf{X}'$ consist of $d>1$ features.  If their distributions $p(\mathbf{X})$ and $p'(\mathbf{X}')$ can be assumed to be multivariate Gaussian, Hotelling's $T^2$ test (\cite{H1931}; implemented in Python as \texttt{hotelling.stats.hotelling\_t2}, \cite{D2021}), which is the multivariate extension of the two-sample Student T-test for differences in means (see Section~\ref{sssec:two_sample_continuous_univariate}), is often used.  

Otherwise, multivariate distributions are often hard to characterize in a nonparametric way.  One commonly-used nonparametric two-sample distance metric is Wasserstein (also known as ``Earth-mover's") distance; it measures the distance between two distributions using transport theory, representing each observation as, say, a grain of sand that must be `moved' from $p$ to $p'$.  The more `distance' each `grain' must be moved to transform $p$ into $p'$, the greater the distance between them.  These metrics are implemented in Python as \texttt{scipy.stats.wasserstein\_distance} (univariate case) and \texttt{ot.emd} (multivariate).  Another nonparametric kernel-based distance is Maximum Mean Discrepancy (MMD, \cite{GBRSS2012}); this is illustrated in \cite{SamBlog} (Q4).

There are also several two-sample nonparametric multivariate difference-in-distribution tests; these tests generally involve calculating pairwise distances between members of the samples $\mathbf{X}$ and $\mathbf{X}'$, and internally between members of each of the samples.  A few examples include the MMD test mentioned above (\cite{GBRSS2012}), the energy distance test (\cite{SR2013}), Henze's test on nearest-neighbor type coincidences (\cite{H1988}), and a test by Biswas and Ghosh (\cite{BG2014}).  The first two tests are implemented in the Python package \texttt{torch-two-sample} (\cite{torch_two_sample}).  

If distribution drift is detected (by performing one of the goodness-of-fit tests above) between these multivariate samples, one may also want to detect which features are most responsible for the measured drift.  One such technique is called Local Depth-Based Isolation Forest Feature Importance (DIFFI, \cite{CTS2020}).  DIFFI is based on Isolation Forests (IF, \cite{LTZ2008}; implemented as \texttt{sklearn.ensemble.IsolationForest}), which is a nonparametric ensemble tree-based method of scoring how much of an outlier a multivariate observation (e.g., one row of $\mathbf{X}'$) is relative to a baseline dataset (e.g., $\mathbf{X}$).  An observation is more of an outlier if a tree, splitting at random locations on the feature domains, can isolate it in fewer tree splits.  This technique is used by DIFFI to score the anomalousness of each feature value in the observation by where it occurs in the tree decision paths.  As illustrated in \cite{SamBlog} (Q11), since IF is nonparametric, it can identify outliers whose feature values lie in low-density not necessarily on the tails of the domain range, as opposed to, say, Mahalanobis distance outlier scoring, which assumes outliers will be at the tails of the range.  Features with higher local feature importance (LFI) scores are most responsible for the observation being an outlier.  If one averages the LFIs for observations in $\mathbf{X}'$ that the IF determines to be outliers, or sums the frequencies at which each feature is the most anomalous, one can determine which features overall are most responsible for the drift.



\subsection{Two-sample (categorical) distribution difference measures on \texorpdfstring{$y$}{y}}
\label{ssec:two_sample_class}

In addition to the tests mentioned in Section~\ref{ssec:two_sample_continuous} on numeric-valued input data $X$, we can also test whether the distributions of observed labels $\mathbf{y}$ differ.  Again, this determination is often made by assuming unobserved population distributions $P$ and $P'$.  Because the values $\mathbf{y}$ are nominal-valued (categorical), such as the state (e.g., Alabama, Alaska,\dots,Wyoming) of residence of the loan applicant, $P$ typically takes the form of a multinomial distribution (\cite{LSHGOZ2003}, page 208).  The multinomial distribution $\mathcal{M}$ is denoted $\mathcal{M}(\boldsymbol{\pi},\:N)$, where $N\in\{1,2,\dots\}$ is a positive integer representing the sample size (number of observations), and $\boldsymbol{\pi}=\begin{bmatrix}\pi_1 & \dots & \pi_k\end{bmatrix}$ is a $k$-length vector where $0\leq \pi_i\leq 1,\:\forall\:i=1,\dots,k$, and $\sum_{i=1}^k\pi_i=1$.  Without lack of generality, let the $k$ potential label values be $\boldsymbol{\ell}=\{\ell_1,\dots,\ell_k\}$.  $\mathcal{M}(\boldsymbol{\pi},\:N)$ models $N$ label values, drawn independently, where each draw takes the $\nth{i}$ label $\ell_i$ with probability $\pi_i$.  Since all that is modeled is the total count of each label out of $N$ draws, and not the order, a vector $\mathbf{x}=\begin{bmatrix}x_1,\dots,x_k\end{bmatrix}$ can be modeled as a draw from $\mathcal{M}(\boldsymbol{\pi},\:N)$, if each $x_i$ is a non-negative integer and $\sum_{i=1}^kx_i=N$.  That is, $x_i$ is the observed occurrence, out if $N$, of label $\ell_i$.  Therefore, given two observed label vectors $y$ and $y'$, where the corresponding counts vectors are $\mathbf{x}$ and $\mathbf{x}'$ (assuming both have the same size $N$), we can determine if they appear to come from the same multinomial distribution $P$.

Probably the most-used test for equality of categorical counts is the 
one-way chi-square goodness-of-fit (\texttt{scipy.stats.chisquare}), not to be confused with the chi-square test for independence of two variables (\texttt{scipy.stats.chi2\_contingency}) performed on a contingency table.  This test requires the sums of $\mathbf{x}$ and $\mathbf{x}'$ to equal ($N$ is the same).  However, it is a one-way test, since one of $\mathbf{x}$ or $\mathbf{x}'$ must be set as the `expected' and the other as the `observed' values, which affects the calculation; in contrast, in the two-way tests, there is no `baseline', and the order of specification of samples does not matter.  This test returns a p-value used in the drift decision.  The test statistic is $\chi=\sqrt{\sum_{i=1}^k \frac{(x_i'-x_i)^2}{x_i}}$, where $x_i$ are the expected counts.

An alternative is to use the effect size metric Cohen's $w=\sqrt{\sum_{i=1}^k \frac{(\hat{\pi}'_i - \hat{\pi}_i)^2}{\pi_i}}$ (\cite{C1988}), where $\hat{\pi}_i=\frac{x_i}{\sum_j x_j}$ and $\hat{\pi}'_i=\frac{x'_i}{\sum_j x'_j}$ are the corresponding proportions in the `expected' ($\mathbf{x}$) and `observed' ($\mathbf{x}'$) samples, respectively. Cohen's $w$ is very similar to the chi-square statistic  except that it operates on the proportions rather than the frequencies, and thus the samples sizes do not have to be equal since the sums of the proportions each equal 1.  The rule-of-thumb thresholds for $w$ are 0.01, 0.2, 0.5, 0.8, 1.2, and 2.0 for very small, small, medium, large, very large, and huge effect sizes (\cite{C1988}, page 227; \cite{S2009}).

The chi-square and Cohen's $w$ metrics are asymmetric tests in that one set of values is set as the `expected' ones. Note also that $w$ is undefined if any $x_i=0$, which makes it unusable if a category level in the observed $\mathbf{x}'$ does not occur in the expected $\mathbf{x}$.  Several alternative metrics exist.  The dissimilarity index (\cite{G1914}) is defined as $\hat{\Delta}=0.5\sum_{i=1}^k|\hat{\pi}_i - \hat{\pi}'_i|$, and a rule of thumb is that $\hat{\Delta}<0.03$ indicates the two distributions are very close (\cite{A2002}, page 329). Hellinger's distance is defined as $H=\sqrt{1-B}$, where $B=\sum_{i=1}^k\sqrt{\hat{\pi}_i\hat{\pi}'_i}$ is the Bhattacharyya coefficient (\cite{B1946}).  It has the property that $0\leq H\leq 1$, with $H=0$ indicating distributional equality; in addition, it obeys the triangle inequality.  Both $\hat{\Delta}$ and $H$ are symmetric.  Note that $\hat{\Delta}$ will reflect labels where, say, $\hat{\pi}'_i\ne 0$ but $\hat{\pi}'_0=0$ (label $i$ occurs in the observed but not expected distribution), but $H$ will not, since the two probabilities are multiplied.

Another metric is Jensen-Shannon distance (\cite{ES2003}), which is the square root of the Jensen-Shannon divergence.  This distance is implemented as \texttt{jensenshannon} in \texttt{scipy.spatial.distance} (\cite{2020SciPy-NMeth}).  It is also symmetric and obeys the triangle inequality.  Given the two probability vectors $\hat{\boldsymbol{\pi}}$ and $\hat{\boldsymbol{\pi}}'$, let $\boldsymbol{m}=\begin{bmatrix}m_i & \dots & m_k\end{bmatrix}$ be their element-wise mean ($m_i=(\hat{\pi}_i+\hat{\pi}_i')/2$) for each discrete level $i$.  The distance is defined as 
$JSD(\hat{\boldsymbol{\pi}}, \hat{\boldsymbol{\pi}}')=\displaystyle{\sqrt{\frac{D(\hat{\boldsymbol{\pi}}\parallel\boldsymbol{m}) + D(\hat{\boldsymbol{\pi}}'\parallel\boldsymbol{m})}{2}}}$, where $D$ is the Kullback-Leibler (KL) divergence.  This distance has the property that $JSD\in [0, \log_b{(2)}]$, where $b$ is the logarithm base used in $D$; the maximum bound is 1 if $b=2$ and $\ln{(2)}$ for natural logarithms.  KL divergence for probability vectors $\boldsymbol{\pi}$ and $\boldsymbol{\pi}'$, which is not symmetric, is defined as $D_{\textrm{KL}}(\boldsymbol{\pi}\parallel \boldsymbol{\pi}')=\sum_i \boldsymbol{\pi}_i\ln{\left(\frac{\boldsymbol{\pi}_i}{\boldsymbol{\pi}'_i}\right)}$.  The summation is done for level indices $i$ for which both vectors are non-zero; thus, $\boldsymbol{m}>0$ whenever at least one is non-zero, so the equation above is defined.  If the logarithm base is $b=2$, the divergence measure (before taking the square root) can also be written as $H(\boldsymbol{m})-\frac{1}{2}(H(\hat{\boldsymbol{\pi}})+H(\hat{\boldsymbol{\pi}}'))$, where $H$ is the distribution's entropy.

If we let $J(i\mid \boldsymbol{\pi},\boldsymbol{\pi}')=\boldsymbol{\pi}_i\ln{\left(\frac{\boldsymbol{\pi}_i}{m_i}\right)} + \boldsymbol{\pi}'_i\ln{\left(\frac{\boldsymbol{\pi}'_i}{m_i}\right)}$, then the JS distance above can be written as $JSD(\hat{\boldsymbol{\pi}}, \hat{\boldsymbol{\pi}}') = \sqrt{0.5\sum_{i=1}^K J(i\mid\hat{\boldsymbol{\pi}},\hat{\boldsymbol{\pi}}')}$.  Thus, the value $i$ for which $J(i\mid\hat{\boldsymbol{\pi}},\hat{\boldsymbol{\pi}}')$ is maximum is the level which differs the most between the two distributions.  This can allow us to score (using $J(i)$) the contribution of levels $i$ to the divergence calculation, and thus to assign relative responsibility for the observed drift.

We note that JSD, like the KL divergence on which it is based, can also be used on continuous samples $\mathbf{x}$ and $\mathbf{x}'$.  
However, in this case, a fine discretization of the domain shared by both (i.e., from $\textrm{min}(\textrm{min}(\mathbf{x}),\textrm{min}(\mathbf{x}'))$ to $\textrm{max}(\textrm{max}(\mathbf{x}),\textrm{max}(\mathbf{x}'))$) to a set of (typically equally-spaced) 
points $\{v_i\}$. Then, we need to obtain $\hat{f}$ and $\hat{f'}$, kernel density estimates of the samples $\mathbf{x}$ and $\mathbf{x}'$. 
Let $b_i$ be the estimated bin width at $v_i$ (in the equally-spaced case, all $b_i$ equal some constant $b$).  
Because the JSD requires probability vector inputs, then $\pi_i=\hat{f}(v_i)b_i$ 
and $\pi_i'=\hat{f'}(v_i)b_i$. 
Using JSD on continuous values thus requires the intermediate step of a kernel density estimate.


\section{Drift in characterizations of data
\label{sec:drift_in_characterizations}}

In Section~\ref{sec:measuring_distribution_differences}, we presented a series of two-sample statistical tests, distance, and effect-size measures to detect distributional drift between two datasets $D$ and $D'$.  There, we assumed we could, or desired to, model the dataset or label distributions directly.  However, sometimes it is desired to model intermediate `aspects' of the data, or a model's performance on it, and detect drift on these aspects instead.  We present several examples here.

\subsection{Drift in data slices \label{ssec:drift_in_data_slices}}

Letting $D$ and $D'$ be tabular structured datasets of numeric or categorical features.  \cite{ARZ20} introduces the notion of a data `slice' rule as a conjunction of subsets of a group of feature; a subset on a feature is an interval with a minimum and maximum value if the feature is numeric, or a set of potential values if it's nominal.  For instance, an example of a slice $S$ is $\{\$30,000\:\leq\:\textrm{INCOME}\:\leq\:\$60,000\}\:\&\:\{\textrm{STATE}\in\{\textrm{New York},\textrm{Ohio},\textrm{Michigan}\}\:\&\:\{\textrm{SEX}\in\{\textrm{Male}\}\}$, which is defined on the three features INCOME, STATE, and SEX.  An observation falls in a slice if its feature values satisfy all conditions in the slice; for instance, any males with an income in the range \$30,000--\$60,000 and living in either New York, Ohio, or Michigan.  The size, or support of a slice on a dataset of $N$ total observations is the number of observations falling in the slice; the fractional support is the support divided by $N$.  Given a classifier model that returns predictions on $D$, \cite{ARZ20} present an algorithm to find a set of such slices where specifically the classification error rate of the model is higher than the average over $D$; such slices are called `error-based slices'.

Given two similar datasets $D$ and $D'$ and the classifier's predictions on each, \cite{ADFRZ2021} presents a method for detecting drift between $D$ and $D'$.  The drift is not detected directly on the datasets' feature distributions $p(\mathbf{X},\:y)$ and $p'(\mathbf{X},\:y)$, but rather by extracting a set of error-based slice rules on $D$, and detecting differences between this set and the rules when mapped to $D'$.  Note that the $K$ slices can overlap in that an observation can fall into more than one of them.  If $K$ slice rules are extracted, $\hat{\pi}_{1,i}$ and $\hat{\pi}_{2,i}$ be the observed fractional support of the $\nth{i}$ slice out of $K$ on datasets $D$ and $D'$, respectively.  If there is no drift between $D$ and $D'$, we expect $\hat{\pi}_{1,i}\approx\hat{\pi}_{2,i}$; the same is true of all $K$ slices.  A difference-in-proportions test (\cite{Y1934}, mentioned above in Section~\ref{sssec:two_sample_continuous_univariate}) can be used to test this; since $K$ hypotheses, one for each slice, are conducted, we have $K$ p-values $p_1,\dots,p_K$.  

Ultimately, we want a single decision of drift over all the slice p-values, and not just to see if each slice individually has drifted (changed in size).  This is done by using an adjustment for multiple comparisons (see \cite{LSHGOZ2003} page 424), specifically Holm's method (\cite{H1979}), which produces a single p-value with a statistical guarantee on the familywise error rate (FWER) of the decision (i.e., across the `family' of multiple hypotheses).    

In this example, \cite{ADFRZ2021} used an `indirect' drift test based on the set of slices, which has several advantages. First, it allows repurposing an existing technology for slice-extraction (\cite{ARZ20}) for drift detection; this method can be used in other settings where `useful' observation subsets can be defined.  Second, since the purpose of the slices was to locate concentrations of model errors by the feature values, the technique allows detection of drift specifically in these areas, which are particularly useful because they indicate likely changes in model accuracy, assuming stability of the slice rules, and not just drift in the feature distributions.  Thirdly, and most importantly, distilling the dataset into the simpler aspect of slice rules, which are now modeled by the univariate measure of proportion, simplifies the analysis from the multivariate case of actually modeling all the feature distributions.

\subsection{Drift in density-based slices}

For the dataset $D$, let its feature space $\mathcal{S}$ denote the mutual intersection of the observed domains of each feature (i.e., the minimum to maximum value observed for numeric features, or the set of unique levels for categorical features). \cite{AFRZZ2021} present a way to partition the space $\mathcal{S}$ into a set of slices, which are defined in the same way as in \cite{ARZ20}. However, here the $K$ slices extracted differ from \cite{ARZ20} in two ways.  First, they form a partition, in that together they contain all observations in $D$ and that each observation belongs to exactly one of them (as opposed to \cite{ARZ20}, where there may be overlaps and observations that do not fall in any of the slices).  Second, these slices are constructed to contain observations with similar `spatial' density within the feature space, rather than classification error; furthermore, some slices may define feature subsets that are empty, containing no observations on the input dataset $D$.  

As discussed in Section~\ref{ssec:drift_in_data_slices}, this method distills the feature space of $D$, which may be high-dimensional, into the lower-dimensional abstraction of useful slice rules.  Furthermore, as in \cite{AFRZZ2021}, though not discussed there, these slices can be used for drift detection in a similar way by testing differences in univariate measures, such as their fractional support or volume.  

For instance, say the $K$ density-based slices $\{S_i\}$ on $D$ can be categorized as either `not very sparse' (type 1), `very sparse' (type 2), or `empty' (type 3); the sparsity threshold can be decided based on, say, the average core distance, or slice volume divided by fractional support (see \cite{AFRZZ2021} for details).  Let us further define each slice $S_i=S_i\bigcap\mathcal{S}$, meaning an observation $x_i$ falls in the slice if it satisfies the feature constraints defined in the slice, but also that $x_i\in\mathcal{S}$; that is, $x_i$ must satisfy the feature constraints $\mathcal{S}$ for all features, even those not used in the slice definition.  On $D$ itself, this additional requirement is automatically true.

In $D$, observations must fall only into either slices of type 1 or 2, since those of type 3 are by definition empty.  Now, let each observation in another dataset $D'$ be mapped to one of the $K$ slices.  Then, each observation in $D'$ can fall into one of either types 1, 2, or 3 (which can now be non-empty).  In addition, observations $x_i\in D'$ for which $x_i \notin \mathcal{S}$ can belong to one of
\begin{itemize}
    \item type 4: $x_i$ would fall in a slice $S_i$ if $S_i$ were not further restricted to its intersection with $\mathcal{S}$.  This happens if the feature values that cause $x_i\notin \mathcal{S}$ (e.g., an income higher than that observed for any record in $D$, or a category level previously unobserved in $D$) are not used in any slice's definition.
    \item type 5: at least one of the features that cause $x_i$ to be $\notin \mathcal{S}$ has a slice explicitly defined on it, and hence $x_i$ would not satisfy any slice even without the additional restriction to $\mathcal{S}$.
\end{itemize}

Similarly to in \cite{ADFRZ2021} (Section~\ref{ssec:drift_in_data_slices}), if there is no drift in feature distributions between $D$ and $D'$, we may expect each type 1--5 to have similar fractional support on the two datasets (and close or equal to 0 for types 3--5 for $D'$).  Significant drift in these proportions---after an adjustment for multiple hypotheses, or by the distance metrics in Section~\ref{ssec:two_sample_class}---may indicate drift.  Furthermore, this drift is easily explainable, in that we can point to which of type 1--5 changed the most, and identify some of the anomalous observations.  For instance, letting $\hat{\boldsymbol{\pi}}$ and $\hat{\boldsymbol{\pi}}'$ be the observed proportions of observations belonging to types 1--5 in each of datasets $D$ and $D'$, we can use the element-wise terms $J(i\mid\hat{\boldsymbol{\pi}},\hat{\boldsymbol{\pi}}')$ of the Jensen-Shannon distance (see Section~\ref{ssec:two_sample_class}) to identify the most responsible slice type.

\subsection{Drift in feature polynomial relations}

Given a tabular dataset $D$ of only numeric features, \cite{RARF2021} present a method to extract strong polynomial relations from it.  Say that the input data $\mathbf{X}$ contains $m$ features, denoted $X_1,\dots,X_m$.  A polynomial relation is an polynomial `equation' between, say, $X_1$ and some $k$ (e.g., 2) of the features, allowing feature interactions up to a limited degree $\ell$ (say, 2).  For example, $X_1\approx2 + 3X_2 - 5X_2X_3 + 1.5X_2^2$; let us denote this relation $\mathcal{L}_1$. The relation between $X_1$ and the expression involving $X_2$ and $X_3$ is found using linear regression; hence the $\approx$ symbol means that this is not a strict equality, but that there is some error, which is measured by the error term of the linear regression equation.  Strong relations are polynomials where the regression coefficient of determination $R^2$ is high, indicating a strong linear correlation between the true value (e.g., $X_1$) and the `prediction' of the polynomial on the other features $X_2$ and $X_3$.

Given a polynomial $\mathcal{L}_1$ determined on $D$, we can see how good its fit is on the same features in another dataset $D'$; in the absence of drift, we expect the fit to be about the same.  The degree of change in fit is quantified by the Bayes Factor of $\mathcal{L}_1$ on $D$ vs $D'$.  In experiments with simulated drift insertion in \cite{RARF2021}, it is shown that for relations that had high initial $R^2$ (strong), the Bayes Factor was more responsive to drift insertion than weaker relations; that is, the strong relations were better indirect sensors of feature drift.  Since many relations can be extracted from $D$, a correction should be done to adjust for the multiple comparisons performed.

As in the previous examples discussed above, drift analysis based on the relations, rather than $\mathbf{X}$ itself, can be simpler.  \cite{RARF2021} suggest constraining the relations by $k=\ell=2$, to prevent over-fitting and so they are relatively human-interpretable.  The logic of drift detection here is that a strong relation is likely a fixed aspect of the data that should be stable; for instance, we may expect a person's SALARY to have a fixed polynomial relationship to their years of EXPERIENCE and EDUCATION, and if this changes, it may indicate an underlying feature drift.  In particular, if an ML model is to be be deployed on $D'$, its performance may differ significantly from that on $D$ if there is drift, if the model exploits existing feature correlations for its predictions.  Even if the intermediate relations themselves are not of interest, they can still be used as `detectors' of drift.

\section{Sequential drift detection}

So far, the statistical tests and examples of indirect drift detection (Section~\ref{sec:drift_in_characterizations}) dealt with a single decision on $D$ vs $D'$.  In many cases, however, we may observe an ordered sequence of datasets $D_1,D_2,\dots$, often ordered in time, and want to determine if any differ from the initial $D$.  A practical example is if each $D_i$ is a sample of measured attributes (e.g., quality score, breaking strength) of individual units of an item produced on an assembly line on day $i$; $D_i$ are monitored over time to see if the industrial process seems to have different results, which may indicate a quality change.

\subsection{Supervised vs unsupervised detectors
\label{ssec:types_sequential}}
Previously, we considered the observed data to consist of two samples $D$ and $D'$.  In sequential detection, the data may consist of batches or samples, each known to come from a potentially different distribution $D_i$, or may just consist of a sequence of individual observations without any such demarcation.  In general, consider the data as a sequence $x_1,x_2,\dots$; $x_i$ may be multivariate, but we will initially assume it is univariate.  Here, the task often consists of identifying one or more time indices $t_1, t_2, \dots$  (typically called changepoints), if they exist, where the data distribution has changed, or drifted.  Due to the vast literature on sequential changepoint detection, we will not attempt to provide an in-depth review, but rather summarize some of the aspects of such algorithms.  
Broadly speaking, sequential algorithms can be thought of as either supervised, semi-supervised, or unsupervised.  In general, a supervised model, such as a classifier, returns a prediction (e.g., of the label), which is then compared to a ground truth value.  A supervised sequential detection algorithm can be used when, for instance, $x_i$ are observations for which the ground truth label $y_i$ is available\footnote{We mean that the ground truth is known (e.g., we know, whether the customer with attributes $x_i$ ends up buying the product ($y_i=1$) or not ($y_i=0$), from an observed interaction.  In contrast, say $x_i$ are mammogram images or hardware test logs, which require an expert to examine and assign a true label $y_i$ for.  It may be `expensive' (in terms of time, effort, and money) to determine $y_i$, and perhaps it may be feasible to only label a small subset of instances.  The time aspect is particularly important: obtaining $y_i$ may cost no effort or money, but only time, in that it will be known only after a long time delay of the `arrival' of the initial data $x_i$.  For instance, $y_i$ is the success/failure of a treatment or death/survival of a patient with attributes $x_i$ in a clinical trial.  In these cases, it may be difficult to assess the model accuracy for changes, since $y_i$ may not be available for comparison with the prediction $\hat{y}_i$; alternative approaches which we discuss, such as monitoring changes in $x_i$ or in the model's prediction confidence, may be used.}, and for which an ML model has been trained to predict a label $\hat{y}_i$.  Typically, these detectors measure changes in a sequence of model accuracy measures, such as $I(\hat{y}_i=y_i)$ (binary indicator of correctness, from which the accuracy rate can be estimated) or the error $\hat{y}_i-y_i$ when the target is numeric rather than a class.  The relevant drift aspect is typically whether the error (in terms of its distribution or average) changes over time; as before, this may be separate from whether the distribution of $\{x_i\}$ themselves have changed.

In unsupervised\footnote{Clustering is an example of a unsupervised algorithm.} algorithms, there may or may not be an associated ground truth $y_i$.  Unsupervised drift detection algorithms typically try to detect drift in the distribution of $\{x_i\}$ themselves.  In the simplest cases, $x_i$ are univariate and numeric, and the sequence is monitored for changes in the average value or variance.  A comprehensive review and taxonomy of unsupervised detection algorithms is given in \cite{GCGD2020}. If $x_i$ (as opposed to the target $y_i$) is itself a binary variable, then one can monitor changes in it by applying some of the same supervised detectors, which typically assume the observed binary variable is $I(\hat{y}_i=y_i)$.  

\subsection{Aspects of sequential detectors}
\label{ssec:aspects_sequential}

As mentioned in Section~\ref{ssec:types_sequential}, supervised algorithms typically detect changes in an ML model performance by monitoring changes in average accuracy (since the ground truth value $y_i$ is available), while unsupervised techniques typically monitor changes in the underlying numeric observation $x_i$ distributions (particularly average value).  As such, to detect drift, typically two measured quantities (e.g., average accuracies or means of $x$) or samples of values are compared, and a threshold is used to decide if the comparison is divergent enough to indicate a significant change.  Usually, either the two samples (representing more recent and older data) are compared directly, or the current value (of, say, the average value or consecutive difference) is compared to the minimum value observed in the past.  The algorithms, whether supervised or unsupervised, often differ in some of the following aspects:

 \begin{enumerate}
  	\item \textbf{Parametric vs nonparametric}: can the data be assumed to follow a particular parametric distribution (particularly Gaussian)?  If so, given that the distribution can be characterized by a single parameter $\theta$ (e.g., Gaussian mean), many methods involve detecting when $\{x_t\}$ seem to change distribution from $\theta_0$ to $\theta_1$, which are pre-specified.
  	\item \textbf{Memory and windowing}: Memory refers to the amount of past data values $x_t$ (or sufficient statistics, such as a transformation of the values) that are kept in the algorithm memory, to detect drift.  A window is a subset of the observed data, typically the most recent data $\{x_k,\dots,x_t\}$, where $t-k+1$ is the window size.  Some algorithms have unlimited memory, comparing the newest data to the full recorded history (again, either the actual data values, or a running average or overall maximum/minimum of the historical values), or only perform a comparison versus a window of data (i.e., not the full history), which moves over time. Some methods also detect drift by comparing two windows of data, particularly the two most recent ones.
  	\item \textbf{Fixed window size vs adaptive}: If a window is used, then the window may be of fixed size $t-k+1$, or may vary over time.  For instance, if the data appears to be changing, one may want to increase the window size.
  	\item \textbf{Online vs offline}:  An algorithm is online if it has access to only a subset (possibly a moving window) of the data to make decisions each time; in contrast, an offline algorithm can examine the whole sequence of $\{D_i\}$ when making the decision.  The choice to use an online or offline algorithm often has to do with the circumstances of the observations themselves.  For instance, data $\{D_i\}$ may have to be monitored in an online fashion if the full historical data cannot be stored\footnote{However, it may be possible to store some summaries of fixed size, say the cumulative means and standard deviations of the data $\{D_1,\dots,D_t\}$ up to each time $t$, and use this to detect drift, even if the individual past observations cannot be stored.} (perhaps due to memory or storage limitations), and so drift must be detected without examining the full past history, or not.
\end{enumerate}

For offline drift detection, algorithms also typically either detect only one or multiple changepoints.  Sometimes, the number of changepoints must be specified in advance, or a parameter (e.g., a penalty term) is specified to reduce overfitting, by deciding how significant a changepoint should be to be considered.  Ideally, an algorithm should not require such parameters to be specified, particularly if their values are hard to interpret.  An online algorithm will typically simply detect and collect changepoints over time, and hence this distinction usually applies to offline algorithms.

We will focus on the nonparametric case since they are more realistically applicable.  Regarding the window size, if the user specifies a fixed window size or time decay weight, this implies knowledge of the time scale that indicates a change in distribution, particularly if one wants to detect multiple changepoints.  For instance, consider the following toy sequence $\{x_i\}=\{\splitatcommas{1,1,1,1,0,0,0,0,0,0,1,1,1,1,1,0,0,1,0,0,0,1,1,1,1}\}$.  The sequence changes between 0 and 1 roughly every 5 instances, meaning this is the time-scale of drift occurrence.  Of course, in reality, the time-scale is unlikely to be fixed and the drift is unlikely to be so drastic and frequent.  In this case, the ideal window size is 5, since the window average (e.g., the sample mean or proportion) changes sharply as the window captures instances from the same distribution. If the window size was, say 10, then the window mean would remain roughly equal as it slides.  See the discussion of ADWIN in Section~\ref{sssec:univariate_sequential_binary} below.

Below, we will focus on drift detection algorithms that are implemented in Python.  However, we note that the Massive Online Analytics (MOA,~\cite{MOA}) framework, frequently cited in research papers, provides a wrapper for simulating and detecting drift, and may be an alternative.

\subsection{Univariate sequential drift detection}
\label{ssec:univariate_sequential}

\subsubsection{Univariate sequential drift detection on binary \texorpdfstring{$x_i$}{x} or \texorpdfstring{$y_i$}{y}}
\label{sssec:univariate_sequential_binary}

Here, we summarize common algorithms for drift detection on binary variables; as mentioned, the supervised algorithms for binary targets $y_i$ can be used on binary input data $x_i$ as well.  The discussion is summarized largely from the survey paper \cite{BS2018}.  These drift detectors often rely on changes in the observed sequence of binary values, or in changes in average values (current values of proportions $p_i\in[0,1]$, possibly with their standard deviations $s_i\ge 0$, which may be calculated cumulatively with unlimited memory, or over a past time window only).  If $y_i$, rather than $x_i$ is observed, then $p$ is accuracy (and $1-p$ is the error) rate of the classifier.

DDM (Drift Detection Method, \cite{GMCP2004}) monitors changes in $p$; it alerts when $p_i+s_i\geq p_{\textrm{min}}+k\times s_{\textrm{min}}$, where the $\phantom{}_{\textrm{min}}$ subscript denotes the minimum observed values of these summary statistics.  $k=2$ is a warning threshold, while $k=3$ gives the detection threshold.  The threshold resembles the formula for the $z$-score of $p$, except the minimum rather than average values are used.  RDDM (Reactive Drift Detection Method, \cite{BCGC2017}) is a modification of DDM which discards some past data to achieve better detection.  STEPD (Statistical Test of Equal Proportions,~\cite{NY2007}) performs a two-sample difference-in-proportions test (see Sections~\ref{sssec:two_sample_continuous_univariate}, ~\ref{ssec:drift_in_data_slices}) on a historical vs recent moving window of fixed size of the binary indicators.  In contrast, EDDM (Early Drift Detection Method,~\cite{BCFBGM2006}) detects drift in the distance between consecutive errors (on the assumption that errors should be more rare than correct predictions).

ADWIN (ADaptive WINdowing,~\cite{BG2007}) is another popular method.  Here, a moving window $W$ is initialized as $\{x_1,\dots,x_n\}$, for a specified $n$, but the size of $W$ is data-adaptive, rather than constant, throughout the algorithm's search.  This eliminates the need for the user to specify the fixed window size, which implies knowledge of the time-scale of drift occurrence (see above, Section~\ref{ssec:aspects_sequential}).  The window $W$, say of size $k$, always contains the most recent data subset that is determined to not have drift in it.  $W$ is repeatedly subdivided into $W_0$ (the first $r=1,\dots,n-1$, in turn, items) and $W_1$ (the remaining last $r=n-1,\dots,1$ items).  Drift is detected if at any of the $k-1$ splits, $|\mu_0-\mu_1|\geq \epsilon_{\delta}$, where $\mu_i$ is the sample mean of window $W_i,\:i\in\{0,1\}$, and $\delta$ is a confidence parameter\footnote{The decision threshold is $\epsilon_{\delta}=\sqrt{0.5(\frac{1}{n_0}+\frac{1}{n_1})\log{(\frac{4(n_1+n_2)}{\delta})}}$, where $n_0$ and $n_1$ are the current sizes of $W_0$ and $w_1$.  The threshold guarantees that if the sub-samples $W_0$ and $W_1$ were actually generated from distributions with means that differ by at least $\epsilon_{\delta}$, this drift would be detected with probability at least $1-\delta$.  Also, if they were actually generated from the same distribution, drift would \textit{not} be detected with probability at least $1-\delta$.  This is essentially false positive and negative control at each observation.}.  This iterative testing means that ADWIN can detect drift at varying time-scales (i.e., sizes of sub-windows $W_0,\:W_1$).  If no drift is detected at any split, $W$ grows to include the newest observation, since the potential time-scale for drift has grown.  If drift is detected at a split $(W_0,\:W_1)$, $W_0$ is discarded and $W=W_1$, which represents the best guess of the new distribution.  Thus, as before, detections of drift cause the window size to shrink, while not detecting causes the window size to expand.


\subsubsection{Univariate sequential drift detection on continuous \texorpdfstring{$x_i$}{x}} 
\label{sssec:univariate_sequential_continuous}

Whereas the methods in Section~\ref{sssec:univariate_sequential_binary} assume the observed data are binary (i.e., Bernoulli-distributed), here the observed $x_i$ are continuous-valued.  In general, drift is detected by either a single jump or spike in the values, or a more sustained change in the average value or variance that.  We first mention common methods that are available in several software implementations.

Page-Hinkley (PH,~\cite{P1954}) is one of the oldest detection algorithms.  Letting $\bar{x}_t=\frac{1}{t}\sum_{i=1}^t x_t$, the cumulative sample mean, let $m_{t+1}=\sum_{i=1}^t(x_t - \bar{x}_t + \alpha)$. PH detects drift if $m_t - \textrm{min}(\{m_i\}_{i=2}^t)$ exceeds a specified parameter $\lambda>0$.  In its original formulation, PH only detects increases in the means.

HDDM (Hoeffding Drift Detection Method,~\cite{FCRMOC2015}) detects drift in a moving window of real-valued observations. Detection of drift is based on Hoeffding's inequality, which gives probabilistic bounds on the likelihood of a sum of independent random variables exceeding their expected value by given thresholds; as such, it has both a probabilistic guarantee and is nonparametric.  HDDM works as such: two complementary windows $\{x_1,\dots,x_m\}$ (`before') and $W=\{x_{m+1},\dots,x_t\}$ (`after') are maintained and updated sequentially.  Let $\bar{R},\bar{W}$ and $\mu_R,\mu_W$ be the window sample and hypothetical population means, and $\alpha>0$ is a confidence parameter.  A threshold $\epsilon_\alpha$, determined by $\alpha$ and $n$, is set that $|\bar{R}-\bar{W}|$ must exceed to provide sufficient evidence (judged by confidence $\alpha$) that their population means $\mu_R$ and $\mu_W$ must also differ significantly.  If they do, this is evidence of drift in the mean values, before an after index $m$, the best guess of the changepoint.
The HDDM algorithm can give lower weight to older observations, and detect one-sided (specifically increase or decrease) or two-sided (either) in $\mu_R$ vs $\mu_W$. It also can detect either abrupt (`A') or gradual (`W' for weighted averages) changes in the mean value.

KSWIN (Kolmogorov-Smirnov WINdowing,~\cite{RHS2020}) uses the Kolmogorov-Smirnov two-sample test (see Section~\ref{sssec:two_sample_continuous_univariate}) to detect drifts by changes in distribution between the most recent data (sample $R$, of size $r$) and older data (sample $W$, also of size $r$).  $W$ is drawn uniformly from the first $n-r$ observations of a larger window of size $n$ ($n \geq 2r$), the final $r$ values of which constitute $R$.  The parameter $r$ indicates the sample size used to make the decision, while the larger $n$ is, the more memory it has, because older values can be selected for $W$.  Drift between $W$ and $R$ is detected based on the KS test statistic threshold and a specified confidence level $\alpha$.

There are several comprehensive Python implementations of these detection algorithms:   \texttt{scikit-multiflow}'s (\cite{MRBA2018}) \texttt{drift\_detection} module and \texttt{river}'s (\cite{river}) \texttt{drift} module both implement the ADWIN, DDM, EDDM, HDDM (with extensions HDDM\_A and HDDM\_W), KSWIN, and PH algorithms.

Changefinder (\cite{TY2006}; implemented in Python as \texttt{changefinder},~\cite{changefinder}) is an online detection algorithm that uses sequentially-discounted auto-regressive (SDAR) learning.  In auto-regression (AR), a regression model is learned from observed values to predict future values.  For instance, if $x_t$ is the observed price of a stock on day $t$, a model might predict $x_t=p_{t-1}= -1.5x_{t-2} + 3.2x_{t-3} + \epsilon_t$, where $\epsilon_t$ is a random error component.  AR models are the simplest example of a time series model; the `order' of the model is the maximum lagged term used, which here is 3 since $x_{t-3}$ is the earliest term used to predict $x_t$.  In the changefinder algorithm, an AR model of fixed order is learned, where the AR regression parameters are updated sequentially with discounting, so that the estimates learned at past input values $t-k,\:k>0$ have less input on the estimates at time $t$.

Given the current regression model $p_{t-1}$, the predicted value, say $\hat{x}_t=-1.5x_{t-2} + 3.2x_{t-3}$ (without the error $\epsilon$, whose variance is also learned over time), is calculated.  $s(x_t)$ is a scoring function that measures the prediction loss, that is, the deviation, between the observed $x_t$ and its predicted value $\hat{x}_t$.  Changefinder detects loss when the score $s(x_t)$ appears unusual.  That is, it is not necessarily that the values $x_t$ themselves change, but rather that the predicted AR relationship appears to have changed, which indicates distribution drift.  For instance, if the learned model is $x_t=2x_{t-1} +\epsilon_t$, $x$ should approximately double each time, and thus we expect to see a sequence such as $x_{t-2}=3$, $x_{t-1}=6$, $x_t=12$; note that $x$ continues to grow and not linearly, since the successive differences $x_t-x_{t-1}$ also grow.  If, however, $x_t=5$ rather than the predicted $\hat{x}_t=12$, this would appear anomalous given the learned AR relationship, even though the value 5 is not in itself unusual relative to the previous values (treated as a sample).  This algorithm would be most appropriate if the data can be reasonably assumed to follow such an AR relationship (and thus are not independent draws from a fixed distribution), although presumably it could also be used in those instances, except that the AR model would resemble noise, where $x_t$ would not be expected to be much different than past values.

\subsection{Multivariate sequential drift detection on continuous \texorpdfstring{$x_i$}{x}}
\label{ssec:multivariate_sequential_continuous}
 
We now mention several algorithms for multivariate sequential drift detection.  We note, however, that is the observed $x_t$ is actually the multivariate embedding of natural language documents, then it is likely better to use methods that are specific to natural language.  As before, we also focus on nonparametric methods.

The algorithms mentioned here are all offline (retrospective) and return a partition of the observed $\{x_1,\dots,x_t\}$ into contiguous segments, each of which is separated by a changepoint.  If no changepoints are detected, the entire sequence comprises one segment.  The entire sequence is typically modeled as piecewise stationary, so that within each segment, the observed $\{x_i\}$ follow a single stationary (stable) distribution.

The Energy Change Point (ECP) algorithm (\cite{JM2014}; originally implemented in \texttt{R} (\cite{Rlang}) as \texttt{ecp}, \cite{JMW2019}, and in Python as \cite{G2019}; see also \texttt{R} vignette \cite{JM2014vig}), can detect multiple changepoints in a sequence of multivariate (or univariate) observations, assuming independent draws, without having to specify a priori how many changepoints are expected.  The energy statistic (also used in \cite{SR2013}, see Section~\ref{sssec:two_sample_continuous_multivariate}), with discounted time weighting, is used to measure multivariate distribution divergence.  Compared to other methods, ECP makes few assumptions, does not require user-specified parameters (such as a penalty term value to determine a changepoint's significance), and can detect various types of distributional change, not only in the mean or variance.  They demonstrate that ECP can also detect changes in the joint distribution (e.g., in the covariance), while the marginal distributions remain the same.  Also, using experiments on mixtures of multivariate Gaussians, they show it can also detect changes in multi-modal distributions (e.g., a 2-D topography with multiple peaks).

ECP has two different modes:
\begin{itemize}
	\item divisive: the algorithm uses a tree approach to recursively divide the entire observed sequence into segments, each of which is separated by a changepoint.  The significance of a new potential changepoint, given the  is evaluated by a permutation test, while keeping the previous division fixed.  If no division is performed (i.e., the tree consists only of a root), no significant changepoints are found.
	\item agglomerative: given an initial division of the sequence into segments (either provided by the user, thus allowing a priori knowledge of potential changepoints to be used; or if not, each observation is its own changepoint), the segments are recursively agglomerated as long as the agglomeration is statistically significant.  It is assumed there is at least one changepoint (i.e., the agglomeration cannot return a single changepoint).
\end{itemize}

The Python library \texttt{ruptures} (\cite{ruptures}) provides a suite of tools for simulation of univariate and multivariate data with known changepoints (data can be piecewise constant, linear, Gaussian, or sinusoidal, with specified noise magnitude) and detection of changepoints using various methods (see \cite{TOV2020} survey article).  Various cost or kernel functions can be used as inputs to the detectors; there is also an option to create a custom cost function.  The cost (or loss) functions serve to model the deviation that is expected to be observed relative to a baseline.  The various supported algorithms perform a segmentation that minimizes the total value of the specified cost function, where the total is the sum of the costs of each segment separated by the changepoints.  If the number of changepoints is unknown, a penalty function (which penalizes each additional segment, or changepoint) is included in the function to be minimized.  The penalty serves to prevent over-segmentation (over-fitting); on the other hand, if the penalty is too high, then few, if any, changepoints will be significant enough to be detected.

The choice of an appropriate cost function depends on the modeling assumptions.  Note, following the notation in \cite{TOV2020}, we use $y_t\in \mathds{R}^d$, rather than $x_t$, to denote the multivariate $d$-dimensional signal.  Below, we outline the cost functions available in \texttt{ruptures}; the cost functions described are per-segment, where typically the cost is calculated as the deviation from some fixed value (e.g., mean signal value $\bar{y}_t$ in that segment, or some other value that must be optimized to minimize the segment cost).

\begin{itemize}
\item \textbf{$L_2$ (squared error) loss}: if drift (a changepoint) is characterized by a change in the mean value (but not variance) of $y_t$.  Cost is the the sum of squared deviation from the segment vector mean.
\item Say that for segment indexed $k$, $y_t=x_t'\mu_k + z_t'\eta + \epsilon_t$, where $x_t\in\mathds{R}^p$ and $z_t\in\mathds{R}^q$.  That is, $y_t$ (here univariate) is modeled by a multiple linear regression model on covariates $x_t$ and $z_t$, where the coefficients $\mu_k,\:\eta$ are unknown, but $y$'s dependence (constant coefficients $\eta$) on $z_t$ is fixed throughout the sequence of observations, but the dependence on $x_t$ changes by the segment (hence the segment-varying coefficients $\mu_k$, which cause the distribution drift in $y_t$).  An example is if, say, $y_t$ is the monthly price of a stock, $z_t$ is the national unemployment rate, and $x_t$ is a monthly profitability measure of the company.  Perhaps the segments represent tenures of the company's CEOs, any the relationship between stock price and profitability depends on the CEO in charge.  In this scenario,
	\begin{itemize}
	\item \textbf{linear cost} measures squared divergence between $y_t$ and $x_t'\mu$, where $\mu$ is some fixed (not varying) coefficient in that segment; thus, this cost measures divergence from some baseline based on changing coefficients $\mu_k$ (unknown) on $x_t$ only.  
	\item \textbf{$L_1$ (linear) loss} measures the absolute value (not squared) deviation of $y_t$ from both $x_t$ and $z_t$, again assuming a fixed coefficient $\mu$ on $x_t$.
	\item \textbf{Auto-regressive (AR) loss} measures the loss when $y_t$ is modeled auto-regressively with a specified lag order within the segment, with fixed coefficients $\mu$, which may have similar results to the \texttt{changefinder} algorithm (Section~\ref{sssec:univariate_sequential_continuous}).
	\end{itemize}
\item \textbf{Mahalanobis loss}: Similar to $L_2$ loss, except here Mahalanobis distance is used, where the element-wise squared deviation from the segment mean $\bar{y}_t$ is penalized by the observed standard deviation of that feature.  That is, a fixed squared deviation $c>0$ for a given feature is considered to be a larger distance (higher cost) if that feature had lower variation.  This cost is useful if features have differing variances (or measurement scales) within a segment.
\end{itemize}


\subsection{Statistical control of sequential detection}
\label{ssec:sequential_statistical_control}

The statistical guarantee on a statistical test is generally only valid when performed once.  Consider the two-sample hypothesis tests or effect size metrics in Sections~\ref{ssec:two_sample_continuous} and \ref{ssec:two_sample_class}.  Say we have two independent numeric samples $\mathbf{x}_1\sim P$ and $\mathbf{x}_2\sim P'$.  To test whether the unknown means of the distributions $P$ and $P'$ are equal, we can conduct either a two-sample T-test (which produces a p-value, which is then compared to a significance threshold $\alpha$, and drift is declared if the p-value is less than $\alpha$), or use Cohen's $d$ metric (which is then compared to significance rules of thumb).  A threshold of, say, $\alpha=0.05$ means that if $P$ and $P'$ actually have the same mean, then two samples will be (falsely) detected as having different means 5\% of the time; this is because a p-value returned by the test will fall below $\alpha$ on only 5\% of random samples.  

When the test is only conducted once, on a particular pair $\mathbf{x}_1$ and $\mathbf{x}_2$, this statistical guarantee holds.  However, if each different pair's p-values are (falsely) judged as significant with probability $p=0.05$ (by definition), if, say, we draw $n=20$ pairs, then on average one pair will be significant, and the probability that \textit{at least one}\footnote{Since the number of pairs judged as significant can be modeled as a binomial variable $X$ with size $n=20$ and probability $p=0.05$, this probability is $\textrm{Pr}(X\geq 1)\approx 0.264$, as confirmed by \texttt{1 - scipy.stats.binom.cdf(k=1, n=20, p=0.05)}.} will be significant is about 0.26.  The statistical correctness guarantee of $\alpha=0.05$ no longer holds because now we repeat the experiment $n=20$ times and wait for at least one\footnote{See Section~\ref{ssec:drift_in_data_slices} for a discussion on adjusting for the fact we are conducting multiple ($n$) hypotheses.} significant result.  If our method uses such a procedure to detect drift, it will likely have a higher false positive rate than desired.

It seems that for the sequential detection algorithms mentioned in Sections~\ref{ssec:univariate_sequential} and \ref{ssec:multivariate_sequential_continuous} where monitoring is done online, if a statistical test or threshold is used, usually the decision takes into account only the data sample used to calculate it.  If there is no adjustment for the fact that monitoring has actually applied the criterion over many past samples, then it's possible that changepoints may be falsely detected.  This is particularly true if we are allowed to make only one decision of drift (identify one changepoint), and we want to guarantee that, if we decide there has been drift, that the probability this is a false premature detection is at most, say $\alpha=0.05$; in addition, of course, we would like our detection of drift, when correct, to happen with minimal delay from the beginning of distribution change. 

For instance, the ADWIN criterion (Section~\ref{sssec:univariate_sequential_binary}) determines the threshold $\epsilon_{\delta}$ at which the window means $\mu_0,\:\mu_1$ must differ by by specifying the false positive control $\delta$.  However, this same threshold is applied anew each time without regard to the amount of time passed since the beginning of monitoring, and thus the probability of an eventual false positive may be high.

It seems that one of the few algorithms to perform such false positive control is the change point method (CPM).  The original algorithm (\cite{RA12}; implemented in \texttt{R} as \texttt{cpm}, \cite{R2015}) detects multiple changepoints in univariate numeric data, and \cite{PA2019} extends it to categorical data.  The monitoring is done in a streaming sequential manner at each time $t$ but requires the entire data history since the beginning or the last changepoint.  In short, the algorithm works as such: at each time $t$, the set of past values $\{x_1,\dots,x_t\}$ are split into before/after windows $W_0,\:W_1$ of minimum size 2 at every possible split point, similarly to ADWIN.  A divergence statistic between $W_0$ and $W_1$ is calculated for each split; various tests, such as the Student T test or Cram\'{e}r von
Mises (see Section~\ref{sssec:two_sample_continuous_univariate}) can be used, depending on which aspect (e.g., mean, variance, any distribution change) is of interest.  The split with the maximum divergence value is the most likely candidate for a changepoint.  However, the significance of the change is evaluated against a threshold that takes into account the number of splits (which increases linearly with the total observations $t$). In fact, these thresholds increase monotonically over time so that the more observations $t$ have been monitored, the larger the divergence must be; this adjusts for the fact that the more splits are possible, the higher the likelihood that one of them is by random chance falsely significant.  The statistical guarantee here is that \textit{whenever} drift is detected, the probability it is a false positive is controlled at the same level $\alpha$.  The downside of this algorithm is that there is no discounting or discarding of past data (except after a changepoint is detected, in which case the system resets), so the computation may become expensive after a point.  See \cite{ADFRZ2020} for more details and an illustration of drift simulation scenarios.


==> essential.tex <==
\chapter{Essential Economics}
This chapter discusses terminology, stock market dynamics, and important indicators in economics. This will allow us to more accurately judge the value of an economic decision and make predictions on the market.

\section{Funds}

We'll discuss three different types of funds: \acf*{etf}, mutual funds, and hedge funds. Different types of funds are governed under different rules. \ac*{etf}s are similar to stocks in that they are bought and sold at will like stocks- very liquid. However, \ac*{etf}s typically represent baskets of stocks, and it is known to the trader what the fund represents. Mutual funds can only be bought and sold at the end of the day, and the holdings within a mutual fund are only disclosed every quarter. The least transparent holdings are that of a hedge fund. Before investors can buy shares in the fund, they must sign a long term agreement and holdings are rarely disclosed. \\

\subsection{About Funds}

For stocks and \ac*{etf}s, having a large "cap" means that the total value of stocks (number of stocks $\times$ price of a stock) in a company is worth many billions of dollars. Moreover, the price of a stock doesn't reflect the value of a company, but the price at which they are selling shares. \ac*{etf}s, like stocks, can easily be traded through individuals alone, whereas shares in mutual funds require a broker and hedge fund shares require more of a one on one relationship. Managers of \ac{etf}s and mutual funds are compensated based on expense ratios, which denote a percentage of \ac{aum}. For an \ac{etf}, expense ratios range from 0.01\% to 1\%, and in mutual funds from 0.5\% to 3\%. Hedge funds follow a "two and twenty" policy, where managers get 2\% of the \ac{aum} and 20\% of the profits.\\

The type of a fund can be more easily recognized by how it's named. For example, an \ac*{etf} has a ticker, or stock symbol, with three or four letters, like AAPL. A mutual fund has five letters, like VTINX, and a hedge fund doesn't have a ticker because shares are much less liquid. How much money is managed by a fund is known as the \ac{aum}, and shares represent percentages of the \ac{aum}. \\

It's fairly clear to see that hedge funds are very different from \ac{etf}s and mutual funds. Hedge funds typically have no more than 100 investors, whereas \ac{etf}s and mutual funds have thousands. Those that invest in hedge funds are typically very wealthy individuals, institutions, and funds of funds. Funds of funds typically take large sums of money from potentially many places and invest in several hedge funds. This is a bridge for smaller investors to participate in hedge fund. The goal of a hedge fund typically falls along the lines of two ideals. The hedge fund may be out to beat a bench mark which is to say that the hedge fund aims to outperform an index of stocks. A hedge fund could also aim for absolute return, which translates to net positive profit no matter what, but usually takes more time and has fewer returns as a trade off for stability. We'll be focusing on hedge funds because they are the most computationally demanding.

\subsection{Fund Metrics and Operations}
Measuring the performance of a fund is vital for making financial decisions in the market, so here we'll discuss a few. Overall success can be measured by cumulative return, which is the percentage of an original value made in a given time: $\frac{end-start}{start}$. However, this means little if the portfolio is rapidly and wildly fluctuating. Hence it's also useful to measure the volatility of a portfolio. This is simply measured by the standard deviation of daily returns; it's best to have low volatility. Another important measure is the return on risks. This is done by calculating the \ac{sr}, also called risk-adjusted reward. 
\begin{align*}
\ac{sr}=\frac{mean(\mbox{daily returns}-\mbox{risk free rate})}{\mbox{volatility}}\sqrt{252}
\end{align*}
The factor of $\sqrt{252}$ comes from the number of trading days in a year. These factors can give us an idea of how well a portfolio is performing.\\

As previously mentioned, hedge funds are very computationally intensive environments. Let's delve into the details of how a typical hedge fund works. Central to the operation of a hedge fund is its trading algorithms. Normally, a target portfolio is decided upon, then historical stock data and the target portfolio are fed to the trading algorithms to produce orders. The orders are sent to the market to alter the live portfolio, which is again fed back into trading algorithms. 
\newpage

\begin{figure}[h!]
\begin{center}
\includegraphics[scale=.4]{images/operation.JPG}
\caption{Graphical representation of hedge fund operation.}
\end{center}
\end{figure}

Trading algorithms work to place certain orders at the proper time. For example, an order for everything in the target portfolio shouldn't be placed all at once because the price of the stock will go up and more money is spent than if strategic ordering were implemented. Additionally, there is another set of computational structures for determining the target portfolio.

\begin{figure}[h!]
\begin{center}
\includegraphics[scale=.75]{images/target.JPG}
\caption{Producing a target portfolio.}
\end{center}
\end{figure}

Historical data, current portfolio, and prediction algorithms are fed into an optimization program to produce a target portfolio. The majority of machine learning comes into play when determining the market forecast. 

\section{Market Mechanics}

\subsection{Ordering}
The live portfolio is altered by giving orders to a broker in the stock market, so it serves to know what exactly is in an order. The broker needs to know whether to buy or sell and of which stock(s) by their market symbols. The order must also contain the number of shares and the type of order. Stock exchanges only consider limit orders and market orders, but note that orders can be increasingly complex based on instructions given to a broker. A market order is an order at the current market price, and ordering at a limit price tells the broker to only buy or sell at a certain price; for example, some may not want to buy beyond some value or sell below some price. Of course, a limit order must also include the desired price. \\

\begin{table}[h!]
\centering
\begin{tabular}{c|c|c|c|c}
BUY/SELL & SYMBOL & SHARES & TYPE & PRICE \\
\hline
BUY & IBM & 100 & MARKET & - \\
BUY & AAPL & 500 & LIMIT & 100 \\
SELL & FB & 1000 & LIMIT & 110 \\
BUY & GOOG & 100 & LIMIT & 740 \\
SELL & NFLX & 50 & MARKET & - \\
SELL & GE & 50 & LIMIT & 40 \\
\end{tabular}
\caption{Example list of orders.}
\end{table}

After the broker sends the order to the stock exchange, it is made public in the style of an "order book". Others can see the stocks and collective bids that have been made on them, but not who has placed the orders. The order book contains a list for each stock of the orders within it including whether the order asks for others to buy or bids on the stock. Both types include a price at which orders are allowed to be bought/sold at and the size of the order. Orders of the same type and price are lumped together. Market orders always sell at the highest bid and buy at the lowest asking price. \\

\begin{table}[h]
\centering
\noindent\begin{tabular}{c@{}l}
  \begin{tabular}{c|c|c}
  	BID/ASK & PRICE & SIZE \\
    \hline
    ASK & 100.10 & 100 \\
	ASK & 100.05 & 500 \\
	ASK & 100.00 & 1000 \\
	BID & 99.95 & 100 \\
	BID & 99.90 & 50 \\
	BID & 99.85 & 50 \\
  \end{tabular} 
  & 
  $\begin{array}{l}
  \\
    \MyLBrace{5ex}{SELL} \\ 
    \MyLBrace{5ex}{BUY} \\ 
  \end{array}$
\end{tabular}
\caption{Example order book.}
\end{table}

The example order book suggests that the price of the stock will decrease because there is much more selling pressure- more are selling than buying. \\

\subsection{Dynamics of Exchange}
There are many stock exchanges, and each has its own order book. When an order is placed, say by an individual, the order is sent to the broker and the broker chooses between the stock exchanges to execute that order. The broker takes information from all the stock exchanges and makes a transaction based on which one has the stock with the best price. Fees are associated with making transactions in stock exchanges and with using a broker. A broker typically has many clients; the broker can observe clients who want to buy and sell at the same price and circumvent stock exchanges entirely. The law ensures that this trade can only happen if both the buyer and seller get prices that are at least as good as at an exchange. Even if this transaction cuts out the stock exchange, it must still be registered with one, and it's usually with the exchange the stock is housed. \\

Orders can be handled internally or moved through what's called a "dark pool". A dark pool is a place where investors can trade without the transparency of an order book outside of a stock exchange. The results of the trade, like internal trades, still need to be registered with public exchanges after they've occured. A dark pool can act as an intermediary between all types of investors that may want to escape the transparency of stock exchanges. Brokers like this because they don't have to pay fees associated with trading at a stock exchange. They also argue that it's fair because clients are getting prices that are as good as at the market. However, hedge funds and dark pools can heavily exploit this system as it stands if they have well-placed, fast computers. \\

\subsection{Exploiting the Market}
These days the market is entirely digital and computers automate transactions all across the country. As a result, orders can be processed in fractions of a second, and timing is everything. A hedge fund may pay stock exchanges enough money to house computers very close to the exchanges, which gives them a distinct advantage. For example, let's say that someone places an order for a stock, and it's sent to multiple markets. A hedge fund close to those markets can see that order reach one of them first and buy up that stock from the other exchanges through the high speed infrastructure they have in place. Then when that order reaches other exchanges, the hedge fund has already bought those shares and sells it back at a higher price. This is one of many strategies in \ac{hft} that takes place on the order of milliseconds. \\

This can also happen on an international scale. A hedge fund may have computers collocated with international markets rapidly observing and comparing order books between them. If a difference occurs in a stock between the two markets, all that needs to be done is to sell in the market with a higher price and buy in the market with a lower one. This happens very quickly, so the price of the stock is not very different at different markets. \ac{hft} strategies usually trade high volumes to turn a large profit in small price differences. \\

Those that operate on \ac{hft} strategies can not only manipulate a transparent market, but also a dark one. First, let's explain why someone would want to use a dark pool. For example, an investor who wants to sell a high volume of shares in a transparent market would want to do so in small chunks so as not to upset the price all at once and get less for the shares. However, others will see this and lower their bids knowing that a high volume is to be sold and the investor still gets less for their shares. In a dark pool, others can't see those that want to buy or sell, so the investor may get a better price. There are many ways to exploit a dark pool, but it always stems from information leakage. Knowing the order book of a dark pool means a world of advantage. Dark pool operators or constituents may secretly participate in their own pool or leak information about it to others for a price. The private nature of a dark pool allows those who operate it to make their own rules about who can participate and how trading works. Since information is at the discretion of the operator, it's fairly easy for those with direct access to exploit a dark pool. Those that don't have direct access can "game" the pool by probing it with many small volume orders. This yields some idea of the size and prices of bids, which gamers can exploit by selling when they find the bids are highest and buying when asking is lowest.

\subsection{Other Orders and Shorting}
Although exchanges only take market and limit orders, other orders can be made through a broker. Often a broker implements them for clients without their knowledge to benefit both themselves and the client. The most simple order above a limit order is a stop-loss order. The broker holds stock until the price drops below a certain price, then sells at market price. Similarly, a stop-gain order waits until the price climbs to a point at which the client wants to sell. Slightly more complex is the trailing stop. Here the broker sets a stop-loss criteria trailing a stock that's increasing in price. As the price increases, so does the stop-loss criteria; when that stock starts to decrease, the stop-loss criteria is met and stocks are sold. \\

What if someone wanted to bet that a stock will decrease and still profit? Instead of just selling high and buying low, those stocks can be borrowed and sold, so the value of those stocks is gained at a high point but the stocks are still owed. Then when the price of the stock decreases, the stock can be bought at a lower value, and the shares returned to whom they were borrowed while a profit on the difference was made. This is called shorting. As long as the price of the stock goes down, this is a good strategy; however, if the price goes up, then the difference results in a net loss. \\

\section{Worth}
The price of a company's stock is intended to reflect the value of the company. Ergo, if the price of a company's stock deviates significantly from its predicted value based on the company's predicted worth, then there's a profitable opportunity for when it returns to reflect the company's worth. The value of the company can be estimated several different ways. One way is to estimate its intrinsic value, which is based on the future dividends the company will give; these are annual payments to stockholders. This doesn't really describe what the company has though. The book value of a company is founded in the company's assets like its facilities and resources. A company's market cap is yet another way to estimate a company's worth, and it's easiest to calculate. This is effectively what the stock market thinks what the company is worth and it's the value of a stock multiplied by the total number of stocks. \\
\newpage
Intrinsic value may not make sense if we try to imagine the value of a company that will pay dividends consistently as long as it stands. However, the company can never be 100\% reliable, so the value of its dividends amount to the value of a promise. The promise of some money in a year is worth less than the same amount given right now because of this principle. Thus, the value of a those promised dividends decreases as the time they're promised is longer, so the total value will converge to a calculable value. Similarly, we can calculate the \ac{pv} of a dollar that is promised after a certain time. It makes sense that the \ac{pv} of a dollar promised right now is a dollar, but what about in a year? The \ac{pv} is some fraction of its \ac{fv} based \ac{ir} and the length of time, $t$.
\begin{align*}
PV=\frac{FV}{(1+IR)^t}
\end{align*}
In this way we have a conversion between the present value and future value of some amount of money. The interest rate is also called the discount rate and it reflects the risk involved with investment. A more stable company will have a lower discount rate because they're more reliable. The intrinsic value, $IV$, of a company can be calculated knowing its discount rate and dividend payments by
\begin{align*}
IV=\frac{FV}{IR}
\end{align*}
Thus, if a hypothetical company pays dividends of \$5 a year and has a discount rate of 1\%, then the value of this company is $\$5/0.01=\$500$. Book value of a company is simple to calculate because it is just what the company has versus what the company owes. If a company only has a factory worth \$1 million, a patent worth \$500,000, and a loan of \$200,000, then the company is worth \$1 million $-200,000=\$0.8$ million. The patent is considered an intangible asset and isn't counted in calculating the book value. \\

News about companies can drastically change some of these measures. Investors reflect their opinions on the worth of a company through stocks- if they feel the company is worth less, they will sell and vice versa. Let's say bad news about a company comes up; investors will see that as increased risk in investing in the company. The company will have to increase their \ac{ir} to appease investors and the intrinsic value of the company will reduce. This would also reduce the stock price of the company, which decreases the market capitalization of the company. News can affect singular companies, sectors of business, and the market as a whole depending on the scope of the news. \\

Market strategies are based on deviations in the estimated values of a company. For example, if the intrinsic value of a company drops and the stock price is relatively high given its history, then it would probably be a good idea to short that stock because the price will almost certainly go down. The book value of a company provides somewhat of a minimum for the market cap; that is because if the market cap goes below the book value, then a predatory buyer typically buys the whole company, breaks it apart, and sells its parts for the book value to turn a profit.
\newpage
\section{The Capital Assets Pricing Model}
The \ac{capm} is a model that is used to predict the return of stocks. To understand this model, a portfolio must be understood in more depth. The term portfolio has been used throughout this text, but has yet to be clearly defined; a portfolio is a set of weighted assets, namely stocks. A portfolio is a set of stocks that are weighted by their value, and all the weights add to 1. Some stocks might be shorted, so technically their portfolio value is negative and really the sum of the absolute value of their weights is 1. Mathematically written, where $w_i$ is the weight of a stock in a portfolio
\begin{align*}
\sum_i |w_i|=1
\end{align*}
and the return of the portfolio for a given day is
\begin{align*}
\sum_iw_ir_i
\end{align*}
where $r_i$ is the return for a stock in a day. As an example, lets say a portfolio is composed of two stocks, A and B, and their respective weights are 0.75 and -0.25 because stock B is shorted. Then if on a given day, stock A increases by 1\% and stock B decreases by 2\%, the result is a portfolio return of $(0.75)(0.01)+(-0.25)(-0.02)=1.25\%$. \\

A similar portfolio can be made for entire markets. Although, it's typically limited to an index which includes the largest companies in a market, like the S\&P 500 for the US market. These companies are weighted by their market caps, so a company's weight in the market is approximately that company's cap, $c$, divided by the sum of all caps.
\begin{align*}
w_i=\frac{c_i}{\sum_{j}c_j}
\end{align*}
The \ac{capm} predicts the return on stocks within a certain market with the simple equation\footnote{Functions have dependent variables in brackets because they are discrete; a result of using digital time.}
\begin{align*}
r_i[t]=\beta_i r_m[t]+\alpha_i[t]
\end{align*}
This says that the return of a stock is largely based on the return of the market as a whole, $r_m$. The degree to which a stock is affected is based on that stocks particular $\beta$ value. Fluctuations that deviate from this are represented in the (theoretically) random variable, $\alpha$, which (theoretically) has an expected value of zero. The $\beta$ and $\alpha$ values of a stock are calculated based on the historical data of daily returns. The daily returns of a stock are plotted against that of the market and the slope of the fitted line constitutes the $\beta$ value. The y-intercept and random deviations describe the $\alpha$ value.

\subsection{CAPM and Related Theories}
The nature of \ac{capm} suggests a specific strategy when approaching the market. \ac{capm} says that the relationship of stocks to the market is linear with an average fluctuation of zero from this relationship. This suggests that the best tactic is to simply choose a set of stocks that will perform well with a certain market environment and sit on them. Active management is a way of thinking that believes the $\alpha$ value is not entirely random and can be predicted. This mindset promotes carefully choosing and trading stocks on a regular basis depending on predicted $\alpha$ values. This is the dichotomy between active and passive portfolio management. If we assume that $\alpha$ is entirely random, then the only way we can beat the market is by predicting the return on the market. However, this is not entirely true, and \ac{capm} will be used to eliminate market risk entirely. \\

\ac{capm} gives $\beta$ values to each stock, but there are other theories that say it's more complicated. One of these is the \ac{apt}, which says that there is not a contribution based on the whole market, but based on its sectors. Moreover, a stock is affected by what happens in the ten different sectors of the economy, and the \ac{capm} equation becomes
\begin{align*}
r_i=\sum_j\beta_{ij} r_j[t]+\alpha_i[t]
\end{align*}
where $j$ denotes the different sectors. This provides a more in-depth prediction of stock return.
\subsection{Using the CAPM}
Now we want to use the \ac{capm} to create a lucrative portfolio. If we say that the return on the market can never be predicted, then any component associated with market return is risk. Applying the \ac{capm} equation to get an overall portfolio return yields
\begin{align*}
r_p=\sum_iw_i[\beta_i r_m(t)+\alpha_i(t)]
\end{align*}
The only way to remove the market return component is to choose weights such that $\sum_iw_i\beta_i=0$. At this point it may seem that there will not be an expected return for the portfolio because \ac{capm} predicts $\alpha$ to be random. It is here that the assumptions of \ac{capm} are wrong. Using some information, we can predict whether a stock will perform better or worse than the market, which will yield a profit regardless of which way the market goes. This information can come from expertise, some analysis, or, in our case, machine learning.

\section{Technical Analysis}
There are effectively two kinds of analysis: fundamental and technical. Fundamental analysis looks at the properties of a company to determine market decisions. Technical analysis looks at patterns in stock prices to make market decision; since technical analysis is clearly more useful aside from predatory buying, that's what will be discussed. \\

Technical analysis only focuses on stock price and volume. Using these to calculate statistics gives indications on what economic decisions to make. Technical analysis is most useful on shorter time scales and when combinations of indicators point to the same decision. \ac{hft} trade at the millisecond timescale and fundamental analysis firms operate at the timescale of years; humans and computers tend to work together at a timescale in between. 
\newpage

\subsection{Some Good Indicators}
It's useful to develop strategies based on time-series indicators, so here are a few. Momentum is a scale dependent indicator that suggests an upward or downward trend depending on slope. Moreover, an $n$-day momentum, $m$, for a stock with price function, $p[t]$, is calculated as
\begin{align*}
m=\frac{p[t]-p[t-n]}{p[t-n]}=\frac{p[t]}{p[t-n]}-1
\end{align*}
This is simply the difference in price as a ratio to the price $n$ days ago. Typically 5, 10, or 20 day momentum is used with values ranging from -0.5 to 0.5. Another indicator is a \ac{sma}; \ac{sma} is also scale dependent looking over an $n$-day window. The price of a stock over $n$ days is averaged and plotted over time where points are placed at the leading end of the window. However, to get a useful value, this needs to be compared to the real time price. Like momentum, it is done as a ratio
\begin{align*}
{SMA}[n]=\frac{p[t]-E(p[t-n:t])}{E(p[t-n:t])}=\frac{p[t]}{E(p[t-n:t])}-1
\end{align*}
Momentum and \ac{sma} together often prove to be strong indicators. For example, if there is strong positive momentum and a crossing of the price from the price being lower than the average to above- this is a good indicator the price will increase. Larger than normal deviations from the moving average are expected to return back to the average and indicate opportunities. Thus, if \ac{sma} is positive, it's a selling opportunity, and a buying opportunity if \ac{sma} is negative. \\

How those decision are made depends on the state of the stock, or its volatility. The standard deviation of the stock's fluctuations provides an excellent measure for when to make decisions. It depends on how certain we want to be that the price is an outlier. The farther the decision threshold is from the \ac{sma}, the more certain we are that the price is an anomaly. From basic statistics, if the decision threshold is placed two standard deviations away from the \ac{sma}, then we are 95\% sure the price is an anomaly. These bands, typically at two standard deviations away from \ac{sma}, are called Bollinger bands. The way this is written mathematically is, again, a ratio, which is between the price difference and the 2$\sigma$ length where $\sigma$ is the standard deviation.
\begin{align*}
{BB}[t]=\frac{p[t]-{SMA}[t]}{2\sigma}
\end{align*}
When making economic decisions, a Bollinger band value greater than 1 denotes a selling opportunity, and less than -1 denotes a buying opportunity. However, it's better to trade when the price crosses the band for the second time because that signals the price moving in a profitable direction. \\

When using these values in a machine learner, it's important that indicators are normalized. To normalize values, follow
\begin{align*}
normal=\frac{value-mean}{\sigma}
\end{align*}
This provides a z-score by which to compare everything.

\subsection{Adjusted Price}
Analysis of historical data is crucial for determining patterns and making economic decisions, but some things drastically  change the price of stocks without having any effect on the real value of the stock. Dividends and stock splits are two things that do just that. The adjusted price accounts for these events and corrects the computational problems that would occur if only the price were taken into account. \\

Stock splits occur when the price of a stock is too high and the company decides to cut the price, but increase the volume so that the overall market cap is the same. This is a problem when dealing with data because it's seen as a large drop in price. The adjusted price is calculated going backwards in time; moreover, the given and adjusted price are the same for a certain starting present day and adjusted going backward in time. If the price is ever split, say by 3, then at the time of the split, the price is divided by 3 so that there is no discontinuity. \\

At the time a company announces the date for payment of dividends, the price of the stock will increase by the amount of a dividend until they're paid at which point the price rapidly decreases by that amount. This is adjusted looking back in time, and on the day a dividend is paid, the prices preceding are decreased by the proportion of the dividend payment. \\

As a note for machine learning, the data that is chosen for the learner is very important. If the stocks from today are chosen and analyzed starting from 7 years ago, then those stocks will of course do well because they've survived. That's using a biased strategy, so what needs to be done is to take index stocks from 7 years ago and run with those. For adjusted price, it's also important to note that the adjusted price will be different depending on where the starting point is chosen, and that should also be taken into account.

\section{Efficient Markets Hypothesis}
\noindent Until now, we've been assuming, for technical analysis, that there is information in historical data that we can exploit to determine what the market is going to do. The same goes for fundamental analysis in terms of fundamental data. However, the Efficient Markets Hypothesis says that we're wrong on both accounts!\\

\noindent Here are some assumptions of the Efficient Markets Hypothesis:

\begin{enumerate}
	\item \textbf{Large number of investors} The most important assumption of EMH is that there are a large number of investors for-profit. They have incentive to find where the price of a stock is out of line with its true value. Because there are so many investors, any time new information comes out, the price is going to change accordingly.
    
    \item \textbf{New information arrives randomly} 
    \item \textbf{Prices adjust quickly}
    \item \textbf{Prices reflect all available information}
\end{enumerate}

\subsection{The three forms of the EMH}
\noindent There are 3 forms of the EMH, ranging from weak to strong.

\paragraph{Weak} Future prices cannot be predicted by analyzing historical prices. This leaves room for fundamental analysis, however.
\paragraph{Semi-strong} Prices adjust rapidly to new public information
\paragraph{Strong} Prices reflect all information, public and private
\subsection{Is the EMH correct?}
\noindent If the EMH is correct, a lot of what we're trying to do is impossible, so we should cut our losses and go home. Luckily, there is evidence for why certain versions of the hypothesis are incorrect. The existence of hedge funds indicates that you can profit by investing in stocks other than the market portfolio.\\

\noindent The strong version is the weakest of the three, considering there are many examples of insiders using esoteric information for their own benefit. And in many cases, these people have gone to jail!\\

\noindent There is also data that shows that the semi-strong version isn't too likely to be correct. You can see trends in 20-year annualized returns versus 10-year P/E ratio data, which means that you most likely can use fundamentals to predict future performance.\\

\section{The Fundamental Law of Active Portfolio Management}
\noindent Richard Grinold was trying to find a way of relating performance, skill, and breadth. For example, you might have lots of skill to pick stocks well, but you might not have the breadth to use that skill. So he developed the following relationship:
\begin{equation*}
{performance} = {skill}\sqrt{breadth}
\end{equation*}

\noindent So we need some way of measuring skill and breadth. Performance is summarized by something called the \textit{information ratio}:

\begin{equation} \label{eq:inforatio}
{IR} = {IC}\sqrt{BR}
\end{equation}

\noindent where $IC$ is the \textit{information coefficient}, and $BR$ is the number of trading opportunities we have.

\subsection{The Coin-flipping Casino}
\noindent As a thought experiment, instead of buying and selling stocks, we're going to flip coins, and bet on the outcome. This is analogous to buying a stock and holding it-- either you earn or lose money.\\

\noindent The coin is biased (like $\alpha$) to $P(heads) = .51$. The uncertainty of the outcome is like $\beta$.

\paragraph{Betting} Betting works by betting on $N$ coins. If we win, we now have $2N$ coins. If we lose, we now have $0$ coins, so this is an even-money bet (you either gain $N$ coins or lose $N$ coins.)

\paragraph{The Casino} The casino has 1000 tables, each with a biased coin, and you have 1000 tokens, so you can bet them in any way you like: 10 tokens each on 100 tables, 1 token on each table, or 1000 tokens on 1 table. Once bets have been placed, the coins are all flipped in parallel, and for each game you either lose your chips or win.

\noindent So now the question is what scenario is going to net you the best outcome? Let's take the following two bets for example:

\begin{enumerate}
\item 1000 tokens on one table and 0 on the other 999
\item 1 token on each of 1000 tables
\end{enumerate}

\noindent Which is better? Or are they the same? In fact, the expected return of both bets are the same, but bet 2 is much less risky, as with bet 1, if you lose, you lose all of your money, but with bet 2, you might lose around half your money. In fact, the chance of losing all of your money (if you bet tails) is:

\begin{equation*}
(.49)^{1000} \approx 10^{-310}
\end{equation*}

\noindent To determine which is best, we need to consider risk and reward. In this case, the reward is our expected return. If $P_w$ is the chance we would win, and $P_l$ is the chance that we would lose, and $W$ is the amount we would win, whereas $L$ is the amount we'd lose, expected return for a single bet is calculated as follows:

\begin{equation*}
	E[R] = P_wW + P_lL
\end{equation*}

\noindent For the biased coin where we place all of our bets on one table, this would be:

\begin{equation*}
	E[R] = .51(\$1000) + .49(-\$1000) = \$20
\end{equation*}

\noindent If we placed 1 token on each table, the expected return would be:

\begin{equation*}
	E[R] = \sum_{i=1}^{1000} .51(\$1) + \sum_{i=1}^{1000} .49(-\$1) = \$20
\end{equation*}

\noindent So, in terms of reward, neither is better or worse. So how do we choose how to allocate the tokens? It turns out that the risk makes it easy to choose.\\

\noindent First, what's the chance that we lose it all? For the case where all of our tokens are on one table, the chance is 49\%. For the second table, it's around $10^{-308}\%$, which is quite a bit smaller...\\

\noindent Another way to look at the risk is by looking at the standard deviation of the bets. An example of the outcomes for situation 2 is:

\begin{equation*}
	-1,1,1,1,-1,-1,1,-1,...,1
\end{equation*}

\noindent The standard deviation of which is just 1. Now, for the case where we put all of our tokens on one table, the outcomes look like this:

\begin{equation*}
	1000,0,0,0,0,...,0
\end{equation*}
or
\begin{equation*}
	-1000,0,0,0,0,...,0
\end{equation*}

\noindent The standard deviation (risk) in both cases is $\sqrt{1000} \approx 31.62$, which is much higher than the standard deviation for putting bets on each table.

\noindent Now, we can create a risk-adjusted reward (Sharpe Ratio) for the single-bet case:

\begin{equation*}
	R_{s} = \frac{\$20}{\$31.62} = 0.63
\end{equation*}

\noindent For the multi-bet scenario, it's:

\begin{equation*}
	R_{m} = \frac{\$20}{\$1} = 20.0
\end{equation*}

\noindent Clearly, the second case wins based on this ratio. Something interesting about these results is that:

\begin{equation*}
	20 = .63\sqrt{1000}
\end{equation*}
\noindent It turns out that this can be generalized to 

\begin{equation*}
	{SR}_{multi} = {SR}_{single}\sqrt{bets}
\end{equation*}

\noindent Which shows that as we increase the number of bets (diversify), the Sharpe Ratio increases. This is the relationship described in the Fundamental Law of Active Portfolio Management; to increase performance, you can either increase skill or diversify (bets), although diversification only goes as the square root.\\

\noindent Now, back to equation~\ref{eq:inforatio}. Let's define what \textit{information ratio} means. If we consider the CAPM equation:

\begin{align*}
r_p[t]=\beta_p r_m[t]+\alpha_p[t]
\end{align*}

\noindent we can associate the first term, $\beta_p r_m[t]$ with the market, and the second term, $\alpha_p[t]$ with skill. Information ratio is defined as:

\begin{equation} \label{eq:inforatiodef}
IR = \frac{\overline{\alpha_p[t]}}{\sigma_{\alpha_p[t]}}
\end{equation}

\noindent Information ratio can be thought of as a Sharpe Ratio of excess return (due to skill). Now, the \textit{information coefficient}, $IC$, is the correlation of forecasts to returns. $IC$ can range from 0 (no skill) to 1 (perfect skill). $BR$, or breadth, is the number of trading opportunities per year. For example, if you are Warren Buffet, and hold only 120 stocks for a whole year, $BR$ is just 120. However, if you have 120 stocks and trade them daily, $BR = 120*365$.\\

\noindent Let's do an example: say that James Simons and Warren Buffet both have the same information ratio, and that Simons' algorithm is 1/1000 as smart as Buffet's. Buffet only trades 120 times per year. How many trades per year must Simons execute to have the same information ratio (performance)?

\begin{align*}
IR_S &= IC_S\sqrt{BR_S}\\
IR_B &= IC_B\sqrt{BR_B}\\
IC_S &= 1/1000IC_B\\
\frac{IR_B}{IR_S} &= \frac{IC_S\sqrt{BR_S}}{IC_B\sqrt{BR_B}} = 1\\
&= \frac{\frac{1}{1000}\sqrt{BR_S}}{\sqrt{BR_B}}\\
&\Rightarrow BR_S = (1000)^2BR_B\\
&= 120,000,000
\end{align*}

\noindent So Simons must execute 120 million trades, whereas Buffet only needs to execute 120. That's quite a difference! Indeed, skill is an extremely important factor in performance.

\section{Portfolio Optimization}
Now we wish to optimize a portfolio, and what this means is minimizing risk for a given target return. Risk is largely defined as the volatility of a stock. A portfolio is composed of some stocks that individually have their own return-risk ratios, but it is possible to weight them such that the return-risk ratio of the portfolio is higher than that of any individual stock. \\

This is done through combining correlated and anti-correlated stocks to highly reduce volatility. In the case of a highly correlated group of stocks, their combination results in a similar volatility, but if they're combined with highly anti-correlated stocks, then with accurate weighting, fluctuations cancel out and volatility is minimal while yielding similar returns. A useful algorithm to find the best weighting is \ac{mvo}. \textbf{*This algorithm is not explained, but we should find it*}. \ac{mvo} and similar algorithms find the minimal risk for a given target return, and if this is plotted over all target returns, we get a curve called the efficient frontier. On a return-risk plot, a line tangent to the efficient frontier with an intercept at the origin also points to the portfolio with the minimal Sharpe ratio.


==> introduction.tex <==
\chapter{Introduction}

The last decade has seen unprecedented growth in the deployment of Machine Learning (ML) based solutions, %(sometimes referred to as AI),
broadly influencing many aspects of our lives \cite{CNN2019}. %\footnote{See CNN 2019 article for more details -  \href{https://edition.cnn.com/2019/12/21/tech/artificial-intelligence-decade/index.html}{https://edition.cnn.com/2019/12/21/tech/artificial-intelligence-decade/index.html}} 
Significant progress has been made in machine learning tasks such as image recognition, language translation, and tasks related to self-driving cars, to name a few. With such prospects of potential success, the industry is attempting to apply ML to a variety of use cases at an unprecedented rate, including crime prevention, medicine, IT and cloud analysis, cyberspace security, intelligent chatbots, and many more. %various "AI agents" that provide services in various domains.  


ML-based systems combine ML models and regular software to achieve some common goal, e.g., making the driving decisions of the self-driving car. But what are ML models? ML models can be thought of as regular computer programs that were produced by automatically searching over some predefined set of possible programs.  The search is guided by examples of the desired program behavior.  We usually refer to the examples as the training data or simply as data.  Thus, just as we teach young children by example, in the case of ML models, we provide the machine with examples from which it learns the correct behavior; hence, the name machine learning.    


ML models are statistical by design. We do not expect to find an ML model that is always correct.  In fact, we are unlikely to know whether the space of possible models that we search in contains such a perfect model, and even if it does it may be too difficult to find.  Instead, we settle for the model being correct most of the time.  In addition, we require that a successful model will be correct most of the time on unseen data of the same type as the data it was trained on.  %We call this desired trait generalization.  
This trait is commonly referred to as {\em model generalization}. Thus, a bug in an ML model usually cannot be determined from the individual response of the model to a single data point; rather, it is determined by the aggregated behavior of the ML model on many examples. As a result, an ML solution composed of several ML models and regular software can only be successfully crafted if it is validated by statistical experiments.   It also means that the required behavior of an ML solution can only be defined as an aggregate of its behavior on individual data points. Therefore, the control of the aggregated statistical behaviour of the crafted ML system as a whole is indeed a major challenge addressed in this book. The average aggregate behavior and its control can be exemplified in the case of a self-driving car. For example, we can specify that the desired average number of wrongly recognized type of vehicle is no more than 5\%.

With this in mind, we emphasize the need for well-defined quantitative measures that reflect the desired behavior of the ML-based system. An example of such a measure is the average number of service calls a chatbot, whose goal is to address those calls autonomously, is routing to a human service agent. Such measures can be derived from {\em statistical functional requirements} hence denoted {\em statistical functional measures} or SF measures in short. Once SF measures are properly defined, one can utilize them to analyze the desired behavior of the system. As described in this book, this analysis can be performed via appropriately designed statistical experiments that estimate the expected average and variance of the SF measures. A good experiment should provide accurate estimates of the SF measures when the ML-based system is deployed. This practice of defining SF measures and designing experiments that test them throughout the life-cycle of the ML-based system tackles the challenge of crafting an ML-based system that meets its requirements. 

Collecting a set of training examples for a given SF requirement is challenging too. The data may be lacking factors without which the desired model cannot make correct decisions. We might have too few examples, or examples that are not representative of the type and distribution of data that the system will encounter when deployed. %the model is applied.
Finally, in order to guide the learning, the data needs to include the "correct answer" as well as indication that it is indeed correct. Such indication is typically provided %refer to that as
by labeled data, in which case the problem is a supervised learning problem. However, it often happens that an organization holds a representative set of examples that is readily available but are not labeled.  

As suggested above, this book aims to address the challenges of crafting robust ML solutions that meet their design requirements and in particular SF requirements, and hence can be confidently deployed. We focus on an experimental approach to the crafting of ML solutions. This approach can be thought of as the ML equivalent of the test-first approach applied to regular software. To emphasize this similarity, we name our approach {\em experiment-first}. The focus of this approach is on crafting, validating, and continually monitoring ML-based solutions via a series of carefully designed experiments at different levels of abstraction. The book is self-contained and addresses the mathematical and statistical techniques needed to apply the experiment-first approach.  It contains numerous practical programming as well as theoretical exercises and their solutions. Exercises are an integral part of the text and are designed to facilitate understanding of the ideas, concepts and methods introduced. 

The main target audience of this book is data scientists who craft ML-based solutions, architects who define what the solutions need to do, and testers who need to validate that the system actually works and meets its specifications. The book also attempts to bridge communication gaps between the stakeholders involved in the development of ML-based solutions. The experiment-first approach introduced in this book facilitates an end-to-end, unambiguous, quantitative definition of the steps to be taken in the development of an ML-based system. Our approach details the activities performed, and the artifacts consumed and generated, throughout the development and deployment of the solution. 
The book introduces the statistical experiment and its results as the language by which the stakeholders communicate effectively to craft the ML-based solution.        

A preferred way to design and implement experiments entails following a scientific experimental methodology. This methodology includes the definition of a problem, the formulation of a quantitative conjecture, and the design and implementation of an experiment that validates or rejects the conjecture.  For example, a problem could consist of finding the speed at which a ball will touch the ground when dropped from a high tower.  The conjecture is that the speed is proportional to the time, and the experiment involves dropping balls from towers of different heights and measuring how long it takes them to hit the ground. 

This book is organized as follows. In Chapter \ref{Chapter:scientific-method} we paint in broad strokes the scientific experimental methodology and highlight its applicability %relation 
to ML system development and validation. As mentioned in the previous paragraph, following the scientific methodology includes defining a problem, making a conjecture about how the problem may be solved, and then designing and implementing an experiment to validate the conjecture.  When crafting an ML-based solution, the standard conjecture entails generalization, namely, that the system will behave as required on new inputs not seen before.  The problem that the conjecture implicitly aims to solve is being able to construct an ML-based system that meet the requirements on new data.  After defining the requirements we address specifics of how to formulate a generalization conjecture and how to craft the appropriate experiment to validate it and analyze the results in the event that the conjecture was wrong. We also discuss %highlight 
the way in which the results of the experiments influence system design and contribute to the continual monitoring and validation of the system throughout its life-cycle.  

Then, Chapter \ref{mindDirect} details practical aspects of the experiment-first methodology. They are described as a set of best practices and pitfalls that aim to quickly reduce the risks associated with the development of the ML-based system and help address the most important concerns first.  Practices proposed in Chapter \ref{mindDirect} should allow stakeholders to better validate, from day one, the potential for successful generalization given the business requirements and data. The practices should additionally identify optimal usage of information extracted from the data and application of the most suitable ML techniques to the problem at hand. % It is highly beneficial to repeatedly come back to these practices with teams as they are applied in practice.  

When analyzing ML models, the focus is sometimes on generic performance measures, e.g., the accuracy of the model. In contrast, an ML-based solution has unique, specific SF requirements. For example, a service chatbot may be required to autonomously handle at least $90\%$ of its conversations with customers, and send at most $10\%$ of to a human service agent for processing. In addition, specific requirements are frequently realized through the interaction among ML models and regular software.  Chapter \ref{unitSystem} discusses the composition of ML software and regular software in a unified ML-based system, and how such composition impacts system validation.


The next two chapters on ML testing before deployment (Chapter \ref{Chapter:MLtesting}) and on drift (Chapter \ref{Chapter:drift}) address the system correctness concern at different phases of the system life cycle. The ML testing chapter focuses on checking system correctness before it is deployed, while the chapter on drift detection analyzes whether the system operates correctly once it is deployed.  

%As the basic 
Generalization is a fundamental conjecture made about ML-based system correctness. % entails the generalization of some measure, e.g., the volume of service calls that were sent to a human agent in a chatbot scenario, 
Thus, the experiments performed at testing time should indicate %project 
that the desired behavior will manifest once the system is deployed. Due to the stochastic nature of ML-based systems, the validation typically includes a stability assertion %claim.  A claim 
An assertion could suggest, e.g., that on average, 5$\%$ of the service calls received by a service chatbot are diverted to a human service agent, but it is unlikely that more than 10$\%$ of the calls are diverted. 
As data changes over time the system might fail to meet the desired behavior once it is in operation, even if it was well built and tested. For example, in the chatbot scenario, changes in the type of service calls might result in much more than 10$\%$ of the calls being diverted to a human agent. To handle this, drift detection is required. This topic is addressed in Chapter \ref{Chapter:drift}.  

Once the expected system behavior is established, we can define an optimal business process. % that is based on the system expected behaviour.  
In the chatbot example, once we know that up to 10$\%$ of the service calls are diverted to a human agent, we can plan the size of the customer service team that will provide proper response to the diverted calls. The integration of ML-based system behavior with the business process is discussed in Chapter \ref{optimal}. Finally, 
%
in Chapter \ref{industrial}, we present an industrial example to demonstrate the implementation of principles of the experiment-first methodology in practice.
%
Solutions to exercises that appear across the book. Code samples and mathematical background are found in the appendix. 

This concludes the description of the content of this book. It is important to note that the book does not cover topics such as generic trust-related measures and MLops. %We elaborate on this below.  
%
ML models learn from data. Hence, their inferences may be affected by data bias and adversarial manipulation. %For example, gender bias in the ML model may result when learning from historical data. In addition, data can be manipulated by attackers to change the learning results. 
Some ML models can be trusted only if their decisions are comprehensible. %This concern is especially prominent in the legal context. For instance, a court of justice may require an explanation of the rationale behind a decision made by the ML model.
Much research addresses these concerns \cite{trust}, \cite{RSG2016}.
%
%The above concerns are sometimes collectively referred to as trust concerns. This book does not focus on trust concerns. %directly. Instead, when following the experiment-first methodology, the appropriate set of trust concerns that are relevant to the ML solution at hand will naturally surface as the system requirements are defined. This will then lead to the design of experiments that address these trust concerns. 
%At that point, it is advisable to apply state-of-the- art techniques related to trust and model readability\cite{10.1145/2939672.2939778}. 
%
%The book additionally does not address %
Low-level engineering concerns (e.g., automatic model re-training) are out of scope too, %, saving the data that was used for training, and tracing it to the model that was obtained from the training. These topics are well covered in the literature (see, 
and are well covered in the art (e.g., MLops tutorial \cite{MLops}). 
% \href{https://towardsdatascience.com/get-started-with-mlops-fd7062cab018}{\underline{see tutorial on MLops.}}. XX-Onn


  
  

==> mathBackground.tex <==
\chapter{Mathematical Background}

This appendix covers mathematical and statistical background which facilitate the understanding of the main text and ML in general. 

\section{Optimization}

Optimization is at the heart of ML. Typically ML algorithms solve some optimization problem.  We will give examples of such optimization problems in other sections of this appendix.   

We first consider a general optimization setting and describe a pattern of numerical optimization algorithm that will apply to most of our optimization problems.  

Assume $x_n \rightarrow x$ in $R^n$ and that $x_n = A^{n-1}(x_1), n=2,\ldots$.   Further assume that $A: R^n \rightarrow R^n$ is continuous.  The target of our optimization is some $O \subset R^n$.
Assume we have some function $Z : R^n \rightarrow R$ such that $Z(A(x)) < Z(x), x \in R^n - O$ and $Z(A(x)) \leq Z(x)$ for $x \in O$ then we have the following.

\begin{lemma}
Under the above assumptions $x \in O$
\end{lemma}
\begin{proof}
$x_n \rightarrow x$ therefore $A(x_n)$ which is $x_2, x_3, \ldots$ also converges to $x$.  But as $A()$ is continuous $A(x_n)$ also converges to $A(x)$.  Thus, $A(x) = x$.   As a result it is not true that $Z(A(x)) < Z(x)$ therefore $x \in O$. 
\end{proof}

$Z()$ is a descending function that guide the search for an element in $O$. in practice it could be the function itself for which we are seeking a minimum but it could also be the and other monotonic descending function.  Another choice we will use many times is a direction in which the gradient of the function is descending.    

\begin{figure}[h!]
\centering
\includegraphics[scale=0.5]{images/contractionConvergence.png}
\caption{When does a descending sequence converges to the optimum?}
\label{fig:universe}
\end{figure}

\begin{exercise}
In the above proof we use the fact that removing a finite number of elements from a converging sequence does not change its limit. We study this below.
\begin{enumerate}
    \item $1, \frac{1}{2}, \frac{1}{3}, \ldots \rightarrow 0$ but what about $\frac{1}{2}, \frac{1}{3}, \ldots$. Explain why. 
    \item $a_n \rightarrow a$ means that for all $\epsilon > 0$ there exist a $N_{\epsilon}$ so that if $n > N_{\epsilon}$ then $|a_n - a| < \epsilon$.  Prove that if $a_n \rightarrow a$ so that the sequence $b_1 = a_k, b_2 = a_{k+1}, \ldots$ for any $k > 0$.
    \item Can you modify the above proof to work for the removal of any finite set of elements from a converging sequence? That is if $a_n \rightarrow a$ and a finite set of elements is removed from $a_n$ to obtain $b_n$ then $b_n \rightarrow b$.
\end{enumerate}

\end{exercise}

\begin{exercise}
Consider the following process.  Given $f(x) = x^2$ we would like to find the root $f(0) = 0$ by starting from some pair of points $(x, -x), x > 0$.   We define the following process $a1 = (x, -x)$.  Given that $a_n = (a_n^1, a_n^2)$ if $(\frac{a_n^1+a_n^2}{2})^2 > 0$ then $a_{n+1} =(\frac{a_n^1+a_n^2}{2}, a_n^2)$ else $a_{n+1} =(a_n^1, \frac{a_n^1+a_n^2}{2})$.
\begin{enumerate}
    \item Define $A()$ and $Z()$ in this case.
    \item What happens to $Z()$ at $(0, 0)$.   What happens to $Z()$ at $(a, b)$ for which $a>0, b<0$
    \item Prove that for any $n$ $a_n^1 = -a_n^2$.
    \item Is $A()$ continuous?
    \item Write a program that implements the above numeric algorithm and check that it works (finds the root of $f(0) = 0$).  Generalize for any $f()$.
\end{enumerate}
\end{exercise}

\section{Probability}
\label{probability}

Here, we describe and show notation for probability concepts used in this book.

\subsection{Random Variables and Distributions}
\label{ssec:random_variables}

Random variables are introduced in Section~\ref{randomVariable}.  Here, we explain the concept in a less-mathematical way.  A variable (often denoted by a capital letter, e.g., $W,X,Y,Z$, etc.) or `feature' is a an object that can take a value.  For instance, $W$ may take any value in $\{1,2,3,4,5,6\}$, $X$ any real number between $[0,1]$, $Y$ any value in  $\{\splitatcommas{\textrm{Afghanistan},\textrm{Albania},\dots,\textrm{Zimbabwe}}\}$, and $Z$ any non-negative integer $\{0,1,2,3\dots\}$.  Here, $W$, $X$, and $Z$ would be considered numeric, and $Y$ would be categorical (see e.g., \cite{LSHGOZ2003}, page 28).  In addition, $W$ and $Z$ are discrete, and $X$ is continuous. 
Random variables are particularly useful when they represent real measurements.  For instance, $W$ may represent the result of a die being rolled, $X$ can be any potential probability value (which must be between 0 and 1), and $Y$ is a person's native country, and $Z$ can be the answer to the question `how many children do you have' (none or any positive integer).

A random variable also has a distribution associated with it, which determines the probability or likelihood of the variable taking each of the potential values.  For instance, letting $P$ denote `probability' we can speak of $P(Y=\textrm{Germany})=0.1$ or $P(0.1\leq X\leq 0.134)=0.2$, for example. Each of these specific or range of values is known as an `event'.  The probabilities are often calculated from a (random) sample of values of the variable (e.g., the native countries of a random sample of individuals; see \cite{LSHGOZ2003}, page 20--25).  Specific values of the variable are often denoted with lower-case letters (e.g., $w,x,y,z$).  So, for instance, we may consider $P(Z=z)$ for each of $z\in\{0,1,2,3\}$.

Distributions are often denoted $p$ or generality; thus we can use the shorthand $p(X)$ and $p(Y)$ to denote the distributions of $X$ and $Y$.  Distributions of numeric variables often have shapes that can be described by summary statistics (see \cite{LSHGOZ2003}, pages 131--153) such as mean, median, variance, kurtosis, etc.  Categorical variable distributions can be be visualized by bar  charts (see \cite{LSHGOZ2003}, page 101).

\subsection{Joint Distributions}
\label{ssec:joint_distributions}

The joint distribution of two or more variables is the probability of both variables taking specific values simultaneously.  Here, we will only illustrate joint distributions for two variables.  For instance, using the shorthand above, $p(X,\:Y)$ is the joint distribution of $X$ and $Y$.  For instance, letting both $X$ and $Y$ be categorical variables, where $X=\begin{cases}1, &\text{person speaks Spanish}\\0 &
\text{otherwise}\end{cases}$ \qquad and $Y$ being their native country, $p(X, Y)=P(X=x,Y=y)$ is the joint distribution.  Thus $P(X=1,Y=\textrm{Spain})$ is the probability (in a given sample or population) that a person both is from Spain and speaks Spanish.  This probability is zero if there are either no people from Spain, no Spanish speakers, or no people who fulfill both conditions (even though there may be, say, Spanish speakers who are not from Spain).

If both $X$ and $Y$ are numeric, a scatter plot can be used to visualize the joint distribution (see \cite{LSHGOZ2003}, pages 165--169).  Otherwise, except for particular cases (e.g., multivariate normal), the distribution is hard to characterize in a closed-form expression. 

A conditional probability (see \cite{LSHGOZ2003}, pages 194--197) is denoted $P(X=x\mid Y=y)$, which likewise yields a conditional distribution $p(X\mid Y)$.  The variable conditioned on ($Y$) is to the right of the vertical bar, and the variable whose probability is calculated given the conditional ($X$), is on its left.  This means that to calculate the probability, the sample is first restricted to values of the conditioning variable ($Y$) satisfying a condition.  For instance, consider $P(X=1\mid Y=\textrm{Spain})$.  Thus, we first consider only people whose native country is Spain; among these, we calculate the probability that a person speaks Spanish.  This probability is likely nearly 1 because there is a strong association between these two features (nearly all people from Spain speak Spanish), which is very different from the un-conditional joint probability above.

We note that a joint distribution can be decomposed into a product of a conditional and a univariate distribution.  For any variables $X$ and $Y$, $p(X,Y)=p(X\mid Y)p(Y)$.  Since the ordering of variables in the joint is arbitrary, we can also say that $p(X,Y)=p(Y,X)=p(Y\mid X)p(X)$.  That is, for instance, to determine the joint probability $P(X=1, Y=\textrm{Spain})$ we could first calculate $P(Y=\textrm{Spain})$ (likely small), then calculate the conditional probability of speaking Spanish given that one is from Spain (nearly 1).  Or, we could first calculate the probability $P(X=1)$, then calculate the probability of being from Spain (as opposed to, say, Argentina, Mexico, or any other country) among Spanish speakers.  Either way is equivalent.

We noted above that $X$ and $Y$ in this example have a strong association; that is, a person from Spain is more likely than a random person to speak Spanish, and a Spanish speaker is more likely than a random person to be from Spain.  Such an association whereby knowing, say, the value of $Y$ impacts the probability of $X$ being a particular value is called dependence, and lack thereof is called independence.


\subsection{Independence}

\begin{definition}
Two events A and B are independent if $P(A \cap B) = P(A)P(B)$.
\end{definition} 

We next define independence of two random variables.  
\begin{definition}
Two random variables X, and Y are independent if any pair of events $A_X$ and $B_Y$ defined by X and Y respectively are independent.
\end{definition}

\begin{example}
If X defines the height and Y the weight of people then an event defined by X may be $A_X = \{180 cm \le X \le 190 cm\}$ and an event defined by Y may be $B_Y = \{70~ kg~\le X \le 80~kg\}$.  Saying that X and Y are independent will mean that $P(A_X \cap B_Y) = P(A_X)P(B_Y)$.  The same forum la will hold for any two events $A_x$ and $B_Y$ you can define by X and Y.
\end{example}

\begin{exercise}
Are X and Y in the example above intuitively independent?  Explain your answer. 
\end{exercise}


When the two variables are independent we have that the average of their products is equal the product of their average, i.e., $E(XY) = E(X)E(Y)$.  We prove this for the case in which both variables have a finite set of values.  A similar proof holds when the number of possible values is countable (infinite but can be described as a series) or if the random variable is continuous.  In the latter and integral is used instead of a sum to obtain the proof.

Assume X may obtain values $x_1, \ldots x_n$ with positive probability and Y may obtain values $y_1, \ldots, y_n$ with positive probability.  In that case by definition $E(XY) = \sum_i \sum_j x_i y_j P(X = x_i \cap Y = y_j)$
Using the independence of X and Y we get $ = \sum_i \sum_j x_i y_j P(X = x_i)(Y = y_j)$
In the inner sum $x_i$ and $P(X = x_i)$ are constant thus we get $ = \sum_i  x_i P(X = x_i) \sum_j y_j  (Y = y_j)$
next we identify the average of Y as the inner sum thus
$ = \sum_i  x_i P(X = x_i) E(Y)$
but now $E(Y)$ is a constant so we get 
$E(Y) \sum_i  x_i P(X = x_i)$
which is clearly equal to
$= E(X)E(Y)$.  This completes the proof that $E(XY) = E(X)E(Y)$.

\subsection{Controlling the number of defects in a production line}
\label{parametricControl}

Consider a production line that produces a series of identical items.  Each item can be either defective or not.  We want to control the percentage of defected items.  We model the situation parametrically using a series of Bernoulli variables $X_i$ with probability of having a defect p.  For a batch of n items the production lines produced, inspection may yield k defected items.  We want to set our expectation about the production line. Fixing a small probability $\alpha$ we want to understand when seeing k or more defects has probability $\alpha$.   In other words, we would like to determine when the probability of the number of defects being greater than k for a batch of n items is $\alpha$ under the assumption that the probability of seeing a defected item is p.   If we then see more than k defects in a batch of n items we will say that the interpretation of the production line as a system that produces defect in probability p is no longer reasonable as we are seeing an unlikely number of detects (bigger than k).  We will take some action such as stooping the production line and re-collaborating its parameters.  In such a case we will say that the production line is "out of control".

We next formally capture the above reasoning. We require that $P(t \ge k) = \alpha$.   As the probability of t defects is $\binom{n}{t}p^t(1-p)^{n-t}$ we get that the probability of seeing more than k defects is $\sum_{t \ge k}\binom{n}{t}p^t(1-p)^{n-t}$.  We thus are interested in finding k so that $\sum_{t \ge k}\binom{n}{t}p^t(1-p)^{n-t} = \alpha$.  

\begin{exercise}
\label{excercise:a22}
Write a code that finds k. Play with different values of n, k, and $\alpha$ to gain an intuition on the value of k.  Is there a computational limitation to the calculation of k when n is large?

\href{https://colab.research.google.com/drive/10-2OR1zBRtrjNr52WvvU3r2MDEbLbpog?usp=sharing}{Click here for solution} or see solution \ref{excercise:a22_sol} in  appendix \ref{chapter:solution_appendix}.

\end{exercise}



\section{Bayesian Networks}

Recall that any joint distribution $P(X_1, \dots, X_n)$ of the random variables $X_1, \ldots, X_n$ can be factored in the following way $P(X_1, \dots, X_n) =  P(X_n|Z_1, \ldots, X_{n-1}) \times \ldots \times P(X_2|X_1) \times P(X_1)$.  The order of the factoring is arbitrary chosen thus any order may be applied.

\begin{example}
\label{BN1}
Assume the following four Boolean random variables: $R$ for whether or not it rained, $SH$ for whether or not the car was washed, $W$ for whether or not the floor is wet and $S$ for whether or not someone has slipped. The following factorization of the joint distribution applies $P(R, SH, W, S) = P(R|SH,W, S)\times P(SH | W, S)\times P(W|S) \times P(S)$.  Intuitively, this means that for any possible values of the variables say $R = true, SH = true, W = true, S = false$ we can calculate the probability $P(R = true, SH = true, W = true, S = false)$ by calculating $P(R = true |SH = ture,W = true, S = false)\times P(SH = true | W = true, S = false)\times P(W = true|S = false) \times P(S = false)$ or calculating the probability that we did not slip, multiplied by the probability that the floor is wet given that we did not slip, and so on. 
\end{example}

\begin{definition}
We say that a random variable X is independent of a random variable Y if $P(X, Y) = P(X) \times P(Y)$.  As $P(X, Y) = P(X) \times P(Y|X)$ we also get that in such a case $P(Y | X) = P(Y)$.   Similarly $P(X | Y) = P(X)$.
\end{definition}

A Bayesian network (BN) captures the independence and dependence between random variables.  One simple view of a BN network is the corresponding factorization of the joint probability of random variables $V = \{X_1, \ldots, X_n\}$ that it represents.   

\begin{definition}
Assuming that we are given a DAG with vertices $V = \{X_1, \ldots, X_n\}$ and a set of edges E.  We will say that $(V, E)$ is a BN if $P(X_1, \ldots, X_n) = \prod_{i} P(X_i| parents(X_i)) $ where $parent(X_i) = \{X_j | (X_j, X_i) \in E\}$.   
\end{definition}

\begin{example}
\label{BN2}
Revisit example \ref{BN1} above.  Set $V = \{R, SH, W, S\}$ and $E = \{(R, W), (SH, W), (W, S)\}$.  Interpreting (V, E) as a BN we obtain that $P(R, W, SH, S) = P(S | W) \times P(W | R, SH) \times P(SH) \times P(R)$ which is intuitively an appealing factorization.     
\end{example}

\begin{exercise}
what are the Independence assumption Incorporated in the BN representation of example \ref{BN2}.  Hint - write down an appropriate gunnel factorization and use independence assumptions to achieved the factorization represented by the BN.  
\end{exercise}

\begin{lemma}
We are given a BN with three variables, X, Y, and Z and edges $(X, Z), (Y, Z)$. We next show that in such a case X and Y are independent.
\end{lemma}
\begin{proof}
$P(X, Y) = \sum_{z} P(X, Y, Z) = \sum_{z} P(z | X, Y)\times P(Y)\times P(X) =  P(X) \times P(Y) \times \sum_{z} P(z | X, Y) = P(X) \times P(Y)$.   The last inequality is valid as $\sum_{z} P(z | X, Y) = 1$, i.e, $P(Z | X, Y)$ is a distribution probability over the values of Z given some specific values of X and Y.
\end{proof}


\section{Decision Theory}

Chapter \ref{optimal} discusses the interface of the ML embedded system with the business process. As the ML embedded system is non deterministic, we are not certain if its output is correct or not. Dealing with such uncertainties is at the heart of decision theory which we introduce next.  

In decision theory a decision maker is given a set of alternatives or actions A she needs to choose from.  In addition, a possible set of states of the world, S, is given but the decision maker does not know which of the states in S holds.  Once the decision maker chooses an $a \in A$, and given that the unknown to the decision maker state of the world is $s \in S$, the decision has a loss $l(a, s)$.

What decisions would we consider to be rational?  A conservative approach to the problem should assume the worst; given that the decision maker takes the action a, we then check what is the maximal possible loss in this case.  In other words, we calculate $l(a) = max_{s \in S} l(a, s)$. Next, we determine for which action, $a \in A$, the worst possible loss, l(a), is minimal. We thus find the action, $a_0$, such that $a_0 = argmin_{a \in A}~l(a) = argmin_{a \in A}~max_{s \in S}~l(a, s)$.   This is sometimes called the $minmax$ principle and is conservative as in reality there is no adversary who is attempting to force the worst possible loss on the agent given the agent's action.

Another approach is to assume some distribution of the states S representing the likelihood of each state.  Given such an assumption the expected loss of the decision maker when taking an action a is  $l(a) = E(l(a, s))$.  It is then rational for the decision maker to choose an action that minimizes $l(a)$.  This is sometimes referred to as the Bayes rule.

\begin{example}
Consider a decision problem with two actions $A = \{a, b\}$.  we are given that if b is chosen the states of the world is determined and the loss is 1.   If a is chosen, the state of the world is not determined and is some number $0<s<1$.  If the state of the world is actually s, the loss is 2s. Following the $minmax$ principle, we get that l(a) = 2 and l(b) = 1 and it is rational for the decision maker to chose b.  If the decision maker assumes a uniform distribution over the possible values of s, then on the average the decision maker will loss 1 given she chosen a and she is indifference between the choices a and b. 
\end{example}

\begin{exercise}
In the previous example, assume that the decision maker is given the average and standard deviation of the distribution on as and models the distribution as the Beta distribution.  what will be the decision of the decision maker for various values of the average and standard deviation of the distribution s?
\end{exercise}

\begin{exercise}
Assume a binary classification and its associated confusion matrix. Can you define the Bayes rule associated with it and explain how it will be used to define the the usage of the classifier?
\end{exercise}

\href{https://www.youtube.com/watch?v=ztsGe4gOJJk&ab_channel=MLworkshop}{Click for YouTube recording on this topic}
\\



\section{Machine learning}

\subsection{Machine learning techniques}

\subsubsection{Hard support vector machine}

A binary classifier is obtain on data in $R^n$.  We first assume that there is a hyper plane that separates the training set to two different classes. This is referred to as hard support vector machine.  In the next subsection we relax that assumption. 


More precisely given a training set $(x_1, y_1), \ldots, (x_m, y_m)$ that was sampled i.i.d. such that $x_i \in R^n$ and $y_i \in \{-1, 1\}$ we assume that there exist a hyper plane $(w, b), w \in R^n, b \in R$ such that $(w, x_i) + b > 0$  if and only if $y_i = 1$.   Here $(w, x_i)$ is the scalar multiplication of w and $x_i$.   

Figure \ref{fig:hardSVM} represents the situation in $R^2$.  In the figure, the plus sign stands for the label 1 and the minus sign represents the label -1. 
\begin{figure}[h!]
\centering
\includegraphics[scale=0.5]{images/HardSVM.jpg}
\caption{A hyper plane exists that separates the positive and negative examples.}
\label{fig:hardSVM}
\end{figure}

A separating hyper plan is used as a classifier by calculating $(w x)+b$ on a new point $x$.   If the result is positive we say that the label 1 otherwise that the label is $-1$.

We would like to choose a separating hyper plane that will be as resilient as possible to noise.  Consider figure  \ref{fig:hardSVMnoise}.  Hyper plane $l_2$ is more sensitive to noise as it is closer to points in the data set.  If the points $l_2$ is close to change a bit due to noise, their classification by $l_2$ will change.  In contrast $l_2$ is more "in the middle" of the gap between the set that is positively labeled and the set that has negative label.   Thus, $l_1$ is less sensitive to noise. This intuition is captured in the following hard support vector machine optimization problem.

\begin{figure}[h!]
\centering
\includegraphics[scale=0.10]{images/hardSVMnoise.jpg}
\caption{$l_2$ is more sensitive to noise than $l_1$.}
\label{fig:hardSVMnoise}
\end{figure}

Denote the distance between the hyper lane $(w, b)$ and a point $x$ by $d((w, b), x)$.  We would like to find a hyper plane such that the closest point from a point in the training set to it will be as far away as possible.  In other words a hyper plane such that $max_{w \in R^n b \in R} min_{x_i, i = 1, \ldots, m} d((w, b), x_i)$.

\begin{exercise}
What is a hyper plan on the line?  Create a sample of points from the line as follows.  With equal probability randomly choose from normal distribution with average 0 and standard deviation 1 or from normal distribution with average 2 and standard deviation 1.  Obtain a sample of size 100.  Was the sample separable?  Repeat the process a few times.  Did the answer change?  Next change the average of the second distribution to 4, 8, 16, 32.   Did you get a separable sample in these cases?    
\end{exercise}

\begin{solution}
Solution to exercise


\definecolor{LightGray}{gray}{0.9}
\begin{minted}
[
frame=lines,
framesep=2mm,
baselinestretch=1.2,
bgcolor=LightGray,
fontsize=\footnotesize,
linenos
]
{python}

# Imports
%matplotlib inline
import numpy as np
import matplotlib.pyplot as plt

### The is the random function. 
# It generates n samples.
# Each samples has 50-50 probability to be taken from Distribution # 1 or Distribution 2.

def rand(n=10, avg_1=0, avg_2=2, std_1=1, std_2=1):
  r1 = np.random.normal(avg_1, std_1, size=n)  # N samples from dist. 1
  r2 = np.random.normal(avg_2, std_2, size=n)  # N samples from dist. 2
  c1 = np.random.choice([0, 1], size=n)  # Determine which samples will be taken from dist. 1
  c2 = 1 - c1  # Determine which samples will be taken from dist. 2
  r = (r1 * c1) + (r2 * c2)
  return r
  
### First experiment
# We randomize 100 samples from the function defined above and plot # the histogram we see. 
# 
# We repeat 5 times.

repeats = 5
samples_per = 1000
means = [0,2]
fig, axs = plt.subplots(1, repeats,figsize=(50,10))

for i in range(repeats):
  avg_2 = means[1]
  r = rand(n=samples_per,avg_2=avg_2)

  n_bins = 80
  ax = axs[i]
  # We can set the number of bins with the *bins* keyword argument.
  ax.set_title(f"(# {i+1})Histogram of points (mu1 = 0 , mu2 = {avg_2})")
  _ = ax.hist(r, bins=n_bins)
# See plots in the first figure below
  
### Second experiment
# We randomize 1000 samples from the function defined above and
# plot the histogram we see. 
# 
# We test what happens when the first distribution is always (0,1), but the second
# distribution can have a mean of [4,8,16,43].
# We repeat 4 times for each mean.
#
# We can see that the bigger the difference between the means,
# the easier it is to distinguish the two distributions.

repeats = 4
samples_per = 1000
second_means = [4,8,16,32]
fig, axs = plt.subplots(len(second_means), repeats,figsize=(50,8 * len(second_means)))

n_bins = 80
for j in range(len(second_means)):
  second_mean = second_means[j]
  for i in range(repeats):
    r = rand(n=samples_per,avg_2=second_mean)

    ax = axs[j,i]
    # We can set the number of bins with the *bins* keyword argument.
    ax.set_title(f"(# {i+1})Histogram of points (mu1 = 0 , mu2 = {second_mean})")
    _ = ax.hist(r, bins=n_bins)
    
# See plots in the second figure below

\end{minted} 
\end{solution}

\begin{figure}[h!]
\centering
\includegraphics[width=\textwidth]{code_examples/code_imgs/a52_first.png}
\caption{5 repeats of joint distribution of two normal dist. with mu1=0,mu2=2}
\label{fig:code_a522_1}
\end{figure}

\begin{figure}[H]
\centering
\includegraphics[width=\textwidth]{code_examples/code_imgs/a52_second.png}
\caption{Each row represents 4 repeats of the histogram of a joint distribution of two normal dist. with constant Mu. where mu1=0 in all of them, and in rows 1-4 the second mu is 4,8,16,32 respectively}
\label{fig:code_a522_2}
\end{figure}

\href{https://colab.research.google.com/drive/1bvXVLMZO27egVnzCN7oLpa36P6nyKevE?usp=sharing}{Click here for code}
\\

TBC - change to optimization problem due to the use a formula of the distance between a point and the plane

TBC - change to optimization problem to make it convex

TBC - Stress that this is an example of a ML related optimization problem.








==> mindDirecting.tex <==
\chapter{Pitfalls and Best Practices for the Machine Learning Designer and Tester}
\label{mindDirect}

%\section{Overview}

%We are in the middle of the AI and data revolution.  Companies are attempting to utilize data and realize business value. 
%"Data insight" is an old-fashioned application of AI that does not recommend actions.  However, businesses today want to trust AI in their decision making with and even without a human in the loop. This requires the creation of a business-grade reliable and trustable ML solution (or AI-infused solutions).  

There are many good resources on ML technology as well as good courses on theory and algorithms.  We are not attempting to fill that need; if we were, we would be presenting Yet Another Machine Learning Machine or YAMLM.   Instead, this chapter highlights best practices and pitfalls in the development of a ML based system.  Following the best practises and avoiding the pitfalls presented in this chapter will increase the chance that your ML based system is successfully developed.  The practices introduced in the chapters align, support and enhance the experiment first approach in several ways, namely, they either encourage the implementation of an experiment, highlight its value, emphasis that an experiment that should have been implemented can not be implemented for some reason or point to to a non trivial idea that leads to the design of a useful experiment.  The reader is encouraged to examine each practice in that light and actively attempt to find "the hidden experiment" in the description of the practice.   


\section{From day one determine if the data is relevant to the business objective}

Deciding which business objective to implement  depends on the data.  The happy marriage of business requirements with relevant data is the determining factor in creating a high quality ML based system. It is a waste of time to discuss the solution in isolation from the data and without directly inspecting and analyzing it to determine whether the business goal may be achieved.  However, it may be useless to learn whatever is possible to learn from the data as such learning, even if successful, may not serve any useful business goal.

Once a business objective is established, the data can be inspected to determine if it contains information relevant to the business objective.  For example, a court may decide on the custody of a child in a divorce case.  One may establish in initial discussions that the business objective is to recommend which parent will have custody of the child.  It was also established that the data used for learning will be expert reports nominated by the court. 

Following the experiment first approach it is useful at this point to try and identify factors that impact the court decision.  Such factors may include\footnote{The interested reader may find the risk factors detailed here \cite{https://doi.org/10.1111/fcre.12134} instructive.} - 

\begin{itemize}
\item The country the court resides in and within the US, the state as well
\item The type of the court
\item The professional background of the expert evaluator
\item Criminal records of the parent
\item Mental health issues of the parent
\item Mental health issues of the child
\item Steady income of the parent
\item Attachment of the child to the parent
\item The language in which the report is written
\end{itemize}

Such factors may be established through interviewing of subject matter experts involved in the design of the ML based system.   Once a set of factors is established the data may be further analyzed to determine if the factors are represented and lack bias. For example, we may find out that the DB of court ruling includes only court ruling from the UK and from the state of NY for cases in which the child had some sort of mental health disorder.  The chances of training a ML based system that will correctly rule for a court case in California with a child that does not have mental issues are slim.  We say that it is less probable that the data has a signal for a child with no mental health disorder in California.   Thus, an initial factor analysis and further analysis of data bias help setup the expectation of what can be learned from the data and under which conditions the learning will apply.  This first step should be further refined into a full blown experiment design that will help establish the validity of the ML based system throughout its development cycle.  

Another aspect to be tackled at this point are simple rules that most likely apply to the system.  Such rules can be used as baseline to enhance the experiment design and provide necessary conditions for the validity of the ML based system.  Attempting to automatically learn such rules may be unnecessary as possibly they are better implemented as a rule in the final design of the ML learning based system.  For example, in a court custody case, if  one parent is violent or emotionally abusive towards the child that parent will probably not get custody of the child.  The final ML based system may embed this fact as a simple rule instead of attempting to automatically learn it.

%Following items should be added/integrated TBC:

%\begin{itemize}
%\item
%Data may or may not include significant signal supporting the business objective. For example, classification of software defects ODC (Orthogonal Defect Classification) \cite{ODC} vs. custom classification.
%\item
%Data may have a signal that is ‘too strong’
%Ex. It is always the case that a defect opened by a manager is of highest importance. No sense in learning this. Use a rule instead
%\end{itemize}

\begin{exercise}
\label{twoExp}
Experiment first. This section describe two experiments that one may carry out in the case of the child custody example.   Explicitly identify the two experiments.    
\end{exercise}

\begin{exercise}
\label{betterRule}
In the child custody case, we want to determine if the ML model is better than the rules or not.  Suggest an approach to define what "better" means here. 
\end{exercise}



\begin{exercise}
\label{forgetTime}
A knight (we assume knights always tell the truth but maybe not the whole truth) is giving us a hundred balls half of them are red and half are blue.  He says that he obtained them randomly.  We decide to give equal probability to getting a blue or a red ball from the knight and act accordingly in the future.  We do so and get another batch with roughly a quarter of the balls being red.    Answer the following questions.
\begin{itemize}
    \item Under the assumption that the balls are obtained with equal probability what is the probability of getting the second batch?
    \item Provide a situation under which the second batch is likely but the knight is still telling the truth.  Explain.  Hint - One possible explanations follow.  You may come up with another explanation.  Assume that the knight has two bags.  One of the bags contain $\frac{1}{4}$ red balls and the rest blue and another bag contains $\frac{3}{4}$ of the balls red balls and the rest blue.  The knight randomly chooses a balls from the first bag at night and a ball from the second bag during the day. 
    \item If the knight is making his choices at equal time intervals.  Suggest conditions of the relevant length of the day and the night and the length of the time interval that will yield the first batch?
    \item What is the probable time in which the knight made the second batch? 
    \item Suggest factors that we did not take into account when making the first prediction?
\end{itemize}

\end{exercise}

\section{Think science and experiments}

We have already stressed the importance of the scientific approach and the design of experiments in the development of a ML system in chapter \ref{Chapter:scientific-method}
and the previous section.  Specifically, we discussed the identification and quantitative definition of the ML system business objectives.   The quantitative business objectives constitute the dependent variables of our experiments. In addition, the factors that impact the ML system performance should be identified. They constitute the independent variable of our experiment.  We next discuss additional aspects of the experiment design.

Statistical stratification means partitioning of the data.  It may be suggested by the factor that we identified.   Ensuring that we have sufficient data in each element of the partition with a proportion that represents the expected proportion in the real population helps better test the system through our experiment.  Such data preparation may also help the training process of the ML models developed for the ML system.  As the next example demonstrate stratification of the data can also be used to represent additional requirements on the ML system. 

\begin{example}
We are creating a ML system that helps determine if a work candidate will be a successful programmer.  In addition to the accurate estimation of whether or not that candidate will be a successful programmer, which is the main business requirement, the system is required to be fair, in the sense that it does not estimate that a candidate will not be successful because of its gender. We thus partition the data into two sets, namely, male and female candidates, check the performance of the ML system on each partition element to determine if there is a bias in the ML system decision and if in fact the ML system decides with higher probability that the candidate will not be a good programmer if presented with a female candidate. 
\end{example}

\begin{exercise}
\label{factorCombinations}
We have determine that the ML system decision will be impacted by the following factors - gender, height, age.  We have further determined that it is sufficient to consider three categories of height namely, $height = \{tall, average, short\}$, and two categories of age, namely, $age = \{young, adult\}$.  Answer the following.
\begin{enumerate}
    \item Suggest a partition based on the above independent variables.  How many elements are there in the partition?
    \item We find out that the data does not have any examples of tall, young females.  Is that a problem?  
\end{enumerate}
\end{exercise}

The measure we will use to test the ML system in our experiment need to quantify and represent a business requirement..

An ML model has standard measures that can be used to determine the quality of the model.   For example, if a model implements a binary classification task, e.g., to distinguish between a cat and a dog, accuracy is such a standard applicable measure that can be used to determine the quality of the ML model.  Accuracy here means the percentage of time the model identifies correctly the object, in our case the dogs and the cats.  

In contrast, a ML system is composed of ML models and standard software, and typically will have a business measure that determines if the ML system is functioning correctly that does not necessarily match any standard ML model measure.   For example, a self driving car may be required to cause zero accidents with injuries. Note that a self driving car is typically implemented as a ML system with many ML models and regular software combined together. Possible one such model will be identifying "other vehicles".  Such a model accuracy does not maps or indicates in an obvious way if the self driving car can cause an accident with injuries or not.   Thus, designing an experiment that estimates the accuracy of the vehicles identification ML model is necessary but not sufficient to determining if the ML system will meet its business requirements.   

Even if a ML standard off the shelf measures may be used to estimate the quality of the ML system it may be needed to customize the standard off the shelf model to accurately represent the business requirements.  For example, in the example of estimating if a candidate will be a good programmer the ML model may make two types of errors, namely, the ML model may decide that a good programmer is a bad programmer or decide that a bad programmer is a good programmer.  In the first case the company will not hire a good programmer.   If there are many candidates, the only harm to the company is a negligible delay in hiring and the overhead involved in interviewing candidates.  ON the other hand, if a candidate that is hired turned out to be a bad programmer, the impact on the company time to market is huge.  As a result the two type of errors can not be treated equally and the generic accuracy measure should be modified, probably by associating appropriate loss with each type of error, to more accurately reflect the desired business result.  

\begin{exercise}
\label{mindDirectingErrorType}
A ML system should identify cats and dogs or a state that it is neither.  List all type of errors such a system may have. We have run an experiment and it turns out that the system accurately identifies cats and dogs 80 percent of the time.  Is the accuracy measure enough to determine if the system met its requirements?  Explain.
\end{exercise}


%I-infused solutions are heavily dependent on data and are statistically correct by nature: they are by definition sometimes correct and sometimes incorrect. It's the nature of the beast. Business-grade AI-infused solutions need to control the statistical error.  Experimental design approaches should thus be introduced and analyzed. These experiments are equated with ML learning iterations.   This will be further explained here.  To reduce the main risk of AI-infused systems development, frequent experimentation is desirable and architecture should be driven by the experimental results.  Consider a sailing ship attempting to reach point B from point A.   The wind is not going from B to A and needs to be harnessed for the boat to reach its destination. In our case, the wind is the data and the sailing ship is the AI-infused system under development and the harnessing process is realized through experiments.   

%TBC:
%\begin{itemize}
%    \item Explain the scientific method
%    \item Explain design of statistical experiments
%    \item Map statistical experiments to machine learning
%\end{itemize}

\section{Data must be of valuable volume; When not to use learning}

Systems scale in complexity from the ones for which we cannot even list the factors that control them to the ones for which we can easily write their equations, e.g., a physical body that accelerates under a constant force. In such a case use rules; ML may be an overkill. An intermediate situation is where the equation is known but a few constants should be empirically calculated, e.g.,  system performance tuning.  Maybe a few cycles of experiments will do in such a case.  Yet another intermediary case where ML shines is when only a general form is known (a model).  We need to think of the choice of a ML technique as a choice of such a model.  For example, a neural network is a model with a graph of thousands of neurons, where the connecting edges are associated with weights.  Together the set of all weights is our model, and we are tasked with finding the best set of weights.  


Even if we decided to apply learning, sufficient data is required to succeed. A rule of thumb for data sufficiency is that the size of the training data should be an order of magnitude bigger, e.g., at least 10x, than the number of parameters in the ML model.  Another rule of thumb is that if a classification task is attempted, the number of examples per label should be at least 30.  The next few exercises and their solution shade some light on these rules of thumbs.  


\begin{exercise}
\label{mindDirectingHOwMuchData}
In \cite{books/daglib/0033642} bounds are developed to determine how much data is needed to enable learning.   The interested reader can review the discussion of the fundamental theorem of PAC learning in chapter six.  For the purpose of this question the details of the theory are not important.  It is sufficient to observe that if we are willing to allow the system to make a mistake $\epsilon$ percentage of the time then the data should be on the order of $ d \times \frac{log(\frac{1}{\epsilon})}{\epsilon}$ records.  Log here is of base 2.  Heuristically, we will consider $d$ to be some notion of the complexity of the problem, e.g., the number of parameters in the ML model.  Given that $\epsilon = 0.05$ and given that the number of parameters in the ML model is d=300, how much data do we need in order to learn according to this heuristic?     
\end{exercise}




TBC:

\begin{itemize}
    \item is the training data representative of the deployment data?
    \item Remember that you also need data for testing
When training – development set – used multiple times 
When testing – test set – you cannot use it to change your model! If you do, you will need more data for testing
    \item Remember labels. You cannot learn labels that are not in the training set. Need to understand and control labeling mistake rate (see Estimate the probability of a labeling mistake)
    \item Is data adequate for learning? A hybrid approach
\end{itemize}










\section{Use all relevant data and information: Do NOT ignore structure}
\label{mindDirecting}

When designing an AI-infused solution, you will typically consider some desired business value and a given source of data.  For example, the business objective states that "given 1000 tickets (problem reports), try to determine the nature of the problem automatically".  Don’t accept the given data as the only source of information. Instead, explore other possible sources through the following heuristics.  

\begin{itemize}
    \item Exploiting implicit data
    \item Taking advantage of meta data associated with the data you were given
    \item Consider implicit or explicit tracability and represent the data in such a way that takes advantage of these relations
    \item Structure contains information.  Resist the temptation to lose structure in order to apply some ML algorithm. Maybe the data was exported and structure lost.   Try in such cases to reverse engineer the structure.  
\end{itemize}

We'll elaborate on these heuristics here.

  

TBC:

\begin{itemize}
    \item Explain the heuristics : "implicit", "meta data", "traceability" and "structure". 
    \item Use all relevant data: Do NOT ignore structured data!
\end{itemize}


\section{Is the training data representative of deployment data?}

TBC:

Assumption underlying statistical machine learning: the training and test data distributions represent the deployment distribution.  In fact, many times the data is collected in a totally different way than the data the system will encounter during deployment.  For example, if self-driving car is trained in different weather conditions or in different countries.  Another example is that data collected is different due to problems in measurements or different scales

How to handle:

Missing data - The scale is different (camera is positioned higher), Use knowledge about the data distribution to determine if the data meets reality

Domain knowledge:

If you know that percentage of fatal side effects is negligible and you get data that has 0.80 fatal side effects, then something is wrong with the data.  Another example of domain knowledge.  Breast cancer percentage in the population is around 0.5

Statistical relations on data:

Capture and monitor feature relations and behavior (min/max, correlation,…)
Hands-on: 


Otherwise you need to design experiments so that you demonstrate that your model monotonically improves with new data as you know that the data will change over time and your data is not representative.   

\section{Get to a supervised learning problem}

ML shines when supervised learning can be applied.  It is more mature and has a stronger success record.  It’s also an indirect indication that you are able to quantify a business objective that will be used in testing the system.  Accurate labels are required for training and testing.  The challenge is to identify appropriate labels for the data.  

Two general heuristics apply:

\begin{itemize}
\item
Choose a subset of the attributes in the data for the labels.
\item
Create an experiment that will generate desired labeled data.
\end{itemize}

TBC:
To predict system performance, a labeled test set will be required. 

\section{Minimize manual labeling, instead utilize experiments, rules and boosting}



TBC - minimize remove hyper parameters.






==> numpy.tex <==
\noindent The actual data in the dataframe is actually an \textit{ndarray} in NumPy (A multidimensional homogeneous array). That means we can do operations on the data using NumPy. For example, if you have a dataframe \textit{df1}, the \textit{ndarray} would be extracted by doing

\begin{lstlisting}[style=python]
nd1 = df1.values
\end{lstlisting}

\noindent Accessing a cell in the array is as simple as:

\begin{lstlisting}[style=python]
val = nd1[row,col]
\end{lstlisting}

\noindent You can also access subarrays by indexing with the colon:

\begin{lstlisting}[style=python]
sub = nd1[0:3,1:3]
\end{lstlisting}

\noindent would capture the rectangular subarray from the first to the third rows and the second to third columns.

\paragraph{Indexing} Note that the second part of the index is 1 past the actual index that will be the last, so 0:3 only pulls out 0,1, and 2.

\noindent Like in MATLAB, you can pull out everything using just the colon. For example:

\begin{lstlisting}[style=python]
sub = nd1[3,:]
\end{lstlisting}

\noindent would retrieve all columns of row 3.

\paragraph{Negative indexing} To get the last index, you can use negative numbers (the last index would be -1, second to last -2, etc.)

\begin{lstlisting}[style=python]
sub = nd1[-1,1:3]
\end{lstlisting}

\noindent would get columns 1,2 of the last row.

\paragraph{Boolean indexing/masking} Suppose we want to get the values in an array, $a$, which are all less than the mean. NumPy's masking feature makes it really intuitive, as all you need to do is:

\begin{lstlisting}[style=python]
lessThanMean = a[a<a.mean()]
\end{lstlisting}

\noindent The array $a < a.mean()$ would be a boolean array, which might look like
\begin{lstlisting}[style=python]
[[True, True, False, False]]
\end{lstlisting}

\paragraph{Assignment} Assigning values in an array is easy using the NumPy notation. For example, say we wanted to replace the values in the first 2x2 square of \textit{nd1} with the 2x2 square in nd2 with columns 2 and 3, and rows 3, and 4. The operation would be:

\begin{lstlisting}[style=python]
nd1[0:2,0:2] = nd2[-2:,2:4]
\end{lstlisting}

\paragraph{Creating an array} Creating a numpy array is as easy as passing in a normal python list into the array method:

\begin{lstlisting}[style=python]
import numpy as np

print np.array([1,2,3])
\end{lstlisting}

\noindent Creating a 2D $mxn$ array is as simple as passing in a $m$-long list of $n$-tuples.

\begin{lstlisting}[style=python]
import numpy as np

print np.array([(1,2,3),(4,5,6)])
\end{lstlisting}

\noindent would output

\begin{lstlisting}[style=python]
[[1,2,3]
 [4,5,6]]
\end{lstlisting}

\paragraph{More initializers} You can also create arrays with certain initial values.

\begin{lstlisting}[style=python]
np.empty((5,3,2))
\end{lstlisting}

\noindent initializes an "empty" $5x3x2$ dimensional array. The values in the array are actually whatever was in the memory locations of the array pointers, so the output could look like garbage.

\begin{lstlisting}[style=python]
np.ones((5,4), dtype=np.int)
\end{lstlisting}

\noindent creates a $5x4$ array, where the value in each cell is the integer 1.

\begin{lstlisting}[style=python]
np.random.random((5,4))
\end{lstlisting}

\noindent creates a $5x4$ array with random numbers from a uniform distribution in [0.0,1.0). An example result could be:

\begin{lstlisting}[style=python]
[[ 0.82897637  0.36449978  0.91209931  0.96307279]
 [ 0.63777312  0.24482194  0.5817991   0.18043012]
 [ 0.85871221  0.98874123  0.68491831  0.53831711]
 [ 0.52908238  0.81083147  0.97440602  0.81032768]
 [ 0.98566222  0.38902445  0.16922005  0.0873198 ]]
\end{lstlisting}

\noindent Other methods or fields, such as $sum()$ or $size$ can be looked up in online documentation.

==> python_highlighting.tex <==
\definecolor{Code}{rgb}{0,0,0}
\definecolor{Decorators}{rgb}{0.5,0.5,0.5}
\definecolor{Numbers}{rgb}{0.5,0,0}
\definecolor{MatchingBrackets}{rgb}{0.25,0.5,0.5}
\definecolor{Keywords}{rgb}{0,0,1}
\definecolor{self}{rgb}{0,0,0}
\definecolor{Strings}{rgb}{0,0.63,0}
\definecolor{Comments}{rgb}{0,0.63,1}
\definecolor{Backquotes}{rgb}{0,0,0}
\definecolor{Classname}{rgb}{0,0,0}
\definecolor{FunctionName}{rgb}{0,0,.7}
\definecolor{Operators}{rgb}{0,0,0}
\definecolor{Background}{rgb}{0.98,0.98,0.98}

\lstdefinestyle{python}{
  numbers=left,
  numberstyle=\footnotesize,
  numbersep=1em,
  xleftmargin=1em,
  framextopmargin=2em,
  framexbottommargin=2em,
  showspaces=false,
  showtabs=false,
  showstringspaces=false,
  frame=l,
  tabsize=4,
  % Basic
  basicstyle=\ttfamily\small\setstretch{1},
  backgroundcolor=\color{Background},
  language=Python,
  % Comments
  commentstyle=\color{Comments}\slshape,
  % Strings
  stringstyle=\color{Strings},
  morecomment=[s][\color{Strings}]{"""}{"""},
  morecomment=[s][\color{Strings}]{'''}{'''},
  % keywords
  morekeywords={import,from,class,def,for,while,if,is,in,elif,else,not,and,or,print,break,continue,return,True,False,None,access,as,,del,except,exec,finally,global,import,lambda,pass,print,raise,try,assert},
  keywordstyle={\color{Keywords}\bfseries},
  % additional keywords
  morekeywords={[2]@invariant},
  keywordstyle={[2]\color{Decorators}\slshape},
  emph={self},
  emphstyle={\color{self}\slshape},
  breaklines=true
}

==> statistics.tex <==
\chapter{Statistical Analysis of Time Series Data}

\noindent Pandas makes it simple to perform statistical analysis on dataframes, which is extremely important in determining different indicators and acting as inputs to the learning algorithms.\\

\section{Global statistics}
\noindent For example, if you had a dataframe $df1$ which had the closing prices for various stocks over a given time period, you can retrieve an ndarray with the mean of the columns by just calling $df1.mean()$.

\begin{figure}[h]
\begin{lstlisting}[style=python]
SPY     126.396777
IBM     166.380238
GLD     145.029775
AAPL    399.498435
XOM      77.054682
dtype: float64
\end{lstlisting}
\caption{Example output array for $mean()$ (called on closing prices for January 2010 through December 2012)}
\end{figure}

\noindent In addition to $mean$, there around 32 other global statistics that are available in pandas.

\section{Rolling statistics}

\noindent Instead of doing analysis on the entire dataset, you might want to do a rolling analysis, which only looks at certain snapshots of the data to sample. For example, you could have a 20-day moving mean, which you would calculate day-by-day by averaging the last 20 days' data. In later sections, this moving average will be explained in more detail, but some critical points of interest are when the moving average crosses the data.

\subsection{Bollinger bands\textsuperscript{\textregistered}}

\noindent Some analysts believe that significant deviations from the moving mean will result in movement back towards the mean. If the price dips far below the mean, then it might be a buy signal, whereas if it goes too high, it could indicate a time to sell. Bollinger bands are a way of measuring this deviation.\\

\noindent Bollinger observed that if you look at the volatility of the stock, and if it's too large, then you discard the movements above and below the mean, but if it's not, then it might be worth paying attention to.\\

\noindent What he did was place two new moving means, one $2\sigma$ above, and another $2\sigma$ below the moving average. If you look at deviations near to $2\sigma$, then they're worth paying attention to. If the price drops \textit{below} $2\sigma$, and then rises back up through it, then it could be a buy signal. (the price is moving back towards the average).\\

\noindent Conversely, if the price rises above $2\sigma$, then falls back down, it could be a sell signal.

\subsection{Computing rolling statistics in pandas}
\noindent Pandas provides some methods to easily calculate rolling mean ($rolling\_mean()$) and rolling standard deviation ($rolling\_std$).\\

\noindent\begin{minipage}{\linewidth}

\noindent\textit{example 11:} Calculating a 20-day rolling mean

\lstinputlisting[style=python,firstline=37,lastline=37]{code_examples/statistics_1.py}
\end{minipage}

\begin{figure}[h!]
	\centering
	\includegraphics[width=\textwidth]{images/bollinger_bands.png}
    \caption{Plot of rolling mean for \textit{SPY} with Bollinger bands\textsuperscript{\textregistered}}
\end{figure}
\newpage

\noindent The Bollinger bands\textsuperscript{\textregistered} were calculated as follows:\\

\noindent\textit{example 12:} Calculating bollinger bands

\lstinputlisting[style=python]{code_examples/statistics_1.py}

\section{Daily returns}
\noindent Daily returns are how much a stock's price went up or down on a given day. They are an extremely important statistic as they can be a good comparison between different stocks.

\begin{equation*}
	daily\_ret[t] = \frac{price[t]-price[t-1]}{price[t-1]} = \frac{price[t]}{price[t-1]}-1
\end{equation*}

\begin{lstlisting}[style=python]
daily_ret = (df / df.shift(1).values) - 1
daily_ret.ix[0,:] = 0
\end{lstlisting}

\begin{figure}[h!]
	\centering
	\includegraphics[width=\textwidth]{images/daily_returns.png}
    \caption{Plot of \textit{IBM}'s prices (top) with daily returns (bottom)}
\end{figure}

\section{Cumulative Returns}
\noindent Cumulative return is calculated by finding the gain from the beginning of the range to the current time, i.e.

\begin{equation*}
	cum\_ret[t] = \frac{price[t]}{price[0]}-1
\end{equation*}

\noindent For example, if the price at the beginning was \$125, and the current price is \$142, then the gain/cumulative return is $\frac{142}{125}-1 = .136 (13.6\%)$\\

\noindent Cumulative returns are essentially the original dataset normalized.

\section{Incomplete data}
\noindent People assume that financial data is extremely well-documented and that perfect data is recorded minute by minute. They also believe that there are no gaps or missing data points. However, for any particular stock, it might have different prices on different stock exchanges! It's difficult to know who's right all the time. Also, not all stocks trade every day (they might suddenly start trading or stop trading).\\

\noindent You might think you can just interpolate the data between breaks, but that'd cause statistical errors and a side-effect of "looking into the future" when doing analysis on that subset of data. The better way of doing it to minimize error is to fill forward and backwards.

\subsection{Filling}
\noindent To fix the "NaN"/empty data, you can use filling to maintain the last known value until known data is reached. For example, if you had a stock that didn't have data until 2001 and then stopped having data in 2006 but then started having data again in 2012, you could fill forward from 2006-2012 and then fill backwards from 2001 back to whenever you want your data to start.\\

\noindent\begin{minipage}{\linewidth}

\noindent\textit{example 13:} Filling in missing data using $fillna()$
\begin{lstlisting}[style=python]
df = get_data(symbols,dates)

df.fillna(method="ffill",inplace=True)
df.fillna(method="bfill",inplace=True)
\end{lstlisting}
\end{minipage}

\begin{figure}[h!]
	\centering
	\includegraphics[width=\textwidth]{images/filled_data.png}
    \caption{Data will forward and backwards filled values (horizontal lines)}
\end{figure}
\newpage

\section{Histograms and scatter plots}
\noindent It's difficult to draw conclusions directly from daily returns plots, so histograms make it easier to see what's going on. A histogram allows you to see how many occurrences of each return happens relative to other returns. This histogram typically follows a Gaussian over large periods of time.\\

\subsection{Histograms}

\noindent From the histogram we can determine a few key statistics: mean, standard deviation, and kurtosis. Kurtosis is a measure of how close the curve is to a Gaussian. In stock data, there are usually more occurrences at high deviations (causing sort of "fat tails"), which would be reflected as a positive kurtosis. Skinny tails would mean a negative kurtosis.

\begin{figure}[h!]
	\centering
	\includegraphics[width=\textwidth]{images/histograms_1.png}
    \caption{Histogram of daily returns \textit{SPY} from January 2009 through December 2012}
\end{figure}
\newpage

\noindent\begin{minipage}{\linewidth}
\noindent\textit{example 14:} Getting a histogram
\noindent The histogram above was generated by just calling $hist()$ on the daily returns dataframe as such:

\begin{lstlisting}[style=python]
daily_returns.hist(bins=20)
\end{lstlisting}
\end{minipage}

\noindent The $bins$ parameter is essentially the resolution of the histogram. The domain is divided into 20 bins and anything within those bins counts for that bin's count in the histogram.

\noindent Other statistics like mean and standard deviation are easily calculated:

\noindent\begin{minipage}{\linewidth}
\begin{lstlisting}[style=python]
mean = daily_returns['SPY'].mean()
print "mean=",mean

std = daily_returns['SPY'].std()
print "std deviation=",std
\end{lstlisting}
\end{minipage}

\noindent\begin{minipage}{\linewidth}
\noindent Which outputs:
\begin{lstlisting}[style=python]
mean= 0.000509326569142
std deviation= 0.0130565407719
\end{lstlisting}
\end{minipage}

\noindent\begin{minipage}{\linewidth}
\noindent We can now plot the mean and standard deviations on the plot to make analysis easier:
\begin{lstlisting}[style=python]
plt.axvline(mean,color='w',linestyle='dashed',linewidth=2)
plt.axvline(mean+std,color='r',linestyle='dashed',linewidth=2)
plt.axvline(mean-std,color='r',linestyle='dashed',linewidth=2)
\end{lstlisting}
\end{minipage}

\begin{figure}[h!]
	\centering
	\includegraphics[width=\textwidth]{images/histograms_2.png}
    \caption{Histogram with mean (white) and $1\sigma$ (red) plotted}
\end{figure}

\noindent\begin{minipage}{\linewidth}
\noindent The output of
\begin{lstlisting}[style=python]
print daily_returns.kurtosis()
\end{lstlisting}
\end{minipage}

\noindent\begin{minipage}{\linewidth}
\noindent is:
\begin{lstlisting}[style=python]
SPY    3.376644
\end{lstlisting}
\end{minipage}

\noindent which means that the data has fat tails since it's positive.\\

\noindent The utility of these histograms comes when plotting them together. It's easy to compare multiple stocks in terms of their returns and volatility. If stock A's curve is skewed more positive and is thinner than stock B, then it has a low volatility with higher returns vs stock B.\\

\begin{figure}[h!]
	\centering
	\includegraphics[width=\textwidth]{images/histograms_comparison.png}
    \caption{Histogram comparison of \textit{SPY} and \textit{XOM}}
\end{figure}
\newpage
\noindent By looking at this chart, you can see that \textit{SPY} and \textit{XOM} are about the same in volatility ($\sigma_{SPY} = .013057, \sigma_{XOM} = .013647$). However, \textit{SPY} would have higher returns since $\overline{R_{SPY}} = .000509$ whereas $\overline{R_{XOM}} = .000151$ 

\subsection{Scatter plots}
\noindent Scatter plots are another way of visualizing the correlation between two stocks. Say you had a dataframe with the daily returns for \textit{SPY} and \textit{XYZ}. If you took just the $ndarray$ containing the y-axis values, and then plotted \textit{SPY} on the x-axis and \textit{XYZ} on the y-axis, you would see a bunch of points that might have a certain trend.\\

\noindent If you take a linear regression of this data, the slope would be called the beta ($\beta$) value. If the $\beta$ value for \textit{SPY} and \textit{XYZ} is 1, it means that, on average, if \textit{SPY} (the market) moves up by 1\%, then \textit{XYZ} also moves up by 1\%.\\

\noindent The y-intercept of the line is called $\alpha$. It describes how the stock on the y-axis performs with respect the stock on the x-axis. If the $\alpha$ value of \textit{XYZ} with respect to \textit{SPY} is positive, then, on average, \textit{XYZ} is returning more than the market overall.

\paragraph{Correlation} If there isn't any correlation in the dataset, then the linear regression doesn't tell you anything about the relationship. A common method for calculating the correlation is by finding the \textit{sample Pearson correlation coefficient, $r_{xy}$}. It's calculated by the following:

\begin{equation*}
	r_{xy} = \frac{cov(X,Y)}{\sigma_{X}\sigma_{Y}} = \frac{\sum_{i=1}^{n}(x_i - \bar{x})(y_i - \bar{y})}{\sqrt{\sum_{i=1}^{n}(x_i - \bar{x})^2}\sqrt{\sum_{i=1}^{n}(y_i - \bar{y})^2}}
\end{equation*}

where $cov$ is the covariance. In this case, X would be the daily return for \textit{SPY} and Y would be the daily return for \textit{XYZ}.
\noindent If $|r_{X,Y}| = 1$, then the two are perfectly correlated (either positively or negatively, depending on the sign of $\rho$). If $|r| < 1$, then there is possible correlation, but a value closer to 1 means better correlation. If $r = 0$, there is no correlation. \\

\noindent\begin{minipage}{\linewidth}
\noindent\textit{example 15:} Plotting scatter plots, getting $\alpha$ and $\beta$ values, and determining correlation
\begin{lstlisting}[style=python]
# scatter plot for XOM vs SPY
daily_ret.plot(kind='scatter',x='SPY',y='XOM',title="Scatter plot")
beta_XOM,alpha_XOM = np.polyfit(daily_ret['SPY'],daily_ret['XOM'],1)
plt.plot(daily_ret['SPY'],beta_XOM*daily_ret['SPY']+alpha_XOM,'-',color='r')
plt.show()

# scatter plot for GLD vs SPY
daily_ret.plot(kind='scatter',x='SPY',y='GLD',title="Scatter plot")
beta_GLD,alpha_GLD = np.polyfit(daily_ret['SPY'],daily_ret['GLD'],1)
plt.plot(daily_ret['SPY'],beta_GLD*daily_ret['SPY']+alpha_GLD,'-',color='r')
plt.show()

print "Beta XOM: ", beta_XOM
print "Alpha XOM: ",alpha_XOM
print "Beta GLD: ",beta_GLD
print "Alpha GLD: ",alpha_GLD

# calculate correlation using pearson method
print "Correlation matrix: \n", daily_ret.corr(method='pearson')
\end{lstlisting}
\end{minipage}
\noindent which outputs:
\begin{lstlisting}[style=python]
Beta XOM:  0.85753872112
Alpha XOM:  -0.000285580653638
Beta GLD:  0.0663816850634
Alpha GLD:  0.000660583984316
Correlation matrix: 
          SPY       XOM       GLD
SPY  1.000000  0.820423  0.074771
XOM  0.820423  1.000000  0.079401
GLD  0.074771  0.079401  1.000000
\end{lstlisting}

\noindent Looking at the $\beta$ values, you can see that \textit{XOM} is more responsive to market changes, while \textit{GLD} is relatively unresponsive. However, \textit{GLD} tends to perform better than the market on average, since its $\alpha$ is positive.\\

\noindent But these values are meaningless without seeing what their correlations are. Looking at the correlation matrix, \textit{XOM} is pretty well correlated with \textit{SPY}, whereas \textit{GLD} has a very low correlation, so changes \textit{GLD} aren't really correlated with changes in the market.

\begin{figure}[h!]
	\centering
    \subcaptionbox{\textit{XOM}}[.45\linewidth]{
    	\includegraphics[width=.5\linewidth]{images/scatter_XOM.png}
    }
    \subcaptionbox{\textit{GLD}}[.45\linewidth]{
    	\includegraphics[width=.5\linewidth]{images/scatter_GLD.png}
    }
    \caption{Scatter plots for \textit{XOM} and \textit{GLD}}
\end{figure}
\newpage

\noindent Looking at the plots, it's easy to see that the points for \textit{XOM} are more correlated and match the line better than do those of \textit{GLD}.

\section{Sharpe ratio and other portfolio statistics}

\noindent The \textbf{portfolio} is the collection of all stocks currently owned by a person. It's important to know various statistics associated with the portfolio to make informed decisions on what to sell/buy.

\noindent Suppose you begin with a portfolio $p$ consisting of the following parameters:
\begin{lstlisting}[style=python]
start_val = 1000000
start_date = '2009-01-01'
end_date = '2011-12-31'
symbols = ['SPY','XOM','GOOG','GLD']
allocs = [0.4, 0.4, 0.1, 0.1] # @ beginning, 40% to SPY, 40% to XOM, etc
\end{lstlisting}

\noindent Now suppose we want to find the value of this portfolio day-by-day. If we normalize the portfolio dataframe, we essentially have a dataframe containing cumulative returns for each index. If we multiply this by $allocs$, we get returns scaled by each percentage of the total portfolio. Then, multiply by $start\_val$ to get each stock's total value. Finally, take the sum of this penultimate dataframe to get a single-column dataframe with the total portfolio value at each point in time. In Python,

\noindent\begin{minipage}{\linewidth}
\begin{lstlisting}[style=python]
# get cumulative returns
df = get_data(symbols,pd.date_range(start_date,end_date))
df = normalize(df)

# get changes for each stock by their percentages of the starting value
alloced = df*allocs

# get dollar value of changes
vals = alloced*start_val

# sum to get total value
portfolio_value = vals.sum(axis=1)
\end{lstlisting}
\end{minipage}

\noindent We may now compute various statistics on the portfolio's value.

\paragraph{Daily returns} Obviously, daily returns of the entire portfolio would be an important statistic, as they indicate how the portfolio changes over time. For some statistics, we need to get rid of the 0 at the beginning of the daily return or else it'll throw off the values.

\begin{lstlisting}[style=python]
daily_rets = daily_rets[1:]
\end{lstlisting}

\paragraph{Cumulative returns} The total cumulative return of the portfolio is another interesting statistic, as you can see if the overall gain was positive or negative.
\begin{lstlisting}[style=python]
cum_ret = (port_val[-1]/port_val.ix[0,:]) - 1
\end{lstlisting}

\paragraph{Avg. and Std. Deviation} These two are the main statistics that get thrown off by the 0 at the beginning. If it were there, the mean would be closer to 0, even though technically 0 isn't actually one of the returns.

\begin{lstlisting}[style=python]
avg_daily_ret = daily_rets.mean()
std_daily_ret = daily_rest.std()
\end{lstlisting}

\subsection{Sharpe Ratio}
\noindent The \textbf{Sharpe Ratio} is a metric that adjusts return for risk. It enables a quantitative way to compare two stocks in terms of their returns and volatility. The Sharpe Ratio is calculated based on the assumption that, \textit{Ceteris paribus}\footnote{all else held equal},
\begin{itemize}
	\item Lower risk is better
    \item Higher return is better
\end{itemize}
Being an economic indicator, it also takes into account the opportunity cost/return of putting the money in a risk-free asset such as a bank account with interest.

\noindent A sort of risk-adjusted return may be calculated as follows:
\begin{equation*}
	R_{adj} = \frac{R_p - R_f}{\sigma_p}
\end{equation*}
where $R_p$ is the portfolio return, $R_f$ is the risk-free rate of return, and $\sigma_p$ is the volatility of the portfolio return.

\noindent This ratio is a sort of basis for how the Sharpe Ratio is calculated. The Sharpe Ratio is as follows:

\begin{equation*}
	S = \frac{E[R_p - R_f]}{std(R_p-R_f)}
\end{equation*}

\noindent Since we're looking at past data, the expected value is actually the mean of the dataset, so this becomes:\\

\begin{equation*}
	S = \frac{\overline{(R_p - R_f)}}{std(R_p-R_f)}
\end{equation*}

\noindent One question is where $R_f$ comes from. There are three main ways of getting the data for the risk-free rate:
\begin{enumerate}
	\item The London Inter-Bank Offer Rate (LIBOR)
	\item The interest rate on the 3-month Treasury bill
    \item 0\% (what people have been using recently...)
\end{enumerate}

\noindent LIBOR changes each day, and the Treasury bill changes slightly each day, but interest in bank accounts are typically paid in 6-month or yearly intervals. Using this simple trick, you can convert the annual/biannual amount to a daily amount:\\

\noindent Suppose the yearly interest rate is $I$. If we start at the beginning of the year with a value $P$, the new value after interest is paid will be $P'$. To find the equivalent daily interest value, $I_{eq}$,

\begin{align*}
	P' &= P(1+I_{eq})^{252}\\
    P(1+I) &= P(1+I_{eq})^{252}\\
    1+I &= (1+I_{eq})^{252}\\
    (1+I_{eq}) &= \sqrt[\leftroot{-2}\uproot{2}252]{1+I}\\
    I_{eq} &= \sqrt[\leftroot{-2}\uproot{2}252]{1+I} - 1
\end{align*}

\noindent Therefore, $R_f$, the daily risk-free rate, is just $\sqrt[\leftroot{-2}\uproot{2}252]{1+I} - 1$. The reason it's 252 instead of 365 is because there are only 252 trading days in a year.\\

\noindent Since we're treating $R_f$ as constant, the standard deviation in the denominator just becomes $std(R_p)$, so the final equation for the Sharpe Ratio becomes:

\begin{equation*}
	S = \frac{\overline{(R_p - R_f)}}{\sigma_{R_p}}
\end{equation*}

\paragraph{Sampling rate} The Sharpe Ratio can vary widely depending on the sampling frequency. Since SR is an annual measure, any calculations that are done with samples more frequent than yearly need to be scaled to get the annual ratio. To adjust the calculated Sharpe Ratio to be "annualized", you just multiply by a factor of $\sqrt{\# samples\ per\ year}$. So if you sample daily, the Sharpe Ratio would become:

\begin{equation*}
	S = \frac{\overline{(R_p - R_f)}}{\sigma_{R_p}}\sqrt{252}
\end{equation*}

\noindent\textit{example:} Given 60 days of data with the following statistics:\\
\noindent$R_p = 10 bps$\\
$R_f = 2 bps$\\
$\sigma_{R_p} = 10 bps$,\\
what is the Sharpe Ratio? One $bps$ is one hundredth of a percent.

\begin{equation*}
	S = \frac{\overline{(R_p - R_f)}}{\sigma_{R_p}} = \frac{10-2}{10}\sqrt{252} 
    \approx 12.70
\end{equation*}

\section{Optimizers}
\noindent An optimizer can:
\begin{itemize}
  \item Find minimum/maximum values of functions
  \item Build parameterized models based on data
  \item Refine allocations to stocks in portfolios
\end{itemize}

\noindent For example, say you have the function $f(x) = (x-1.5)^2 + .5$, and you want to find the minimum. It's trivial to use calculus and find the minimum analytically, but you can't always do so if you don't have an analytical model of the data. Let's put this in Python:

\noindent\begin{minipage}{\linewidth}
\begin{lstlisting}[style=python]
import pandas as pd
import matplotlib.pyplot as plt
import numpy as np
import scipy.optimize as spo

def f(x):
	y = (x-1.5)**2 + .5
	print "x = {}, y = {}".format(x,y)
	return y
    
def test_run():
 	guess = 2.0
	min_result = spo.minimize(f, guess, method='SLSQP', options={'disp':True})
	print "minima found at:"
	print "x = {}, y = {}".format(min_result.x,min_result.fun)
    
if __name__ == "__main__":
	test_run()
\end{lstlisting}
\end{minipage}

\noindent\begin{minipage}{\linewidth}
\noindent outputs:
\begin{lstlisting}[style=python]
x = [ 2.], y = [ 0.75]
x = [ 2.], y = [ 0.75]
x = [ 2.00000001], y = [ 0.75000001]
x = [ 0.99999999], y = [ 0.75000001]
x = [ 1.5], y = [ 0.5]
x = [ 1.5], y = [ 0.5]
x = [ 1.50000001], y = [ 0.5]
Optimization terminated successfully.    (Exit mode 0)
            Current function value: [ 0.5]
            Iterations: 2
            Function evaluations: 7
            Gradient evaluations: 2
minima found at:
x = [ 1.5], y = [ 0.5]
\end{lstlisting}
\end{minipage}

\begin{figure}[h!]
	\centering
	\includegraphics[width=\linewidth]{images/minima.png}
    \caption{Numerical solution to finding the minimum of $f(x) = (x-1.5)^2 + .5$}
\end{figure}
\newpage

\subsection{Pitfalls}
\noindent Optimizers aren't perfect, and since the method used above uses the gradient of the current point to move to the next point, it can be tripped up by various abnormalities in the function it's trying to minimize, such as:

\begin{itemize}
\item\textit{Flat ranges:} If a portion of the graph is flat (the slope is close to or is 0), then the solver will either take a lot of iterations to solve for the minimum or it might not ever be able to move to a new point, unless it can find a way out.
\item\textit{Discontinuities:} If there are discontinuities, the gradient might not be defined well enough for the solver to continue.
\item\textit{Multiple minima:} Say you have a function $f(x) = x^4-2x^2+x^2$. This function has 2 minima at $(0,0)\ and\ (1,0)$. If the solver starts at $x=1.5$, it'll find the minimum at $(1,0)$, but it won't ever reach the other minimum. Conversely, if the solver starts at $x=-1.5$, it'll find the minimum at $(0,0)$. Therefore, it's easy to get trapped in a local minimum that may not be the actual \textit{global} minimum.
\end{itemize}

\subsection{Convex problems}
\noindent A real-valued function $f(x)$ defined on an interval is called \textbf{convex} if the line segment between any two points on the graph of $f(x)$ on that interval lies above the graph. Otherwise, it's called \textbf{non-convex}.

\subsection{Building a parameterized model}
\noindent If you have a set of data points representing rainfall and humidity that were gathered, you might want to find a function that best fits those points. Say you wanted to fit a line $f(x) = mx + b$ to the points. In this case, you can use linear algebra and find the least-squares solution, but you can also use an optimizer to find the \textit{best} parameters $m$ and $b$.\\

\noindent What does "best" mean? Well, we can devise a measure for the error for each point:

\begin{equation*}
	e_i = (y_i - f(x_i))^2 = (y_i - (mx_i+b))^2
\end{equation*}

\noindent which is just the difference between the actual value and our model's predicted value. The reason it's squared is to ensure that negative errors don't reduce the total error when we sum up every $e_i$. 
\begin{equation*}
	E = \sum^{n}_{i=1}(y_i - (mx_i+b))^2
\end{equation*}
\noindent Now that we have what we want to minimize, $E$, we can use a minimizer to find the best $m$ and $b$. To make the parameters nicer to work with in Python (and allow generalization to higher degrees of polynomials), we'll rename $m$ and $b$ to $C_0$ and $C_1$. Now, $f(x) = C_ox+C_1$.

\noindent\begin{minipage}{\linewidth}
\noindent\textit{example 16:}
\begin{lstlisting}[style=python]
import pandas as pandas
import matplotlib.pyplot as plt
import numpy as np
import scipy.optimize as spo

# line is a tuple (C0, C1)
def error(line, data):
	return np.sum((data[:,1] - (line[0]*data[:,0] + line[1])) ** 2)

def fit_line(data,error_func):
	# initial guess for parameters
	l = np.float32([0, np.mean(data[:,1])])

	return spo.minimize(error_func, l, args=(data,), method='SLSQP', options={'disp':True}).x

def test_run():
	original = np.float32([4,2])
	print "original line: C0 = {}, C1 = {}".format(original[0],original[1])
	Xoriginal = np.linspace(0,10,40)
	Yoriginal = original[0]*Xoriginal + original[1]

	plt.plot(Xoriginal,Yoriginal,'b--',linewidth=2.0,label="Original line")

	# add some random noise to the data
	noise_sigma = 4.0
	noise = np.random.normal(0,noise_sigma,Yoriginal.shape)
	data = np.asarray([Xoriginal,Yoriginal+noise]).T

	plt.plot(data[:,0],data[:,1], 'go', label="Data points")

	l_fit = fit_line(data,error)
	print "Fitted line: C0 = {}, C1 = {}".format(l_fit[0],l_fit[1])
	plt.plot(data[:,0],l_fit[0]*data[:,0] + l_fit[1],'r--', linewidth=2.0,label="Fitted line")

	plt.legend(loc='upper right')
	plt.show()

if __name__ == "__main__":
	test_run()
\end{lstlisting}
\end{minipage}
 the minimizer.
\begin{figure}[h!]
	\centering
	\includegraphics[width=\linewidth]{images/line_fit.png}
    \caption{Line of best fit found using parametric mininimization}
\end{figure}
\newpage

\noindent An example of extending $fit\_line$ to higher-degree polynomials can be found in the appendix.

\section{Portfolio Optimization}
\noindent Now that wee have the tools to optimize a function, we can use it to optimize our portfolio! We can choose to optimize/minimize/maximize various measures, such as daily returns, cumulative returns, or Sharpe Ratio based on the percent allocation of all of the stocks in the portfolio.

\subsection{Framing the problem}
\noindent First we need three things:
\begin{enumerate}
\item a function, $f(x)$, to minimize
\item an initial guess for $x$
\item the optimizer
\end{enumerate}

\noindent In our case, $x$ is actually the set of allocations for the stocks. Also, since we want to maximize Sharpe Ratio, we need to multiply $f(x)$ by -1 to call the minimizer.

==> thanks.tex <==
\chapter*{Thanks}
\label{Chapter:thanks}

We thank Guy Barash for working out solutions for the programming and experiments exercises, Krithika Prakash for commenting on the early text and discussion on the exercises, Diptikalyan Saha for discussion on the unit test vs. system test chapter, Radha Ratnaparkhi for discussion and insights on the unit and system testing concept, and Rakesh Ranjan for discussion, feedback and insights on the early versions of the ML pitfalls material.   

==> unitTestSystemTest.tex <==
\chapter{Unit Test vs. System Test of ML Based Systems}
\label{unitSystem}

Why do we need more than one model to build a system?   Possibly, we can always feedback the entire data to the machine learning algorithm and produce the desired system?  Let's consider the following example. 

\begin{example}
\label{whyDecompose}
Consider a system that identifies the type of vehicle in an image.  We desire a rough classification into land vehicles that requires a track and those that do not, boats, submarines and flying vehicles.   The images have reliable meta data that clearly state if the vehicle is a land vehicle or not.  We could create two possible systems. We could try and build a monolithic model by training a model using the images and their meta data.  Another option is to create a model, $M_1$, that identifies boats, submarines and flying vehicles assuming that the input images are not land vehicles and another model, $M_2$, that identifies if the images are land vehicles that requires a track or not assuming that the vehicles are land vehicles.  We will then compose the two models to get our system in the following way. We will check the meta data of the image to determine if the vehicle is a land vehicle or not.  We will then apply $M_1$ if the image is not a land vehicle and $M_2$ if it is.  Which of the options is better?  As we assumed that the rule is reliable and it seems reasonable to assume that it is stable over time we can probably assume that the second system is much better.  In addition, the learning task in the second case are easier as we have less labels to classify so we may achieve better generalization overall.   
\end{example}

\begin{exercise}
What happens in the two cases if the vehicle is amphibious?
Try different possible assumption on the meta data categorization and analyze how the two possible systems are likely to behave under your assumptions.  
\end{exercise}

The example above demonstrates why a hybrid system composed of ML models and deterministic rules may be the ideal architectural choice.  Another interesting aspect of system decomposition for ML based systems is that its design should be driven by the data available for learning.  To see why, consider a system we would like to develop that assists in diagnosing a patient. There are many medical conditions and most of them are rare. Thus, we may have just a few examples for most of the medical conditions.  As a result, it may prove impossible to train a ML model that successfully predicts that the medical condition is a rare medical condition.  There are simply not enough examples for the ML to generalize and predict in the case of rare conditions!  This is a special case of stratification or slices on the independent variables that do not have enough training examples.  For example, we may know that cities and neighborhoods are both independent variables, that will affect whether or not a child will graduate from school, but we do not have examples for some of the cities or neighborhoods for which we would like to apply the model. Thus, we probably cannot train a ML model to predicts on those combinations of neighborhoods and cities for which we do not have training examples. Instead, the general rules is that slices for which there is not enough training data should be handled in the old fashion by developing deterministic rules that apply to them.  Again, the result is a hybrid system.

\begin{exercise}
\label{excercise:402}
We know that for some $a \in R$ the system is of the form $f(x) = Ax^2$ for $x > a$ and $f(x) = Bx$ when $x \leq a$.  You are given a training set $D = \{ (3, 9), (4, 16), (5, 25), (6, 36), (7, 49)\}$ where for a given point $(x, y)$ in the data set we know that $f(x) = y$.  Which of the following parameters $a, A, B$ can be learned and why?.  Next, assume that $a = 0$, $A = 1$ and $B = -1$. Attempt the following:
\begin{enumerate}
    \item Write a program that randomly generates data for the above case.  
    \item Implement a learning algorithm that will learn $a, A, B$ in this case.  Generalize your data generating process so that it will randomly generate legal data for random choices of $a, A, B$.  Show that your algorithms learns for a random sample of data generated by your data generating program.  
    \item Is your ML algorithm a composition of several ML algorithms or a monolithic solution?  Why did you chose one solution over the other and what were the trade offs that you took into account? 
\end{enumerate}

\href{https://colab.research.google.com/drive/1TlQUi7BaUvwXx3MOvyuIhLKmuc98U3x5?usp=sharing}{Click here for solution} or see solution \ref{excercise:402_sol} in  appendix \ref{chapter:solution_appendix}.
\end{exercise}

For regular systems components or units provide a well defined deterministic interface and they interact at the various levels of the system, create composed components and eventually obtain the desired system objective. Thus, testing for regular software consists of validating the expected deterministic behaviour of the system at each level of components composition. 

For ML based systems, testing consists, in addition to traditional testing, of experiments on random performance variables that needs to be controlled at the different system levels. In addition, the random performance variables need not be the same at all levels of the system. We may thus be interested in the accuracy of intent classifiers of the chatbot solution at the unit level but the average number of service calls that are directed to a human agent at the system level (see chapter \ref{industrial} for details).  Thus, experiments need to be conducted at the unit and system levels to establish control over their their associated and typically different random performance variables. In general any component of the system that has at least one ML model embedded in it will require validation of control of some random performance variables through appropriate experiments.  

As mentioned above, an interesting curiosity of the process of crafting ML based systems is that the optimal architecture is "driven by the data".   Thus, experiments not only serve to test the system but also to design it. In addition, the line between testing and designing is blurred.  We have seen how weakness in training data for slices of the data may drive the decomposition of the system.  Such weaknesses are discovered through experiments. Thus, indeed, the results of the experiments and the data available drive the design of the system. 

It is interesting to note that some view test first for regular software as a design paradigm. From that perspective the analogy between test first for regular software and experiment first for ML embedded systems is strengthen as both approaches are said to drive the design of the system.  

\begin{exercise}
Consider a complete rooted binary tree of depth n (i.e., a path from the root to a leaf has n vertices).  Each node in the tree represents a decision the software is making.  In addition, assume the decision at node $v$ of the tree has error probability $p_v$.   An adversary chooses a path, $v_1, \ldots, v_n$ from the root $v_1$ to a leaf $v_n$. A decision is then made by the system by making a decision at each node of $v_i$ with error probability $p_{v_i}$.  The system makes a correct decision only if all decisions along the path are correct. 
\begin{enumerate}
    \item What is the probability of making a correct decision if $v_1, \ldots, v_n$ is chosen by the adversary?
    \item Which path should the adversary choose?
    \item Implement an algorithm that finds the path the adversary should choose.  What is its running time and is that the best running time possible?
\end{enumerate}
\end{exercise}

A useful abstraction that applies to many ML based systems and will help us better understand the fundamental challenges of crafting ML based systems is a decision tree.   The system is using the decision tree to make decisions.  The nodes of the decision tree are decision point and can utilize either some deterministic rule or a ML model.  If the ML model is used at a decision tree node to make a decision, the decision is correct in probability and its correctness probability may also dependent on the independent variables that govern the system.   We refer to such a decision tree as the ML system hybrid decision tree.  For a detail example of such a system see the chatbot example in \ref{industrial}.  In that example the system uses intent classifiers to decide what the customer is interested in (paying a bill, withdrawing money from their account, etc), the system then proceed to follow a deterministic decision process that obtain the necessary data from the customer and complete the required service.  Given a system with a hybrid decision tree, we can now elaborate on the challenges encountered in testing it as follows.  We will refer below to nodes that use ML models to make a decision as non deterministic nodes and node that use rules to make the decisions as deterministic nodes.

\begin{enumerate}
    \item Each non deterministic node performance dependent variables needs to be identified and statistically controlled through an appropriated experiment. Note that there could be more than one dependent variable to analyze per non deterministic node.  For example, if the decision is whether or not to report some new drug side effect to the government, it may be more important that we report a true new side effect than that we do not report the new side effect when there is one. Thus, the two possible error types, namely reporting on a new side effect when it is not a new side effect or not reporting on a new side effect when it is a new side effect needs to be analyzed.\footnote{TBC - explain why you are not using standard terminology - false negative, false positive, precision and recall.  Not everything is binary..} 
    \item Is the hybrid decision tree the best way to design the system?   Can we suggest a different hybrid decision tree that will better utilize the data and get a better overall performance or a more stable one?
    \item Is the performance of the entire hybrid decision tree satisfactory?   What are the performance variables that need to be analyzed for the entire system?  These overall system performance variables need to be analyzed for each path in the hybrid decision tree that contain a non deterministic node. Some times we can deduce the analysis from the experiments on non deterministic nodes along a path (see proceeding exercises), but most likely we will need to conduct new experiments to test the entire path's performance.     
\end{enumerate}

The following exercises are designed to  clarify the concepts of unit test, system test, and system design using the hybrid decision tree for ML based systems. 

\begin{exercise}
Developers developed a classification model as part of a larger system and wanted to test it.  In order to do that they have obtained a new labeled data set, T, that is representative of the data that will be encountered when the model is deployed as part of the system and that was not used to develop the model.  They calculated the accuracy of the model, i.e., the percentage of correct answers the model gave on T, and the number was $95\%$ which seems to be a good number so they concluded that the model is validated.
\begin{enumerate}
    \item The probability that the model is less than $93\%$ accurate is required to be less than $0.05$.  Can we conclude that the model met this requirement?
    \item Is there anything wrong with what the developers have done?   Discuss your answer in light of statistical stability and system business requirements.  
    \item The classification problem is a binary calcification problem with two possible labels, -1 and 1.  T has 1000 data points 500 of label 1 and 500 of label -1.   On label 1 there are 10 mistakes and on label -1 there are 40 mistakes made by the model. What is the probability of mistake given that the label is -1 or given that the label is 1?  
    \item Every time the model makes a mistake on label 1 the company losses $100\$$ and when a mistake is done on label -1 the company losses $50\$$.   What is the expected loss from a 1000 data points encountered by the system? 
    \item The data in production drifted and now we expect 900 out of a 1000 records to be of label -1.  The model conditional probability of making a mistake on each of the labels (-1 and 1) remains the same.  What is the expected loss of the company on 1000 data point encountered by the system now?
\end{enumerate}
\end{exercise}

\begin{exercise}
To follow the experiment first approach, we use the following steps:
\begin{enumerate}
    \item Identify a requirement and quantify it resulting in a dependent variable we want to analyze through an appropriate experiment.  
    \item Use domain knowledge to identify the independent variables that impact the above dependent variable.
    \item Design an experiment that will predict the relation between the dependent and independent variables.  The dependent variable will be estimated using the result of applying the ML based system or any of its components on the system inputs.  Which part of the system is applied dependents on the level in which the test is conducted.  In the hybrid decision tree model the test may apply to a non deterministic node in the tree or to the entire tree.
\end{enumerate}

Consider the following questions.
\begin{enumerate}
\item Is there a difference in the statistical techniques that are applied to a non deterministic node in the decision tree or to a path in the hybrid decision tree?
\item Does it make sense to apply statistical tests to other parts of the hybrid decision tree (other than a path or a node)?
\item Consider your answer to the previous question.  How would you define unit test and system test in light of your answer?
\end{enumerate}

\end{exercise}

\begin{exercise}
Isaac Asimov defines his three laws of robotic in his 1942 short story "Runaround".  The laws read 
\begin{enumerate}
    \item First Law. A robot may not injure a human being or, through inaction, allow a human being to come to harm.
    \item Second Law. A robot must obey the orders given it by human beings except where such orders would conflict with the First Law.
    \item Third Law. A robot must protect its own existence as long as such protection does not conflict with the First or Second Law.
\end{enumerate}
Define a non deterministic decision tree that implements the above laws and is as "doable" as possible with the current state of the art of ML.
\end{exercise}


==> video.tex <==
\chapter{Videos}

In this chapter we provide videos that supports the text.  The videos are associated with the text through appropriate internal links.

The following videos discusses the testing of ML systems and is associated with chapter \ref{Chapter:MLtesting} introduction and section \ref{randomVariable}.

This video gives an overview of the chapter and discusses the concept of a random variable and its distribution. \href{https://www.youtube.com/watch?v=tW5_kKQHgtg&list=PLC7m9qp0Q1Ydn7ZtR9yeI46yHw-4q11iI&index=2}{\textbf{See link here}}.

This video covers basic properties of the expectation and variance of a random variable.   \href{https://www.youtube.com/watch?v=suGPMSPad70&list=PLC7m9qp0Q1Ydn7ZtR9yeI46yHw-4q11iI&index=6}{\textbf{See link here}}.

A Video covering Chapter \ref{Chapter:drift}, \textbf{Drift Detection and ML Solution Retraining} is available here -  
\href{https://youtu.be/ZoQDK3byQq4}{\textbf{part 1}},
\href{https://youtu.be/5hB-lXnkyX8}{\textbf{part 2}},
\href{https://youtu.be/EAHgLTkugas}{\textbf{part 3}},
\href{https://youtu.be/RwcEW5AHg7s}{\textbf{part 4}}.
